MTFuzz: Fuzzing with a Multi-Task Neural Network

Fuzzing is a widely used technique for detecting software bugs and vulnerabilities. Most popular fuzzers generate new inputs using an evolutionary search to maximize code coverage. Essentially, these fuzzers start with a set of seed inputs, mutate them to generate new inputs, and identify the promising inputs using an evolutionary fitness function for further mutation. Despite their success, evolutionary fuzzers tend to get stuck in long sequences of unproductive mutations. In recent years, machine learning (ML) based mutation strategies have reported promising results. However, the existing ML-based fuzzers are limited by the lack of quality and diversity of the training data. As the input space of the target programs is high dimensional and sparse, it is prohibitively expensive to collect many diverse samples demonstrating successful and unsuccessful mutations to train the model. In this paper, we address these issues by using a Multi-Task Neural Network that can learn a compact embedding of the input space based on diverse training samples for multiple related tasks (i.e., predicting for different types of coverage). The compact embedding can guide the mutation process by focusing most of the mutations on the parts of the embedding where the gradient is high. \tool uncovers $11$ previously unseen bugs and achieves an average of $2\times$ more edge coverage compared with 5 state-of-the-art fuzzer on 10 real-world programs.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)

==> body/1_intro_back.tex <==
\section{Introduction}

%% NOTE: What is the domain? (Opening: Introduce the main topic this paper addresses) 
Coverage-guided graybox fuzzing is a widely used technique for detecting bugs and security vulnerabilities in real-world software~\cite{zalewski2017american, cgc, zalewski2017american, manes2018fuzzing,wang2019superion,Nilizadeh2019,You2019SLFFW,lemieux2017fairfuzz,she2018neuzz, godefroid2008, arya2012fuzzing, evans2011fuzzing, moroz2016guided}. The key idea behind a fuzzer is to execute the target program on a large number of automatically generated test inputs and monitor the corresponding executions for buggy behaviors. However, as the input space of a program is typically very large, unguided test input generation is not very effective at finding bugs.
%% NOTE: How the current non-ml fuzzers do it? 
Therefore, most popular graybox fuzzers use evolutionary search to generate new inputs; they \textit{mutate} a set of \textit{seed inputs} and retain only the most promising inputs (\ie, inputs exercising new program behavior) for further mutations~\cite{zalewski2017american, wang2019superion,Nilizadeh2019,You2019SLFFW, wei2018singularity, steelix, godefroid2017learn,lemieux2017fairfuzz,jiang2018contractfuzzer}.

%% NOTE: What is the problem with non-ml based fuzzers.  
The effectiveness of traditional evolutionary fuzzers tends to decrease significantly over fuzzing time. They often get stuck in long sequences of unfruitful mutations, failing to generate inputs that explore new regions of the target program~\cite{chen2018angora, she2018neuzz, she2019neutaint}. Several researchers have worked on designing different mutation strategies based on various program behavior (e.g., focusing on rare branches, call context, etc.)\needcitation. However, program behavior changes drastically, not only across different programs but also across different parts of the same program. Thus, finding a generic robust mutation strategy still remains subject to active research. 

Recently,  Machine Learning (ML) techniques have shown initial promise to guide the fuzzers~\cite{Saavedra2019, she2018neuzz, Rajpal2017}\rahul{check this ?}. 
These fuzzers typically use existing test inputs to train ML models such that the models can learn to identify promising mutation regions that improve coverage~\cite{she2018neuzz, godefroid2017learn, Rajpal2017, Saavedra2019}. Like any supervised learning techniques, the success of these models relies heavily on the amount and quality of training data. 
However, collecting such training data for fuzzing that can demonstrate successful/unsuccessful mutations is prohibitively expensive. 
First of all, successful mutations that increase coverage are often limited to very few, sparsely distributed input bytes, commonly known as hot-bytes, in a high-dimensional input space. Generating meaningful test inputs without knowing the distribution of hot-bytes is extremely hard~\cite{she2018neuzz,Saavedra2019}. 
Further, the training data should be diverse enough to expose the model to  various program behavior that lead to successful/unsuccessful mutations---this is also challenging as one would require a large amount of test cases exploring different program semantics. 
Thus, the ML-based fuzzers suffer from {\em sparsity} and {\em lack of diversity} of the target domain. 

To address these problems, Multi-Task Learning is a popular solution in traditional ML, where a Multi-Task Neural Network (MTNN) learns from multiple related tasks that share common lower-level features. 
As all the tasks are noisy but with different noise patterns, the model learning multiple tasks simultaneously can ignore task-specific noise patterns and learn a more generalized feature representation. MTNN can further address the data sparsity problem\textemdash the model can boost the attention to the important features (hot bytes in our case)  as all the participating tasks will provide separate evidences for the relevance or irrelevance of those features~\cite{ruder2017overview}.



%that work across different programs or  which location to mutate and with what values still remain a challenge\textemdash mutation parameters not only vary widely across different test programs but also change drastically across different parts of the same program.
%Research on designing new mutation strategies have not so far yielded robust strategies that work across different test programs\needcitation. 

% Coverage guided graybox fuzzing is a widely used technique for detecting bugs and security vulnerabilities in real-world software systems~\cite{zalewski2017american, cgc, zalewski2017american, manes2018fuzzing, wang2019superion,Nilizadeh2019,You2019SLFFW,lemieux2017fairfuzz,she2018neuzz, godefroid2008, arya2012fuzzing, evans2011fuzzing, moroz2016guided}. Most coverage guided fuzzers use an evolutionary search strategy that \textit{mutates} a set of \textit{seed inputs} to generate new inputs, retaining only most promising new inputs, \ie, inputs that exercise new program behavior. 
% % Mutation forms the backbone of this process. It has been subject to much recent research
% ~\cite{zalewski2017american, wang2019superion, Nilizadeh2019, You2019SLFFW, steelix, godefroid2017learn,lemieux2017fairfuzz,jiang2018contractfuzzer, she2018neuzz, Pham2019, Saavedra2019}. 

% Traditional fuzzing, problems with that, and why we need ML? See~\cite{Saavedra2019, she2018neuzz,Rajpal2017}

%Recently, Machine learning (ML) techniques have been shown initial promise at guiding the input mutations performed during fuzzing ~\cite{Saavedra2019, she2018neuzz, Rajpal2017}. Given a set of seed inputs, these ML-based fuzzers typically train a machine learning model to learn to identify promising mutation regions based on the prior program behaviors or sample inputs~\cite{she2018neuzz, godefroid2017learn, Rajpal2017, Saavedra2019}. While such approaches~\cite{she2018neuzz, godefroid2017learn} have reported promising improvements over traditional evolutionary graybox fuzzers, they still tend to get stuck after a while. 

% \rahul{Version 1:~}The key challenge with existing ML-based fuzzers is that there are not enough interesting input samples (\ie, inputs that trigger unique program behaviors) available to train the ML-model. Consequently, these models tend to \textit{lack generalizibility}. They cannot extrapolate the observations from already explored program states to reason about unseen regions of the program space. As a result, they fail to identify potential mutations that may result in reaching these unseen regions~\cite{she2018neuzz,Saavedra2019}. To overcome this, we would require a sufficiently large number of interesting input samples. However, these interesting inputs are \textit{sparsely} distributed over a high-dimensional space. It is often prohibitively expensive to collect enough interesting inputs to train ML-based fuzzers. {\color{red}\textsc{check!}} For example, it takes about 5 hours to generate about a 1000 samples~\cite{zalewski2017american}. Therefore, in this paper we seek to develop a generic ML-based fuzzer than can explore to program states more effectively with only a limited number of input samples.

% \rahul{Version 2 (same as about para, but rephrased):~}
%The key challenge with existing ML-based fuzzers is that the underlying ML models must learn to extrapolate the observations from program behaviors on already explored inputs to unseen regions of the input space. However, the input space of traditional programs is very large and many of the inputs do not cause any change in the program behavior. Learning over such a sparse function is intrinsically extreme hard due to the difficulties involved in ~\cite{she2018neuzz,Saavedra2019}. 

%these interesting inputs are \textit{sparsely} distributed over a high-dimensional space. Thus, it is often prohibitively expensive to collect enough interesting inputs to train ML-based fuzzers. Therefore, in this paper we seek to develop a generic ML-based fuzzer than can operate more effectively with a limited number of available input samples.


% Existing ML-based fuzzers still face several key challenges that limits their overall efficacy: 
% \begin{itemize}
%   \item \textit{Sparse Input Space}. The interesting inputs (\ie, inputs that explore rare program states) are \textit{sparsely} distributed across a high-dimensional space~\cite{wang2017skyfire, you2019slf}. Consequently, it would be prohibitively expensive to collect enough interesting inputs to train ML-based fuzzers. {\color{gray!70} For example, it takes about 5\textsuperscript{\textbf{\textsc{{\color{red} ??}}}} hours to generate about a 1000\textsuperscript{\textbf{\textsc{{\color{red} ??}}}} samples~\cite{zalewski2017american}}. This is problematic because, the number of interesting inputs are often under-represented in the available samples resulting in ML-models with low accuracy.
%   \item \textit{Lack of generalizibility}. Current ML-based fuzzers are \textit{not generalizable}. They have a limited number of interesting input samples available to build a generalizable ML-model. As a result, ML-based fuzzers
%   %tend to \textit{overfit} to the control-flow edges that have been seen so far. They 
%   cannot extrapolate the observations from already explored program states to reason about previously unseen regions of the program space. This is a challenge because, ML-based fuzzers often fail to identify promising mutations that may potentially lead to reaching these unseen regions of the program space~\cite{she2018neuzz,Saavedra2019}. 
% \end{itemize}


% In this paper we offer an alternative approach. we propose reusing existing input samples to predict for multiple related coverage measure. 

% The key intuition of \tool is that an MTNN can be used to reduce the high dimensional input space into a low dimensional \textit{compact embedding} that captures the program state-space.

To address the limitations of ML-based fuzzers, we propose a novel fuzzing framework called \tool that is based on multi-task neural networks. \tool uses a Multi-task Neural Network (MTNN) to predict for \textit{multiple tasks} (\eg, by predicting various coverage measures~\cite{chen2018angora, mcmaster2008call, Wang2019Be, McMinn2004, arcuri2010does, mcminn2011search, pachauri2013automated} invoked by the input). Each task \textit{reuses} the available inputs to model a different aspect of the program behavior exercised by those inputs. The resulting MTNN generates a single \textit{compact embedding} that captures the most general representation of the inputs applicable to all tasks. \tool can identify the \textit{most pertinent input byte-locations} applicable all tasks by computing gradients over the compact embedding with respect to the inputs. \tool then focuses mutations more on those pertinent byte-locations.




%  

% \rahul{Version 1:~}The key challenge with existing ML-based fuzzers is that there are not enough interesting input samples (\ie, inputs that trigger unique program behaviors) available to train the ML-model. Consequently, these models tend to \textit{lack generalizibility}. They cannot extrapolate the observations from already explored program states to reason about unseen regions of the program space. As a result, they fail to identify potential mutations that may result in reaching these unseen regions~\cite{she2018neuzz,Saavedra2019}. To overcome this, we would require a sufficiently large number of interesting input samples. However, these interesting inputs are \textit{sparsely} distributed over a high-dimensional space. It is often prohibitively expensive to collect enough interesting inputs to train ML-based fuzzers. {\color{red}\textsc{check!}} For example, it takes about 5 hours to generate about a 1000 samples~\cite{zalewski2017american}.
% Therefore, in this paper we seek to develop a generic ML-based fuzzer than can explore to program states more effectively with only a limited number of input samples.



% ~\rahul{V3:~}
% Recently, Machine learning (ML) techniques have been shown to significantly improve the performance of graybox fuzzers~\cite{Saavedra2019, she2018neuzz, Rajpal2017}. ML-based fuzzers use a machine learning model to \textit{learn a mapping} between the input and the corresponding program state. Since the program state is complex with a number interacting variables,  This is typically done by training the ML-models to predict the \ec of the inputs. Then, using a specialized algorithm, they identify promising regions in the input to mutate so as to maximize the coverage of the program's state-space~\cite{she2018neuzz, godefroid2017learn, Rajpal2017, Saavedra2019}. % The quality of the underlying ML-technique dictates the effectiveness of the ML-based fuzzers. 

% Since the program state is complex with a large number interacting variables,
% it is typical to measure the program states using code coverage measures such as \ec. 




% Some previous research have alluded to the possible benefits of incorporating additional coverage code measures~\cite{Wang2019}. \tool is first to successfully develop a generic ML-based greybox fuzzing framework that can.

% \rahul{Version II}~{\color{black!60}~The key challenge with existing ML-based fuzzers is that underlying ML-model is not generalizable, \ie, it cannot extrapolate the observations from already explored program states to reason about previously unseen regions of the program's state-space. This makes it difficult to guide the ML-based fuzzers towards reaching these unseen regions. Typically, to train a generalizable ML-models, we require a sufficiently large number of interesting input samples (\ie, inputs that trigger a wide variety of unique program behaviors). It is often difficult, if not prohibitively expensive, to collect enough interesting inputs since these inputs are \textit{sparsely} distributed over a high-dimensional space. For example, generating about 1000 samples takes about 5 hours~\cite{zalewski2017american}.
% Therefore, the goal of this paper is to develop a generalizable ML-based fuzzer than can operate effectively even when the number available input samples are limited.}

% The key challenge with existing ML-based fuzzers is that underlying ML-model is not generalizable, \ie, it cannot extrapolate the observations from already explored program states to reason about previously unseen regions of the program's state-space. This makes it difficult to guide the ML-based fuzzers towards reaching these unseen regions~\cite{she2018neuzz,Saavedra2019}. Typically, to train a generalized ML-models fail to generalize when the number of interesting inputs (\ie, inputs that invoke new program states) provided to it is inadequate. It is often difficult, if not prohibitively expensive, to collect enough interesting inputs because they are \textit{sparsely} distributed over a high-dimensional space. Therefore, the goal of this paper is to develop a generalizable ML-based fuzzer than can operate effectively even when the number available input samples are limited.   

% The key challenge with existing ML-based fuzzers is that underlying ML-model is not generalizable, \ie, it cannot extrapolate the observations from already explored program states to reason about previously unseen regions of the program's state-space. This makes it difficult to guide the ML-based fuzzers towards reaching these unseen regions. Typically, to train a generalize ML-models fail to generalize when the number of interesting inputs (\ie, inputs that invoke new program states) provided to it is inadequate. It is often difficult, if not prohibitively expensive, to collect enough interesting inputs because they are \textit{sparsely} distributed over a high-dimensional space. Therefore, the goal of this paper is to develop a generalizable ML-based fuzzer than can operate effectively even when the number available input samples are limited.   




% AN alternative to increasing the sample size is to reuse the existing sample to learn how they \texttt{perform??} on alternative measure of \texttt{code coverage???} 
%However, current ML-based greybox fuzzers tend to stuck in long sequences of unfruitful mutations, failing to generate inputs that explore novel regions of the target program~\cite{chen2018angora, she2018neuzz, she2019neutaint}.

% The key challenge in designing an ML-based fuzzers is to answer, . %faced by current ML-based fuzzers is that the accuracy of the underlying ML-model directly affects the efficiency of the ML-based fuzzers. Training accurate ML-models requires a sufficiently large number of interesting input samples (\ie, inputs that trigger a wide variety of unique program behaviors). 
%

% Ideally, ML-based fuzzers would be required to exhaustively sample all the variables in the program's state-space. However, this is prohibitively expensive, since the program's state-space is complex and very large.

% \bi
% \item[\textit{a)}] \textit{Insufficiency of Training data.} The accuracy of the underlying ML-model directly affects the efficiency of the ML-based fuzzers. Training accurate ML-models requires a sufficiently large number of interesting input samples (\ie, inputs that trigger a wide variety of unique program behaviors). However, generating a large number of interesting input samples is very hard because the input space is high-dimensional and inputs triggering interesting program behaviors are sparsely distributed over the input space~\cite{lemieux2017fairfuzz, she2018neuzz, she2019neutaint}.
% \item[\textit{b)}] \textit{Lack of generalizability.} With limited training data, ML-models tend to suffer from \textit{over-fitting}. As a result, current ML-models fail to extend generalization from already seen regions to the previously unseen regions of the program. This makes it difficult to guide the ML-based fuzzers towards reaching these unseen regions. % Furthermore, for every new program, we may have to generate high quality data from scratch. Gathering such data can be quite expensive. 
% \ei
% 

% To address the limitations of ML-based fuzzers, we propose a novel fuzzing framework called \tool that is based on multi-task neural networks. Multi-task Neural Networks (hereafter, \textit{MTNN}) learn to model the relationship between the input and the program state-space in terms of different tasks where Each task represents information about a certain aspect of the program state. The MTNN is trained to predict the response elicited by the input with respect to each of the \textit{tasks} simultaneously~\cite{caruana1996algorithms, caruana1997multitask}. The MTNN offers a single compact representation of the program's state-space 

% \textit{MTNN} have been shown to 
% \begin{inparaenum}[(i)]
%     \item alleviate the data insufficiency problem~\cite{caruana1997multitask, zhang2017survey, Binge2017}, and 
%     \item prevent overfitting by learning a general representation of the input that satisfies all the tasks~\cite{caruana1997multitask,baxter2000model}.
% \end{inparaenum}



%% Add compact embedding here--
% To address the limitations of ML-based fuzzers, we propose a novel fuzzing framework called \tool that is based on multi-task neural networks. The multi-task neural networks (hereafter, \textit{MTNN}) learns to model the relationship between the input and the program state-space.
% The key intuition of \tool is that an MTNN can be used to reduce the high dimensional input space into a low dimensional \textit{compact embedding} that captures the program state-space. 
% This is achieved by training the MTNN to predict for \textit{multiple tasks} (\eg, by predicting various coverage measures~\cite{chen2018angora, mcmaster2008call, Wang2019Be, McMinn2004, arcuri2010does, mcminn2011search, pachauri2013automated} invoked by the input). Each task models a different aspect of the program behavior exercised by a given input. The resulting MTNN generates a single \textit{compact embedding} that captures the program's state-space. By computing the gradient over compact embedding with respect to the inputs we can model the \textit{most pertinent input byte-locations} that apply to all tasks. This information will enable \tool to focus the mutations more on those specific byte-locations.% Consequently, \tool would be able to generate significantly larger high-quality inputs.
% Our results indicate that \tool can significantly outperform the current state-of-the-art ML-based fuzzers. 

% The overview of \tool is shown in \fig{intro_fig}. 
\tool comprises of three stages namely, (i)~multi-task training, (ii)~gradient-guided mutation, and (iii)~incremental learning. In the first stage, we pick a set of inputs from the seed corpus to train an MTNN. The MTNN learns the \textit{program behavior elicited by the input bytes} in terms of three coverage measures (or \textit{tasks}) namely, \ec~\cite{zalewski2017american,she2018neuzz}, \ctx~\cite{chen2018angora,Wang2019}, and \softlabel~\cite{McMinn2004, arcuri2010does, mcminn2011search, pachauri2013automated}. The trained MTNN offers an intermediate compact-embedding. In the second stage, we compute the \textit{gradient} between the compact-embedding layer and the input-layer. The value of the gradient informs the subsequent mutation operation of the most relevant bytes in the input to mutate. In the final stage, we run the newly generated test inputs on the instrumented program and update the seed corpus with the most promising seeds. 

\noindent\textbf{Architecture.}~
The architecture of our MTNN model is specifically designed to faciliate learning a compact-embedding of the program's state-space. It comprises of two groups of layers: 
\begin{itemize}
  \item[\mybullet]\textit{Shared Encoding Layer.}~These comprise of a set of 3 hidden layers (each narrower than its predecessor). These layers are \textit{shared} among all the tasks. The goal of the shared encoding layer is to \textit{distill} the high-dimensional inputs into a \textit{compact-embedding}, \ie, a low-dimensional representation of the input comprising of only the most salient input bytes that matter to all tasks. In essence, this shared encoding represents a neural embedding of the input format.
  \item[\mybullet]\textit{Task specific decoder.}~These consist of a set of decoders (one for each task) that map the shared encoding layer to the output layers specific to each task.    
\end{itemize}


The shared encoding layer offers \textit{a powerful feature extractor} for reducing the complex program state-space into a \textit{low-dimensional compact embedding}. Empirical results demonstrate that fuzzers operating on the compact-embedding are are significantly more effective than those operating on the original program space.

Our architecture offers two key advantages:

\noindent\textbf{Adaptability.}~\tool can be easily adapted to incorporate a diverse set of additional tasks. Theoretical results show that an MTNN can perform just as well when it is extended to include novel tasks~\cite{baxter2000model}. To demonstrate this, we present promising preliminary results with an additional task to assert the validity of newly generated mutants (see RQXX). We make available a replication package\footnote{Replication Package: \href{https://blinded.for.review}{https://blinded.for.review}} in order to enable adding new tasks. These tasks may fall under any category of learning tasks, \eg, supervised (classification/regression), unsupervised, reinforcement learning, etc.

%This paper incorporates 3 coverage metrics--- \ec, \ctx, and \softlabel. 
% These were chosen since they were shown previously to independently have the most impact on improving fuzzing~\cite{zalewski2017american,she2018neuzz,chen2018angora,Wang2019}. 


\noindent\textbf{Transferability.}~\tool can be used to \textit{transfer} the learned compact-embedding among programs that parse similar file formats. In essence, \tool that is modeled on one program can be used to efficiently fuzz a different program that shares the same input, \eg, the compact-embedding learned with \tool for one pdf parser may be transferred to other pdf parsers. Our results (RQ4) show that such transfer is quite effective and it mitigates the need to generate high quality data from scratch for new programs which can be quite expensive.

We evaluate \tool on 9 real world programs against 6 state-of-the-art fuzzers. \tool covers at least a 1000 more edges on 5 programs and several 100 more on the rest. \tool also finds 15 previously unseen real-world bugs (see RQ1). When compared to learning each task individually, \tool offers significantly more edge coverage (see RQ2). Lastly, our results from transfer learning show that the compact-embedding of \tool can be transferred within parsers for pdf, xml, and elf binaries. \tool \textit{offers similar edge coverage} compared to fuzzing with bespoke models that were built from scratch (see RQ3).

Overall, our paper makes the following key contributions:
\bi

\item We present a novel fuzzing framework based on multi-task neural networks called \tool that offers a compact embedding of an otherwise complex and high-dimensional input space.

\item We offer empirical results demonstrating that \tool which operates on the compact-embedding space is significantly more effective than current state-of-the-art fuzzers. \texttt{Needs numbers}.

\item We offer promising results on the transferability of \tool. Results demonstrate that transferred \tool offers competing coverage to non-transfer models. {\texttt{Need Numbers}}.
 
\item We offer an open-source replication package to reproduce and extend \tool at \href{https://blinded.for.review}{https://blinded.for.review}.

\ei


% \squishlist
% \item 
% We propose \tool, a Multi-Task Netural Network adaptive framework that can automatically find good mutation parameter values by learning from diverse information sources (\eg  branch distances~\cite{arcuri2010does}, encoding of new-edges, rare-edges, \etc) collected from program executions. To achieve this, we formulate the problem of finding optimal parameter values as gradient-guided optimization which \tool solves to automatically find the optimal mutation parameters at any given step the of the fuzzing operation.

% \item
% We present a new parameterized mutation scheme that can leverage information about the probability of different control-flow edges being taken in a program for different inputs to distribute the mutations across the input space so that they maximize the chances of new edge discovery. 

% \item
% Our experiments demonstrate that \tool outperforms current state-of-the-art methods in discovering more new-edges (RQ1), rare-edges (RQ3), and novel seeds (RQ2) (see~\tion{rqs}). Our experiments further show that our framework can leverage different types of information sources like a branch-distance~\cite{arcuri2010does} based soft-labeling scheme and a customized loss function to prioritize mutations that might result in exploring rare edges according to our ML model. 

% \item
% We demonstrate that our ML models mapping from program input to the control-flow edge probability space offer a high degree of generalizibility. \tool modeled using inputs from one program can be used to efficiently update the parameters of a similar program (e.g., a program that parses the same file format as the first one). We believe that such sharing of models can potentially result in drastic reduction of fuzzing overhead for programs with share functionalities.
% \squishend

The rest of this paper is structured as follows. \tion{} summarizes . \tion{our_method} describes \tool in detail. 
In \tion{implementation}, we present the instrumentation details followed by answers to our research questions in \tion{rqs}. In \tion{threats}, we list some of the threat to validity of our findings. Other related work in this area are discussed in \tion{related} and conclusion in \tion{conclusion}.


% \subsection{Research Questions}

% \rqone The first RQ assesses the number of bugs found by \tool and the improvements in edge-coverage compared to other state-of-the-art graybox fuzzers. We note that:


% \rqtwo In this RQ, ensembles of each individual task is compared to a multi-task neural-network model. Also, each task (\ie, coverage measures) within \tool is disassembled to study their effect on the overall performance. We show that:

% \begin{goal} 
% Fuzzing with an ensembles of each task is more computationally burdensome than multi-task models (up to 3$\times$). Ensembles also offer inferior edge coverage compared a multi-task models (up to 1000 few edges covered). 
% \end{goal}

% \rqthree We evaluate the transferability of \tool across different programs that share similar input formats. We show that: 

% \begin{goal}
% \tool modeled on one program can be \textit{transferred} to a different program operating on the same input format, \ie, \tool can be transferred within parsers for pdf, xml, and elf binaries. \tool \textit{offers similar edge coverage} compared to fuzzing with bespoke models built from scratch.
% \end{goal}




% Consequently, current graybox fuzzers tend to stuck in long sequences of unfruitful mutations, failing to generate inputs that explore novel regions of the target program~\cite{chen2018angora, she2018neuzz, she2019neutaint}.

% It has been argued that, in order to explore the input space better, one may have to look beyond traditional coverage measures such as \ec so as to model aspects of program behavior that are not fully conveyed by \ec~\cite{chen2018angora, Wang2019Be, GREYONE} . For instance, while \ec measures the number of unique control-flow edges taken by a test-input, it fails to distinguish between inputs that invoke the same control-flow edges but via new internal states (for instance through completely different \textit{call-stack})~\cite{chen2018angora, mcmaster2008call, Wang2019Be}. Such information may be obtained using additional coverage measures such as \ctx~\cite{chen2018angora, Wang2019Be}. Similarly, in order guide fuzzing towards reaching specific branches in the \cfg, it may make sense to use a measure of proximity such as \textit{approach level}~\cite{McMinn2004, arcuri2010does, mcminn2011search, pachauri2013automated}, so as to calculate how close a generated input was to triggering specific control-flow branches. 

% In a recent study, Wang \etal~\cite{Wang2019Be} report that there is no universal best coverage measure. Instead, they demonstrate that it is best to incorporate a combination of coverage measures in order to maximize the fuzzing efficiency. However, the efforts to incorporate these additional coverage metrics by the state-of-the-art fuzzers currently rely on arduous manual instrumentation atop existing fuzzers such as AFL~\cite{zalewski2017american}. As a consequence, current coverage-guide graybox fuzzers lack \textit{extensibility}, \ie, it is difficult to incorporate additional sources of coverage information in the future without significant additional instrumentation. Additionally, it is also hard to determine how generalizable these instrumentations are across programs that exhibit different behavior. 


% \begin{itemize}
%   \item Firstly, t
%   \item Secondly, current ML-based fuzzers can only model the relationship between inputs and the corresponding \ec. It is not clear how to exploit other sources of coverage information such as \ctx or \softlabel. While it may theoretically be possible to build different models for different information sources and combine their results, finding good parameter values, optimizing them, and managing such ensemble models is intractable in practice. Further, training and inference with ensemble models imposes a significant computational overhead slowing down the overall fuzzing process, as shall be shown by this article.
% \end{itemize}

% To overcome these issues, we seek a fuzzer that can:
% \begin{inparaenum}[(i)]
%     \item~Mitigate the problems presented by a sparse and a high-dimensional input space; and 
%     \item~Leverage \textit{multiple} sources of coverage information.  
% \end{inparaenum} 

% To this end, we propose \tool--- a generic fuzzing framework that can learn from several sources of information using a Multi-task Neural Network (hereafter, MTNN). \fig{intro_fig} shows the overview of \tool comprising main three stages that are repeated until the budget allocated for fuzzing is exhausted. In Stage 1, we pick a set of inputs from the seed corpus to train a MTNN. The MTNN learns the \textit{program behavior elicited by the input bytes} in terms of three coverage measures (or \textit{tasks}) namely, \ec, \ctx, and \softlabel. The MTNN architecture used in \tool comprises of two groups of layers: 
% \begin{inparaenum}[(a)]
%   \item A set of hidden layers, \textit{shared} among all the tasks, that encodes the high-dimensional inputs into a compact joint-embedding, \ie, a low-dimensional representation of the input comprising of the most salient input bytes that matter to all tasks; and
%   \item Task specific decoding layers, that learn the relationship between the joint-embedding and the individual tasks.    
% \end{inparaenum}
% Next, in Stage 2, we compute the \textit{gradient} between the joint-embedding layer and the input. The value of the gradient informs the subsequent mutation operation of the most relevant bytes in the input to mutate. Finally, in Stage 3, we run the newly generated test inputs on the instrumented program. We update the seed corpus with the most promising seeds.     

% In summary, this paper makes the following contributions:

% \be
% \item \textit{Extensibility:}~A novel fuzzing framework based on multi-task neural networks called \tool that can incorporate diverse information sources. This paper incorporates 3 coverage metrics--- \ec, and \ctx, \softlabel. Additional metrics may be added using our replication package\footnote{\href{https://blinded.for.review}{https://blinded.for.review}}.
% \item \textit{Compactibility:}~\tool offers a powerful feature extractor for reducing sparse and high-dimensional input in a compact low-dimensional embedding. Empirical results demonstrating that fuzzers operating on the compacted embedding space are more effective.
% \item \textit{Transferability:}~
% \ee

% 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Introduction}


% Coverage guided graybox fuzzing is a widely used technique for detecting bugs and security vulnerabilities in real-world software systems~\cite{zalewski2017american, cgc, zalewski2017american, manes2018fuzzing, wang2019superion,Nilizadeh2019,You2019SLFFW,lemieux2017fairfuzz,she2018neuzz, godefroid2008, arya2012fuzzing, evans2011fuzzing, moroz2016guided}. The key idea behind a fuzzer is to execute the target program on a large number of automatically generated test inputs and monitor the executions for buggy behaviors. However, as the input space of a program is typically very large, unguided test input generation is not effective at finding bugs.

% Most popular fuzzers (especially the graybox ones) use 
% some form of evolutionary search strategy to generate new inputs by \textit{mutating} a set of \textit{seed inputs} and retain only the promising inputs for further mutations that exercise new program behavior~\cite{zalewski2017american, wang2019superion,Nilizadeh2019,You2019SLFFW, wei2018singularity, steelix, godefroid2017learn,lemieux2017fairfuzz,jiang2018contractfuzzer}. 

% However, with time, the evolutionary fuzzers tend to become 
% increasingly less effective at reaching new code locations. 
% Although much research effort has been spent on designing different mutation strategies to increase edge coverage, the success not only varies widely across different test programs but also change drastically depending on the actual input values being mutated.

% Recently, Machine learning (ML) techniques have been shown to significantly improve the performance of graybox fuzzers \cite{Saavedra2019, she2018neuzz,Rajpal2017}.  These, ML-based fuzzers attempt to model a particular information source (\ie, input format) with respect to its coverage behavior. Then, using a specialized algorithm, they identify promising regions in the input to mutate so as to maximize code coverage~\cite{she2018neuzz,godefroid2017learn,Saavedra2019,Rajpal2017}. However, these ML-based fuzzers face two critical challenges that limit their overall efficiency: 
% % \bi
% % \item[\textit{a)}] \textit{Insufficiency of Training data.} The accuracy of the underlying ML-model directly determines the efficiency of the ML-based fuzzers. Training accurate ML-models requires a sufficiently large number of interesting input samples (\ie, inputs that trigger a wide variety of unique program behaviors). However, generating a large number of interesting input samples is very hard because the input space is high-dimensional and inputs triggering interesting program behaviors are sparsely distributed over the input space~\cite{lemieux2017fairfuzz, she2018neuzz, she2019neutaint}.
% % \item[\textit{b)}] \textit{Lack of generalizability.} With limited training data, ML-models tend to suffer from \textit{over-fitting}. As a result, current ML-models fail to extend generalization from already seen regions to the previously unseen regions of the program. This makes it difficult to guide the ML-based fuzzers towards reaching these unseen regions. % Furthermore, for every new program, we may have to generate high quality data from scratch. Gathering such data can be quite expensive. 
% % \ei

% % To address the limitations of ML-based fuzzers, we propose a novel fuzzing framework called \tool based on multi-task deep neural networks. Multi-task Neural Networks (hereafter, \textit{MTNN}) learn to model the relationship between the input and several tasks simultaneously~\cite{caruana1996algorithms, caruana1997multitask}. \textit{MTNN} have been shown to 
% % \begin{inparaenum}[(i)]
% %     \item alleviate the data insufficiency problem~\cite{caruana1997multitask, zhang2017survey, Binge2017}, and 
% %     \item prevent overfitting by learning a general representation of the input that satisfies all the tasks~\cite{caruana1997multitask,baxter2000model}.
% % \end{inparaenum}
% %Our results indicate that \tool can significantly outperform the current state-of-the-art ML-based fuzzers. 

% % \textbf{Compact Embedding.}~

% The key intuition of \tool is that an MTNN can be trained to learn the relationship between the input and various tasks (\eg, coverage measures~\cite{chen2018angora, mcmaster2008call, Wang2019Be, McMinn2004, arcuri2010does, mcminn2011search, pachauri2013automated}) so as to model different aspects of program behavior exercised by the input. This would enable MTNN to model the most pertinent input byte-locations that apply to all tasks. Using this information, \tool can focus the mutations more on those specific byte-locations.% Consequently, \tool would be able to generate significantly larger high-quality inputs.

% \input{tex/fig-1.tex}

% The overview of \tool is shown in \fig{intro_fig}. It comprises of three stages that are repeated iteratively. In Stage 1, we pick a set of inputs from the seed corpus to train an MTNN. The MTNN learns the \textit{program behavior elicited by the input bytes} in terms of three coverage measures (or \textit{tasks}) namely, \ec~\cite{zalewski2017american,she2018neuzz}, \ctx~\cite{chen2018angora,Wang2019}, and \softlabel~\cite{McMinn2004, arcuri2010does, mcminn2011search, pachauri2013automated}. Next, in Stage 2, we compute the \textit{gradient} between the joint-embedding layer and the input-layer. The value of the gradient informs the subsequent mutation operation of the most relevant bytes in the input to mutate. Finally, in Stage 3, we run the newly generated test inputs on the instrumented program and update the seed corpus with the most promising seeds. 

% \tool offers numerous benefits over current ML-based fuzzers:\\
% \noindent\textbf{Compact Embedding.}~
% The architecture of our MTNN model comprises of two groups of layers: 
% \begin{itemize}
%   \item\textit{Shared Encoding Layer.}~These comprise of a set of 3 hidden layers (each narrower than its predecessor). These layers are \textit{shared} among all the tasks. The goal of the shared encoding layer is to \textit{distill} the high-dimensional inputs into a \textit{compact joint-embedding}, \ie, a low-dimensional representation of the input comprising of only the most salient input bytes that matter to all tasks. In essence, this shared encoding represents a neural embedding of the input format.
%   \item\textit{Task specific decoder.}~These consist of a set of decoders (one for each task) that map the shared encoding layer to the output layers specific to each task.    
% \end{itemize}

% The shared encoding layer offers \textit{a powerful feature extractor} for reducing sparse and high-dimensional input into a \textit{compact low-dimensional embedding}. Empirical results demonstrate that fuzzers operating on the low-dimensional joint-embedding are are more effective than those operating on the high-dimensional input layer.\\
% \noindent\textbf{Adaptability.}~\tool can be easily adapted to incorporate a diverse set of additional information sources (as new tasks). Theoretical results show that an MTNN can perform just as well when it is extended to include novel tasks~\cite{baxter2000model}. This paper incorporates 3 coverage metrics--- \ec, \ctx, and \softlabel. These were chosen since they were shown previously to independently have the most impact on improving fuzzing~\cite{zalewski2017american,she2018neuzz,chen2018angora,Wang2019}. Additional tasks may be added using our replication package\footnote{Replication Package: \href{https://blinded.for.review}{https://blinded.for.review}}. These tasks may fall under any category of learning tasks, \eg, supervised (classification/regression), unsupervised, reinforcement learning, etc.\\
% \noindent\textbf{Transferability.}~The joint-embedding layer obtained from~\tool learns a representation  of the input format. 
% This representation can be transferred to programs that parse similar file formats. In essence, \tool that is modeled on one program can be used to efficiently fuzz a different program with very little overhead. This mitigates the need to generate high quality data from scratch for new programs which can be quite expensive.

% The rest of this paper is structured as follows. \tion{} summarizes . \tion{our_method} describes \tool in detail. 
% In \tion{implementation}, we present the instrumentation details followed by answers to our research questions in \tion{rqs}. In \tion{threats}, we list some of the threat to validity of our findings. Other related work in this area are discussed in \tion{related} and conclusion in \tion{conclusion}.


% \subsection{Research Questions}
% We evaluate \tool on 9 real world programs against 6 state-of-the-art fuzzers. The findings of this paper are summarized below as answers to three key research questions. 

% \rqone The first RQ assesses the number of bugs found by \tool and the improvements in edge-coverage compared to other state-of-the-art graybox fuzzers. We note that:

% \begin{goal} 
% \tool covers at least a 1000 more edges on 5 programs and several 100 more on the rest. \tool also finds 15 previously unseen real-world bugs. 
% \end{goal}

% \rqtwo In this RQ, ensembles of each individual task is compared to a multi-task neural-network model. Also, each task (\ie, coverage measures) within \tool is disassembled to study their effect on the overall performance. We show that:

% \begin{goal} 
% Fuzzing with an ensembles of each task is more computationally burdensome than multi-task models (up to 3$\times$). Ensembles also offer inferior edge coverage compared a multi-task models (up to 1000 few edges covered). 
% \end{goal}

% \rqthree We evaluate the transferability of \tool across different programs that share similar input formats. We show that: 

% \begin{goal}
% \tool modeled on one program can be \textit{transferred} to a different program operating on the same input format, \ie, \tool can be transferred within parsers for pdf, xml, and elf binaries. \tool \textit{offers similar edge coverage} compared to fuzzing with bespoke models built from scratch.
% \end{goal}




% % Consequently, current graybox fuzzers tend to stuck in long sequences of unfruitful mutations, failing to generate inputs that explore novel regions of the target program~\cite{chen2018angora, she2018neuzz, she2019neutaint}.

% % It has been argued that, in order to explore the input space better, one may have to look beyond traditional coverage measures such as \ec so as to model aspects of program behavior that are not fully conveyed by \ec~\cite{chen2018angora, Wang2019Be, GREYONE} . For instance, while \ec measures the number of unique control-flow edges taken by a test-input, it fails to distinguish between inputs that invoke the same control-flow edges but via new internal states (for instance through completely different \textit{call-stack})~\cite{chen2018angora, mcmaster2008call, Wang2019Be}. Such information may be obtained using additional coverage measures such as \ctx~\cite{chen2018angora, Wang2019Be}. Similarly, in order guide fuzzing towards reaching specific branches in the \cfg, it may make sense to use a measure of proximity such as \textit{approach level}~\cite{McMinn2004, arcuri2010does, mcminn2011search, pachauri2013automated}, so as to calculate how close a generated input was to triggering specific control-flow branches. 

% % In a recent study, Wang \etal~\cite{Wang2019Be} report that there is no universal best coverage measure. Instead, they demonstrate that it is best to incorporate a combination of coverage measures in order to maximize the fuzzing efficiency. However, the efforts to incorporate these additional coverage metrics by the state-of-the-art fuzzers currently rely on arduous manual instrumentation atop existing fuzzers such as AFL~\cite{zalewski2017american}. As a consequence, current coverage-guide graybox fuzzers lack \textit{extensibility}, \ie, it is difficult to incorporate additional sources of coverage information in the future without significant additional instrumentation. Additionally, it is also hard to determine how generalizable these instrumentations are across programs that exhibit different behavior. 


% % \begin{itemize}
% %   \item Firstly, t
% %   \item Secondly, current ML-based fuzzers can only model the relationship between inputs and the corresponding \ec. It is not clear how to exploit other sources of coverage information such as \ctx or \softlabel. While it may theoretically be possible to build different models for different information sources and combine their results, finding good parameter values, optimizing them, and managing such ensemble models is intractable in practice. Further, training and inference with ensemble models imposes a significant computational overhead slowing down the overall fuzzing process, as shall be shown by this article.
% % \end{itemize}

% % To overcome these issues, we seek a fuzzer that can:
% % \begin{inparaenum}[(i)]
% %     \item~Mitigate the problems presented by a sparse and a high-dimensional input space; and 
% %     \item~Leverage \textit{multiple} sources of coverage information.  
% % \end{inparaenum} 

% % To this end, we propose \tool--- a generic fuzzing framework that can learn from several sources of information using a Multi-task Neural Network (hereafter, MTNN). \fig{intro_fig} shows the overview of \tool comprising main three stages that are repeated until the budget allocated for fuzzing is exhausted. In Stage 1, we pick a set of inputs from the seed corpus to train a MTNN. The MTNN learns the \textit{program behavior elicited by the input bytes} in terms of three coverage measures (or \textit{tasks}) namely, \ec, \ctx, and \softlabel. The MTNN architecture used in \tool comprises of two groups of layers: 
% % \begin{inparaenum}[(a)]
% %   \item A set of hidden layers, \textit{shared} among all the tasks, that encodes the high-dimensional inputs into a compact joint-embedding, \ie, a low-dimensional representation of the input comprising of the most salient input bytes that matter to all tasks; and
% %   \item Task specific decoding layers, that learn the relationship between the joint-embedding and the individual tasks.    
% % \end{inparaenum}
% % Next, in Stage 2, we compute the \textit{gradient} between the joint-embedding layer and the input. The value of the gradient informs the subsequent mutation operation of the most relevant bytes in the input to mutate. Finally, in Stage 3, we run the newly generated test inputs on the instrumented program. We update the seed corpus with the most promising seeds.     

% % In summary, this paper makes the following contributions:

% % \be
% % \item \textit{Extensibility:}~A novel fuzzing framework based on multi-task neural networks called \tool that can incorporate diverse information sources. This paper incorporates 3 coverage metrics--- \ec, and \ctx, \softlabel. Additional metrics may be added using our replication package\footnote{\href{https://blinded.for.review}{https://blinded.for.review}}.
% % \item \textit{Compactibility:}~\tool offers a powerful feature extractor for reducing sparse and high-dimensional input in a compact low-dimensional embedding. Empirical results demonstrating that fuzzers operating on the compacted embedding space are more effective.
% % \item \textit{Transferability:}~
% % \ee

% % 

==> body/1_introduction_v2.tex <==
\section{Introduction}

%% NOTE: What is the domain? (Opening: Introduce the main topic this paper addresses) 
Coverage guided graybox fuzzing is a widely used technique for 
detecting bugs and security vulnerabilities in real-world software systems~\cite{zalewski2017american, cgc, zalewski2017american, manes2018fuzzing,wang2019superion,Nilizadeh2019,You2019SLFFW,lemieux2017fairfuzz,she2018neuzz, godefroid2008, arya2012fuzzing, evans2011fuzzing, moroz2016guided}. The key idea behind a fuzzer is to execute the target program on a large number of automatically generated test inputs and monitor the executions for buggy behaviors. However, as the input space of a program is typically very large, unguided test input generation is not very effective at finding bugs.
%% NOTE: How the current non-ml fuzzers do it? 
Therefore, most popular graybox fuzzers use some form of evolutionary search to generate new inputs; they \textit{mutate} a set of \textit{seed inputs} and retain only the most promising inputs (\ie, inputs exercising new program behavior) for further mutations~\cite{zalewski2017american, wang2019superion,Nilizadeh2019,You2019SLFFW, wei2018singularity, steelix, godefroid2017learn,lemieux2017fairfuzz,jiang2018contractfuzzer}.

%% NOTE: What is the problem with non-ml based fuzzers.  
The effectiveness of traditional evolutionary fuzzers tends to decrease significantly over time. They get often get stuck in long sequences of unfruitful mutations, failing to generate inputs that explore novel regions of the target program~\cite{chen2018angora, she2018neuzz, she2019neutaint}. Research on designing new mutation strategies have so far had varying degrees of success across different test programs\needcitation. 

% Coverage guided graybox fuzzing is a widely used technique for detecting bugs and security vulnerabilities in real-world software systems~\cite{zalewski2017american, cgc, zalewski2017american, manes2018fuzzing, wang2019superion,Nilizadeh2019,You2019SLFFW,lemieux2017fairfuzz,she2018neuzz, godefroid2008, arya2012fuzzing, evans2011fuzzing, moroz2016guided}. Most coverage guided fuzzers use an evolutionary search strategy that \textit{mutates} a set of \textit{seed inputs} to generate new inputs, retaining only most promising new inputs, \ie, inputs that exercise new program behavior. 
% % Mutation forms the backbone of this process. It has been subject to much recent research
% ~\cite{zalewski2017american, wang2019superion, Nilizadeh2019, You2019SLFFW, steelix, godefroid2017learn,lemieux2017fairfuzz,jiang2018contractfuzzer, she2018neuzz, Pham2019, Saavedra2019}. 

% Traditional fuzzing, problems with that, and why we need ML? See~\cite{Saavedra2019, she2018neuzz,Rajpal2017}

Recently, Machine learning (ML) techniques have been shown to significantly improve the performance of graybox fuzzers~\cite{Saavedra2019, she2018neuzz, Rajpal2017}. Given a set of seed inputs, these ML-based fuzzers typically train a machine learning model to learn a mapping between the inputs and the program states they exercise, \ie, the ML-based fuzzers are trained to \textit{predict} for coverage measures such as \ec. Then, using a specialized algorithm, they \textit{identify promising regions in the input} to mutate so as to maximize the code coverage~\cite{she2018neuzz, godefroid2017learn, Rajpal2017, Saavedra2019}. ML-based fuzzers such as Neuzz~\cite{she2018neuzz} and Learn\&Fuzz~\cite{godefroid2017learn} have reported demonstrable improvements over traditional evolutionary graybox fuzzers. 

% \rahul{Version 1:~}The key challenge with existing ML-based fuzzers is that there are not enough interesting input samples (\ie, inputs that trigger unique program behaviors) available to train the ML-model. Consequently, these models tend to \textit{lack generalizibility}. They cannot extrapolate the observations from already explored program states to reason about unseen regions of the program space. As a result, they fail to identify potential mutations that may result in reaching these unseen regions~\cite{she2018neuzz,Saavedra2019}. To overcome this, we would require a sufficiently large number of interesting input samples. However, these interesting inputs are \textit{sparsely} distributed over a high-dimensional space. It is often prohibitively expensive to collect enough interesting inputs to train ML-based fuzzers. {\color{red}\textsc{check!}} For example, it takes about 5 hours to generate about a 1000 samples~\cite{zalewski2017american}. Therefore, in this paper we seek to develop a generic ML-based fuzzer than can explore to program states more effectively with only a limited number of input samples.

% \rahul{Version 2 (same as about para, but rephrased):~}
The key challenge with existing ML-based fuzzers is that they are \textit{not generalizable}. They cannot extrapolate the observations from already explored program states to reason about unseen regions of the program space. As a result, they fail to identify promising mutations that may potentially lead to these unseen regions of the program space~\cite{she2018neuzz,Saavedra2019}. To overcome this, we would need to acquire a sufficiently large number of interesting input samples (\ie, inputs that trigger unique program behaviors) to train the ML-based fuzzer. However, these interesting inputs are \textit{sparsely} distributed over a high-dimensional space. Thus, it is often prohibitively expensive to collect enough interesting inputs to train ML-based fuzzers. %For example, it takes about 5 hours to generating about a 1000 samples~\cite{zalewski2017american}. 
Therefore, in this paper we seek to develop a generic ML-based fuzzer than can operate more effectively with a limited number of available input samples.


% Existing ML-based fuzzers still face several key challenges that limits their overall efficacy: 
% \begin{itemize}
%   \item \textit{Sparse Input Space}. The interesting inputs (\ie, inputs that explore rare program states) are \textit{sparsely} distributed across a high-dimensional space~\cite{wang2017skyfire, you2019slf}. Consequently, it would be prohibitively expensive to collect enough interesting inputs to train ML-based fuzzers. {\color{gray!70} For example, it takes about 5\textsuperscript{\textbf{\textsc{{\color{red} ??}}}} hours to generate about a 1000\textsuperscript{\textbf{\textsc{{\color{red} ??}}}} samples~\cite{zalewski2017american}}. This is problematic because, the number of interesting inputs are often under-represented in the available samples resulting in ML-models with low accuracy.
%   \item \textit{Lack of generalizibility}. Current ML-based fuzzers are \textit{not generalizable}. They have a limited number of interesting input samples available to build a generalizable ML-model. As a result, ML-based fuzzers
%   %tend to \textit{overfit} to the control-flow edges that have been seen so far. They 
%   cannot extrapolate the observations from already explored program states to reason about previously unseen regions of the program space. This is a challenge because, ML-based fuzzers often fail to identify promising mutations that may potentially lead to reaching these unseen regions of the program space~\cite{she2018neuzz,Saavedra2019}. 
% \end{itemize}


% In this paper we offer an alternative approach. we propose reusing existing input samples to predict for multiple related coverage measure. 

% The key intuition of \tool is that an MTNN can be used to reduce the high dimensional input space into a low dimensional \textit{compact embedding} that captures the program state-space.

To address the limitations of ML-based fuzzers, we propose a novel fuzzing framework called \tool that is based on multi-task neural networks. \tool uses a Multi-task Neural Network (MTNN) to predict for \textit{multiple tasks} (\eg, by predicting various coverage measures~\cite{chen2018angora, mcmaster2008call, Wang2019Be, McMinn2004, arcuri2010does, mcminn2011search, pachauri2013automated} invoked by the input). Each task \textit{reuses} the available inputs to model a different aspect of the program behavior exercised by those inputs. The resulting MTNN generates a single \textit{compact embedding} that captures the most general representation of the inputs applicable to all tasks. \tool can identify the \textit{most pertinent input byte-locations} applicable all tasks by computing gradients over the compact embedding with respect to the inputs. \tool then focuses mutations more on those pertinent byte-locations.




%  

% \rahul{Version 1:~}The key challenge with existing ML-based fuzzers is that there are not enough interesting input samples (\ie, inputs that trigger unique program behaviors) available to train the ML-model. Consequently, these models tend to \textit{lack generalizibility}. They cannot extrapolate the observations from already explored program states to reason about unseen regions of the program space. As a result, they fail to identify potential mutations that may result in reaching these unseen regions~\cite{she2018neuzz,Saavedra2019}. To overcome this, we would require a sufficiently large number of interesting input samples. However, these interesting inputs are \textit{sparsely} distributed over a high-dimensional space. It is often prohibitively expensive to collect enough interesting inputs to train ML-based fuzzers. {\color{red}\textsc{check!}} For example, it takes about 5 hours to generate about a 1000 samples~\cite{zalewski2017american}.
% Therefore, in this paper we seek to develop a generic ML-based fuzzer than can explore to program states more effectively with only a limited number of input samples.



% ~\rahul{V3:~}
% Recently, Machine learning (ML) techniques have been shown to significantly improve the performance of graybox fuzzers~\cite{Saavedra2019, she2018neuzz, Rajpal2017}. ML-based fuzzers use a machine learning model to \textit{learn a mapping} between the input and the corresponding program state. Since the program state is complex with a number interacting variables,  This is typically done by training the ML-models to predict the \ec of the inputs. Then, using a specialized algorithm, they identify promising regions in the input to mutate so as to maximize the coverage of the program's state-space~\cite{she2018neuzz, godefroid2017learn, Rajpal2017, Saavedra2019}. % The quality of the underlying ML-technique dictates the effectiveness of the ML-based fuzzers. 

% Since the program state is complex with a large number interacting variables,
% it is typical to measure the program states using code coverage measures such as \ec. 




% Some previous research have alluded to the possible benefits of incorporating additional coverage code measures~\cite{Wang2019}. \tool is first to successfully develop a generic ML-based greybox fuzzing framework that can.

% \rahul{Version II}~{\color{black!60}~The key challenge with existing ML-based fuzzers is that underlying ML-model is not generalizable, \ie, it cannot extrapolate the observations from already explored program states to reason about previously unseen regions of the program's state-space. This makes it difficult to guide the ML-based fuzzers towards reaching these unseen regions. Typically, to train a generalizable ML-models, we require a sufficiently large number of interesting input samples (\ie, inputs that trigger a wide variety of unique program behaviors). It is often difficult, if not prohibitively expensive, to collect enough interesting inputs since these inputs are \textit{sparsely} distributed over a high-dimensional space. For example, generating about 1000 samples takes about 5 hours~\cite{zalewski2017american}.
% Therefore, the goal of this paper is to develop a generalizable ML-based fuzzer than can operate effectively even when the number available input samples are limited.}

% The key challenge with existing ML-based fuzzers is that underlying ML-model is not generalizable, \ie, it cannot extrapolate the observations from already explored program states to reason about previously unseen regions of the program's state-space. This makes it difficult to guide the ML-based fuzzers towards reaching these unseen regions~\cite{she2018neuzz,Saavedra2019}. Typically, to train a generalized ML-models fail to generalize when the number of interesting inputs (\ie, inputs that invoke new program states) provided to it is inadequate. It is often difficult, if not prohibitively expensive, to collect enough interesting inputs because they are \textit{sparsely} distributed over a high-dimensional space. Therefore, the goal of this paper is to develop a generalizable ML-based fuzzer than can operate effectively even when the number available input samples are limited.   

% The key challenge with existing ML-based fuzzers is that underlying ML-model is not generalizable, \ie, it cannot extrapolate the observations from already explored program states to reason about previously unseen regions of the program's state-space. This makes it difficult to guide the ML-based fuzzers towards reaching these unseen regions. Typically, to train a generalize ML-models fail to generalize when the number of interesting inputs (\ie, inputs that invoke new program states) provided to it is inadequate. It is often difficult, if not prohibitively expensive, to collect enough interesting inputs because they are \textit{sparsely} distributed over a high-dimensional space. Therefore, the goal of this paper is to develop a generalizable ML-based fuzzer than can operate effectively even when the number available input samples are limited.   




% AN alternative to increasing the sample size is to reuse the existing sample to learn how they \texttt{perform??} on alternative measure of \texttt{code coverage???} 
%However, current ML-based greybox fuzzers tend to stuck in long sequences of unfruitful mutations, failing to generate inputs that explore novel regions of the target program~\cite{chen2018angora, she2018neuzz, she2019neutaint}.

% The key challenge in designing an ML-based fuzzers is to answer, . %faced by current ML-based fuzzers is that the accuracy of the underlying ML-model directly affects the efficiency of the ML-based fuzzers. Training accurate ML-models requires a sufficiently large number of interesting input samples (\ie, inputs that trigger a wide variety of unique program behaviors). 
%

% Ideally, ML-based fuzzers would be required to exhaustively sample all the variables in the program's state-space. However, this is prohibitively expensive, since the program's state-space is complex and very large.

% \bi
% \item[\textit{a)}] \textit{Insufficiency of Training data.} The accuracy of the underlying ML-model directly affects the efficiency of the ML-based fuzzers. Training accurate ML-models requires a sufficiently large number of interesting input samples (\ie, inputs that trigger a wide variety of unique program behaviors). However, generating a large number of interesting input samples is very hard because the input space is high-dimensional and inputs triggering interesting program behaviors are sparsely distributed over the input space~\cite{lemieux2017fairfuzz, she2018neuzz, she2019neutaint}.
% \item[\textit{b)}] \textit{Lack of generalizability.} With limited training data, ML-models tend to suffer from \textit{over-fitting}. As a result, current ML-models fail to extend generalization from already seen regions to the previously unseen regions of the program. This makes it difficult to guide the ML-based fuzzers towards reaching these unseen regions. % Furthermore, for every new program, we may have to generate high quality data from scratch. Gathering such data can be quite expensive. 
% \ei
% 

% To address the limitations of ML-based fuzzers, we propose a novel fuzzing framework called \tool that is based on multi-task neural networks. Multi-task Neural Networks (hereafter, \textit{MTNN}) learn to model the relationship between the input and the program state-space in terms of different tasks where Each task represents information about a certain aspect of the program state. The MTNN is trained to predict the response elicited by the input with respect to each of the \textit{tasks} simultaneously~\cite{caruana1996algorithms, caruana1997multitask}. The MTNN offers a single compact representation of the program's state-space 

% \textit{MTNN} have been shown to 
% \begin{inparaenum}[(i)]
%     \item alleviate the data insufficiency problem~\cite{caruana1997multitask, zhang2017survey, Binge2017}, and 
%     \item prevent overfitting by learning a general representation of the input that satisfies all the tasks~\cite{caruana1997multitask,baxter2000model}.
% \end{inparaenum}



%% Add compact embedding here--
% To address the limitations of ML-based fuzzers, we propose a novel fuzzing framework called \tool that is based on multi-task neural networks. The multi-task neural networks (hereafter, \textit{MTNN}) learns to model the relationship between the input and the program state-space.
% The key intuition of \tool is that an MTNN can be used to reduce the high dimensional input space into a low dimensional \textit{compact embedding} that captures the program state-space. 
% This is achieved by training the MTNN to predict for \textit{multiple tasks} (\eg, by predicting various coverage measures~\cite{chen2018angora, mcmaster2008call, Wang2019Be, McMinn2004, arcuri2010does, mcminn2011search, pachauri2013automated} invoked by the input). Each task models a different aspect of the program behavior exercised by a given input. The resulting MTNN generates a single \textit{compact embedding} that captures the program's state-space. By computing the gradient over compact embedding with respect to the inputs we can model the \textit{most pertinent input byte-locations} that apply to all tasks. This information will enable \tool to focus the mutations more on those specific byte-locations.% Consequently, \tool would be able to generate significantly larger high-quality inputs.
% Our results indicate that \tool can significantly outperform the current state-of-the-art ML-based fuzzers. 

% The overview of \tool is shown in \fig{intro_fig}. 
\tool comprises of three stages namely, (i)~multi-task training, (ii)~gradient-guided mutation, and (iii)~incremental learning. In the first stage, we pick a set of inputs from the seed corpus to train an MTNN. The MTNN learns the \textit{program behavior elicited by the input bytes} in terms of three coverage measures (or \textit{tasks}) namely, \ec~\cite{zalewski2017american,she2018neuzz}, \ctx~\cite{chen2018angora,Wang2019}, and \softlabel~\cite{McMinn2004, arcuri2010does, mcminn2011search, pachauri2013automated}. The trained MTNN offers an intermediate compact-embedding. In the second stage, we compute the \textit{gradient} between the compact-embedding layer and the input-layer. The value of the gradient informs the subsequent mutation operation of the most relevant bytes in the input to mutate. In the final stage, we run the newly generated test inputs on the instrumented program and update the seed corpus with the most promising seeds. 

\noindent\textbf{Architecture.}~
The architecture of our MTNN model is specifically designed to faciliate learning a compact-embedding of the program's state-space. It comprises of two groups of layers: 
\begin{itemize}
  \item[\mybullet]\textit{Shared Encoding Layer.}~These comprise of a set of 3 hidden layers (each narrower than its predecessor). These layers are \textit{shared} among all the tasks. The goal of the shared encoding layer is to \textit{distill} the high-dimensional inputs into a \textit{compact-embedding}, \ie, a low-dimensional representation of the input comprising of only the most salient input bytes that matter to all tasks. In essence, this shared encoding represents a neural embedding of the input format.
  \item[\mybullet]\textit{Task specific decoder.}~These consist of a set of decoders (one for each task) that map the shared encoding layer to the output layers specific to each task.    
\end{itemize}


The shared encoding layer offers \textit{a powerful feature extractor} for reducing the complex program state-space into a \textit{low-dimensional compact embedding}. Empirical results demonstrate that fuzzers operating on the compact-embedding are are significantly more effective than those operating on the original program space.

Our architecture offers two key advantages:

\noindent\textbf{Adaptability.}~\tool can be easily adapted to incorporate a diverse set of additional tasks. Theoretical results show that an MTNN can perform just as well when it is extended to include novel tasks~\cite{baxter2000model}. To demonstrate this, we present promising preliminary results with an additional task to assert the validity of newly generated mutants (see RQXX). We make available a replication package\footnote{Replication Package: \href{https://blinded.for.review}{https://blinded.for.review}} in order to enable adding new tasks. These tasks may fall under any category of learning tasks, \eg, supervised (classification/regression), unsupervised, reinforcement learning, etc.

%This paper incorporates 3 coverage metrics--- \ec, \ctx, and \softlabel. 
% These were chosen since they were shown previously to independently have the most impact on improving fuzzing~\cite{zalewski2017american,she2018neuzz,chen2018angora,Wang2019}. 


\noindent\textbf{Transferability.}~\tool can be used to \textit{transfer} the learned compact-embedding among programs that parse similar file formats. In essence, \tool that is modeled on one program can be used to efficiently fuzz a different program that shares the same input, \eg, the compact-embedding learned with \tool for one pdf parser may be transferred to other pdf parsers. Our results (RQ4) show that such transfer is quite effective and it mitigates the need to generate high quality data from scratch for new programs which can be quite expensive.

We evaluate \tool on 9 real world programs against 6 state-of-the-art fuzzers. \tool covers at least a 1000 more edges on 5 programs and several 100 more on the rest. \tool also finds 15 previously unseen real-world bugs (see RQ1). When compared to learning each task individually, \tool offers significantly more edge coverage (see RQ2). Lastly, our results from transfer learning show that the compact-embedding of \tool can be transferred within parsers for pdf, xml, and elf binaries. \tool \textit{offers similar edge coverage} compared to fuzzing with bespoke models that were built from scratch (see RQ3).

Overall, our paper makes the following key contributions:
\bi

\item We present a novel fuzzing framework based on multi-task neural networks called \tool that offers a compact embedding of an otherwise complex and high-dimensional input space.

\item We offer empirical results demonstrating that \tool which operates on the compact-embedding space is significantly more effective than current state-of-the-art fuzzers. 

\item We offer promising results on the transferability of \tool. Results demonstrate that transferred \tool offers competing coverage to non-transfer models. {\texttt{Need Numbers}}.
 
\item We offer an open-source replication package to reproduce and extend \tool at \href{https://blinded.for.review}{https://blinded.for.review}.

\ei


% \squishlist
% \item 
% We propose \tool, a Multi-Task Netural Network adaptive framework that can automatically find good mutation parameter values by learning from diverse information sources (\eg  branch distances~\cite{arcuri2010does}, encoding of new-edges, rare-edges, \etc) collected from program executions. To achieve this, we formulate the problem of finding optimal parameter values as gradient-guided optimization which \tool solves to automatically find the optimal mutation parameters at any given step the of the fuzzing operation.

% \item
% We present a new parameterized mutation scheme that can leverage information about the probability of different control-flow edges being taken in a program for different inputs to distribute the mutations across the input space so that they maximize the chances of new edge discovery. 

% \item
% Our experiments demonstrate that \tool outperforms current state-of-the-art methods in discovering more new-edges (RQ1), rare-edges (RQ3), and novel seeds (RQ2) (see~\tion{rqs}). Our experiments further show that our framework can leverage different types of information sources like a branch-distance~\cite{arcuri2010does} based soft-labeling scheme and a customized loss function to prioritize mutations that might result in exploring rare edges according to our ML model. 

% \item
% We demonstrate that our ML models mapping from program input to the control-flow edge probability space offer a high degree of generalizibility. \tool modeled using inputs from one program can be used to efficiently update the parameters of a similar program (e.g., a program that parses the same file format as the first one). We believe that such sharing of models can potentially result in drastic reduction of fuzzing overhead for programs with share functionalities.
% \squishend

The rest of this paper is structured as follows. \tion{} summarizes . \tion{our_method} describes \tool in detail. 
In \tion{implementation}, we present the instrumentation details followed by answers to our research questions in \tion{rqs}. In \tion{threats}, we list some of the threat to validity of our findings. Other related work in this area are discussed in \tion{related} and conclusion in \tion{conclusion}.


% \subsection{Research Questions}

% \rqone The first RQ assesses the number of bugs found by \tool and the improvements in edge-coverage compared to other state-of-the-art graybox fuzzers. We note that:


% \rqtwo In this RQ, ensembles of each individual task is compared to a multi-task neural-network model. Also, each task (\ie, coverage measures) within \tool is disassembled to study their effect on the overall performance. We show that:

% \begin{goal} 
% Fuzzing with an ensembles of each task is more computationally burdensome than multi-task models (up to 3$\times$). Ensembles also offer inferior edge coverage compared a multi-task models (up to 1000 few edges covered). 
% \end{goal}

% \rqthree We evaluate the transferability of \tool across different programs that share similar input formats. We show that: 

% \begin{goal}
% \tool modeled on one program can be \textit{transferred} to a different program operating on the same input format, \ie, \tool can be transferred within parsers for pdf, xml, and elf binaries. \tool \textit{offers similar edge coverage} compared to fuzzing with bespoke models built from scratch.
% \end{goal}




% Consequently, current graybox fuzzers tend to stuck in long sequences of unfruitful mutations, failing to generate inputs that explore novel regions of the target program~\cite{chen2018angora, she2018neuzz, she2019neutaint}.

% It has been argued that, in order to explore the input space better, one may have to look beyond traditional coverage measures such as \ec so as to model aspects of program behavior that are not fully conveyed by \ec~\cite{chen2018angora, Wang2019Be, GREYONE} . For instance, while \ec measures the number of unique control-flow edges taken by a test-input, it fails to distinguish between inputs that invoke the same control-flow edges but via new internal states (for instance through completely different \textit{call-stack})~\cite{chen2018angora, mcmaster2008call, Wang2019Be}. Such information may be obtained using additional coverage measures such as \ctx~\cite{chen2018angora, Wang2019Be}. Similarly, in order guide fuzzing towards reaching specific branches in the \cfg, it may make sense to use a measure of proximity such as \textit{approach level}~\cite{McMinn2004, arcuri2010does, mcminn2011search, pachauri2013automated}, so as to calculate how close a generated input was to triggering specific control-flow branches. 

% In a recent study, Wang \etal~\cite{Wang2019Be} report that there is no universal best coverage measure. Instead, they demonstrate that it is best to incorporate a combination of coverage measures in order to maximize the fuzzing efficiency. However, the efforts to incorporate these additional coverage metrics by the state-of-the-art fuzzers currently rely on arduous manual instrumentation atop existing fuzzers such as AFL~\cite{zalewski2017american}. As a consequence, current coverage-guide graybox fuzzers lack \textit{extensibility}, \ie, it is difficult to incorporate additional sources of coverage information in the future without significant additional instrumentation. Additionally, it is also hard to determine how generalizable these instrumentations are across programs that exhibit different behavior. 


% \begin{itemize}
%   \item Firstly, t
%   \item Secondly, current ML-based fuzzers can only model the relationship between inputs and the corresponding \ec. It is not clear how to exploit other sources of coverage information such as \ctx or \softlabel. While it may theoretically be possible to build different models for different information sources and combine their results, finding good parameter values, optimizing them, and managing such ensemble models is intractable in practice. Further, training and inference with ensemble models imposes a significant computational overhead slowing down the overall fuzzing process, as shall be shown by this article.
% \end{itemize}

% To overcome these issues, we seek a fuzzer that can:
% \begin{inparaenum}[(i)]
%     \item~Mitigate the problems presented by a sparse and a high-dimensional input space; and 
%     \item~Leverage \textit{multiple} sources of coverage information.  
% \end{inparaenum} 

% To this end, we propose \tool--- a generic fuzzing framework that can learn from several sources of information using a Multi-task Neural Network (hereafter, MTNN). \fig{intro_fig} shows the overview of \tool comprising main three stages that are repeated until the budget allocated for fuzzing is exhausted. In Stage 1, we pick a set of inputs from the seed corpus to train a MTNN. The MTNN learns the \textit{program behavior elicited by the input bytes} in terms of three coverage measures (or \textit{tasks}) namely, \ec, \ctx, and \softlabel. The MTNN architecture used in \tool comprises of two groups of layers: 
% \begin{inparaenum}[(a)]
%   \item A set of hidden layers, \textit{shared} among all the tasks, that encodes the high-dimensional inputs into a compact joint-embedding, \ie, a low-dimensional representation of the input comprising of the most salient input bytes that matter to all tasks; and
%   \item Task specific decoding layers, that learn the relationship between the joint-embedding and the individual tasks.    
% \end{inparaenum}
% Next, in Stage 2, we compute the \textit{gradient} between the joint-embedding layer and the input. The value of the gradient informs the subsequent mutation operation of the most relevant bytes in the input to mutate. Finally, in Stage 3, we run the newly generated test inputs on the instrumented program. We update the seed corpus with the most promising seeds.     

% In summary, this paper makes the following contributions:

% \be
% \item \textit{Extensibility:}~A novel fuzzing framework based on multi-task neural networks called \tool that can incorporate diverse information sources. This paper incorporates 3 coverage metrics--- \ec, and \ctx, \softlabel. Additional metrics may be added using our replication package\footnote{\href{https://blinded.for.review}{https://blinded.for.review}}.
% \item \textit{Compactibility:}~\tool offers a powerful feature extractor for reducing sparse and high-dimensional input in a compact low-dimensional embedding. Empirical results demonstrating that fuzzers operating on the compacted embedding space are more effective.
% \item \textit{Transferability:}~
% \ee

% 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Introduction}


% Coverage guided graybox fuzzing is a widely used technique for detecting bugs and security vulnerabilities in real-world software systems~\cite{zalewski2017american, cgc, zalewski2017american, manes2018fuzzing, wang2019superion,Nilizadeh2019,You2019SLFFW,lemieux2017fairfuzz,she2018neuzz, godefroid2008, arya2012fuzzing, evans2011fuzzing, moroz2016guided}. The key idea behind a fuzzer is to execute the target program on a large number of automatically generated test inputs and monitor the executions for buggy behaviors. However, as the input space of a program is typically very large, unguided test input generation is not effective at finding bugs.

% Most popular fuzzers (especially the graybox ones) use 
% some form of evolutionary search strategy to generate new inputs by \textit{mutating} a set of \textit{seed inputs} and retain only the promising inputs for further mutations that exercise new program behavior~\cite{zalewski2017american, wang2019superion,Nilizadeh2019,You2019SLFFW, wei2018singularity, steelix, godefroid2017learn,lemieux2017fairfuzz,jiang2018contractfuzzer}. 

% However, with time, the evolutionary fuzzers tend to become 
% increasingly less effective at reaching new code locations. 
% Although much research effort has been spent on designing different mutation strategies to increase edge coverage, the success not only varies widely across different test programs but also change drastically depending on the actual input values being mutated.

% Recently, Machine learning (ML) techniques have been shown to significantly improve the performance of graybox fuzzers \cite{Saavedra2019, she2018neuzz,Rajpal2017}.  These, ML-based fuzzers attempt to model a particular information source (\ie, input format) with respect to its coverage behavior. Then, using a specialized algorithm, they identify promising regions in the input to mutate so as to maximize code coverage~\cite{she2018neuzz,godefroid2017learn,Saavedra2019,Rajpal2017}. However, these ML-based fuzzers face two critical challenges that limit their overall efficiency: 
% % \bi
% % \item[\textit{a)}] \textit{Insufficiency of Training data.} The accuracy of the underlying ML-model directly determines the efficiency of the ML-based fuzzers. Training accurate ML-models requires a sufficiently large number of interesting input samples (\ie, inputs that trigger a wide variety of unique program behaviors). However, generating a large number of interesting input samples is very hard because the input space is high-dimensional and inputs triggering interesting program behaviors are sparsely distributed over the input space~\cite{lemieux2017fairfuzz, she2018neuzz, she2019neutaint}.
% % \item[\textit{b)}] \textit{Lack of generalizability.} With limited training data, ML-models tend to suffer from \textit{over-fitting}. As a result, current ML-models fail to extend generalization from already seen regions to the previously unseen regions of the program. This makes it difficult to guide the ML-based fuzzers towards reaching these unseen regions. % Furthermore, for every new program, we may have to generate high quality data from scratch. Gathering such data can be quite expensive. 
% % \ei

% % To address the limitations of ML-based fuzzers, we propose a novel fuzzing framework called \tool based on multi-task deep neural networks. Multi-task Neural Networks (hereafter, \textit{MTNN}) learn to model the relationship between the input and several tasks simultaneously~\cite{caruana1996algorithms, caruana1997multitask}. \textit{MTNN} have been shown to 
% % \begin{inparaenum}[(i)]
% %     \item alleviate the data insufficiency problem~\cite{caruana1997multitask, zhang2017survey, Binge2017}, and 
% %     \item prevent overfitting by learning a general representation of the input that satisfies all the tasks~\cite{caruana1997multitask,baxter2000model}.
% % \end{inparaenum}
% %Our results indicate that \tool can significantly outperform the current state-of-the-art ML-based fuzzers. 

% % \textbf{Compact Embedding.}~

% The key intuition of \tool is that an MTNN can be trained to learn the relationship between the input and various tasks (\eg, coverage measures~\cite{chen2018angora, mcmaster2008call, Wang2019Be, McMinn2004, arcuri2010does, mcminn2011search, pachauri2013automated}) so as to model different aspects of program behavior exercised by the input. This would enable MTNN to model the most pertinent input byte-locations that apply to all tasks. Using this information, \tool can focus the mutations more on those specific byte-locations.% Consequently, \tool would be able to generate significantly larger high-quality inputs.

% \input{tex/fig-1.tex}

% The overview of \tool is shown in \fig{intro_fig}. It comprises of three stages that are repeated iteratively. In Stage 1, we pick a set of inputs from the seed corpus to train an MTNN. The MTNN learns the \textit{program behavior elicited by the input bytes} in terms of three coverage measures (or \textit{tasks}) namely, \ec~\cite{zalewski2017american,she2018neuzz}, \ctx~\cite{chen2018angora,Wang2019}, and \softlabel~\cite{McMinn2004, arcuri2010does, mcminn2011search, pachauri2013automated}. Next, in Stage 2, we compute the \textit{gradient} between the joint-embedding layer and the input-layer. The value of the gradient informs the subsequent mutation operation of the most relevant bytes in the input to mutate. Finally, in Stage 3, we run the newly generated test inputs on the instrumented program and update the seed corpus with the most promising seeds. 

% \tool offers numerous benefits over current ML-based fuzzers:\\
% \noindent\textbf{Compact Embedding.}~
% The architecture of our MTNN model comprises of two groups of layers: 
% \begin{itemize}
%   \item\textit{Shared Encoding Layer.}~These comprise of a set of 3 hidden layers (each narrower than its predecessor). These layers are \textit{shared} among all the tasks. The goal of the shared encoding layer is to \textit{distill} the high-dimensional inputs into a \textit{compact joint-embedding}, \ie, a low-dimensional representation of the input comprising of only the most salient input bytes that matter to all tasks. In essence, this shared encoding represents a neural embedding of the input format.
%   \item\textit{Task specific decoder.}~These consist of a set of decoders (one for each task) that map the shared encoding layer to the output layers specific to each task.    
% \end{itemize}

% The shared encoding layer offers \textit{a powerful feature extractor} for reducing sparse and high-dimensional input into a \textit{compact low-dimensional embedding}. Empirical results demonstrate that fuzzers operating on the low-dimensional joint-embedding are are more effective than those operating on the high-dimensional input layer.\\
% \noindent\textbf{Adaptability.}~\tool can be easily adapted to incorporate a diverse set of additional information sources (as new tasks). Theoretical results show that an MTNN can perform just as well when it is extended to include novel tasks~\cite{baxter2000model}. This paper incorporates 3 coverage metrics--- \ec, \ctx, and \softlabel. These were chosen since they were shown previously to independently have the most impact on improving fuzzing~\cite{zalewski2017american,she2018neuzz,chen2018angora,Wang2019}. Additional tasks may be added using our replication package\footnote{Replication Package: \href{https://blinded.for.review}{https://blinded.for.review}}. These tasks may fall under any category of learning tasks, \eg, supervised (classification/regression), unsupervised, reinforcement learning, etc.\\
% \noindent\textbf{Transferability.}~The joint-embedding layer obtained from~\tool learns a representation  of the input format. 
% This representation can be transferred to programs that parse similar file formats. In essence, \tool that is modeled on one program can be used to efficiently fuzz a different program with very little overhead. This mitigates the need to generate high quality data from scratch for new programs which can be quite expensive.

% The rest of this paper is structured as follows. \tion{} summarizes . \tion{our_method} describes \tool in detail. 
% In \tion{implementation}, we present the instrumentation details followed by answers to our research questions in \tion{rqs}. In \tion{threats}, we list some of the threat to validity of our findings. Other related work in this area are discussed in \tion{related} and conclusion in \tion{conclusion}.


% \subsection{Research Questions}
% We evaluate \tool on 9 real world programs against 6 state-of-the-art fuzzers. The findings of this paper are summarized below as answers to three key research questions. 

% \rqone The first RQ assesses the number of bugs found by \tool and the improvements in edge-coverage compared to other state-of-the-art graybox fuzzers. We note that:

% \begin{goal} 
% \tool covers at least a 1000 more edges on 5 programs and several 100 more on the rest. \tool also finds 15 previously unseen real-world bugs. 
% \end{goal}

% \rqtwo In this RQ, ensembles of each individual task is compared to a multi-task neural-network model. Also, each task (\ie, coverage measures) within \tool is disassembled to study their effect on the overall performance. We show that:

% \begin{goal} 
% Fuzzing with an ensembles of each task is more computationally burdensome than multi-task models (up to 3$\times$). Ensembles also offer inferior edge coverage compared a multi-task models (up to 1000 few edges covered). 
% \end{goal}

% \rqthree We evaluate the transferability of \tool across different programs that share similar input formats. We show that: 

% \begin{goal}
% \tool modeled on one program can be \textit{transferred} to a different program operating on the same input format, \ie, \tool can be transferred within parsers for pdf, xml, and elf binaries. \tool \textit{offers similar edge coverage} compared to fuzzing with bespoke models built from scratch.
% \end{goal}




% % Consequently, current graybox fuzzers tend to stuck in long sequences of unfruitful mutations, failing to generate inputs that explore novel regions of the target program~\cite{chen2018angora, she2018neuzz, she2019neutaint}.

% % It has been argued that, in order to explore the input space better, one may have to look beyond traditional coverage measures such as \ec so as to model aspects of program behavior that are not fully conveyed by \ec~\cite{chen2018angora, Wang2019Be, GREYONE} . For instance, while \ec measures the number of unique control-flow edges taken by a test-input, it fails to distinguish between inputs that invoke the same control-flow edges but via new internal states (for instance through completely different \textit{call-stack})~\cite{chen2018angora, mcmaster2008call, Wang2019Be}. Such information may be obtained using additional coverage measures such as \ctx~\cite{chen2018angora, Wang2019Be}. Similarly, in order guide fuzzing towards reaching specific branches in the \cfg, it may make sense to use a measure of proximity such as \textit{approach level}~\cite{McMinn2004, arcuri2010does, mcminn2011search, pachauri2013automated}, so as to calculate how close a generated input was to triggering specific control-flow branches. 

% % In a recent study, Wang \etal~\cite{Wang2019Be} report that there is no universal best coverage measure. Instead, they demonstrate that it is best to incorporate a combination of coverage measures in order to maximize the fuzzing efficiency. However, the efforts to incorporate these additional coverage metrics by the state-of-the-art fuzzers currently rely on arduous manual instrumentation atop existing fuzzers such as AFL~\cite{zalewski2017american}. As a consequence, current coverage-guide graybox fuzzers lack \textit{extensibility}, \ie, it is difficult to incorporate additional sources of coverage information in the future without significant additional instrumentation. Additionally, it is also hard to determine how generalizable these instrumentations are across programs that exhibit different behavior. 


% % \begin{itemize}
% %   \item Firstly, t
% %   \item Secondly, current ML-based fuzzers can only model the relationship between inputs and the corresponding \ec. It is not clear how to exploit other sources of coverage information such as \ctx or \softlabel. While it may theoretically be possible to build different models for different information sources and combine their results, finding good parameter values, optimizing them, and managing such ensemble models is intractable in practice. Further, training and inference with ensemble models imposes a significant computational overhead slowing down the overall fuzzing process, as shall be shown by this article.
% % \end{itemize}

% % To overcome these issues, we seek a fuzzer that can:
% % \begin{inparaenum}[(i)]
% %     \item~Mitigate the problems presented by a sparse and a high-dimensional input space; and 
% %     \item~Leverage \textit{multiple} sources of coverage information.  
% % \end{inparaenum} 

% % To this end, we propose \tool--- a generic fuzzing framework that can learn from several sources of information using a Multi-task Neural Network (hereafter, MTNN). \fig{intro_fig} shows the overview of \tool comprising main three stages that are repeated until the budget allocated for fuzzing is exhausted. In Stage 1, we pick a set of inputs from the seed corpus to train a MTNN. The MTNN learns the \textit{program behavior elicited by the input bytes} in terms of three coverage measures (or \textit{tasks}) namely, \ec, \ctx, and \softlabel. The MTNN architecture used in \tool comprises of two groups of layers: 
% % \begin{inparaenum}[(a)]
% %   \item A set of hidden layers, \textit{shared} among all the tasks, that encodes the high-dimensional inputs into a compact joint-embedding, \ie, a low-dimensional representation of the input comprising of the most salient input bytes that matter to all tasks; and
% %   \item Task specific decoding layers, that learn the relationship between the joint-embedding and the individual tasks.    
% % \end{inparaenum}
% % Next, in Stage 2, we compute the \textit{gradient} between the joint-embedding layer and the input. The value of the gradient informs the subsequent mutation operation of the most relevant bytes in the input to mutate. Finally, in Stage 3, we run the newly generated test inputs on the instrumented program. We update the seed corpus with the most promising seeds.     

% % In summary, this paper makes the following contributions:

% % \be
% % \item \textit{Extensibility:}~A novel fuzzing framework based on multi-task neural networks called \tool that can incorporate diverse information sources. This paper incorporates 3 coverage metrics--- \ec, and \ctx, \softlabel. Additional metrics may be added using our replication package\footnote{\href{https://blinded.for.review}{https://blinded.for.review}}.
% % \item \textit{Compactibility:}~\tool offers a powerful feature extractor for reducing sparse and high-dimensional input in a compact low-dimensional embedding. Empirical results demonstrating that fuzzers operating on the compacted embedding space are more effective.
% % \item \textit{Transferability:}~
% % \ee

% % 

==> body/2_formalization.tex <==
\section{Background}% and Motivation}
\label{sect:background}

% We briefly review the challenges with current coverage guided \gf~\tion{cov_gf}. Next we discuss the key components of our fuzzing framework--- Multi-task Networks Networks (\tion{multitask_learning}), compact embedding (\tion{compact}), and gradient-guided mutation (\tion{gradients}).  

% % Opening para: On ML based graybox fuzzing
% \subsection{Coverage-Guided Greybox Fuzzing}
% \label{sect:cov_gf}

%\begin{comment}


% The goal of \gf is to generate inputs that can maximize the number of program states that is explored. Formally, if $\mathcal{X}$ is the space of all possible inputs, then \gf tries to mutate exisiting inputs $\mathrm{x}\in\mathcal{X}$ to generate \textit{promising} new inputs that exercises as many new program states as possible within a given budget. The program state is usually measured using code-coverage metrics such as \ec.

% % In order to find these interesting inputs, a \gf attempts to maximize the \ec by \textit{mutating} inputs using the following three main steps: 
% % \begin{inparaenum}[a)]
% %     \item Finding\textit{ which inputs} $\mathrm{x}\in\mathcal{X}$ to mutate; 
% %     \item Finding \textit{which byte locations} in the inputs should be mutated; and 
% %     \item Finding \textit{how to mutate} those byte location.
% % \end{inparaenum}

% In order to effectively mutate an input, identifying the most important byte locations in the input (also known as \textit{hotbytes}) is critical~\cite{taintscope}. Much research effort has been dedicated toward finding these \textit{hotbytes}~\cite{lemieux2017fairfuzz, You2019ProFuzzerOI, You2019SLFFW, vuzzer, steelix, chen2018angora, bohme2017coverage, she2018neuzz,she2019neutaint}. Among these, Machine learning (ML) based fuzzers have shown the most promise in offering the best approximations of the distribution of hot-bytes~\cite{she2018neuzz,godefroid2017learn}. 

% ML-based fuzzers operate by predicting how input bytes affect coverage measures such as \ec. In order to accuarately make these predictions, ML-based fuzzers require a large number of training examples. However, the input space $\mathcal{X}$ is typically \textit{very sparse}, \ie, the inputs $\mathrm{x}\in\mathcal{X}$ are high-dimensional and inputs invoking rare program behavior are not very prevelant. As a result, obtaining sufficient training examples can be costly, if not prohibitively expensive. Hence, the hot-byte approximations of ML-based fuzzers tend to be localized to only what can be infered from the available training inputs. The hot-byte approximations of ML-based \textit{do not generalize} well across different regions of the same program, \ie, the approximation of hot-byte distribution does not reflect unseen regions of the program space. This limits how effectively ML-based fuzzers can explore deeper regions of the program space.  

% % In order to effectively mutate an input, indentifying the most important byte locations in the input (also known as \textit{hotbytes}) is critical~\cite{taintscope}. Much research effort has been dedicated toward finding these \textit{hotbytes}. For instance, FairFuzz~\cite{lemieux2017fairfuzz}, ProFuzz~\cite{You2019ProFuzzerOI} and SLF~\cite{You2019SLFFW} modify the mutation strategy of AFL by using aggregate statistics to identify which input regions are most likely to trigger ``rare-branches''. In contrast, Vuzzer~\cite{vuzzer}, Steelix~\cite{steelix} and Angora~\cite{chen2018angora} use dynamic taint analysis to identify ``hot'' regions and focus on mutating them. However, the approaches based on aggregated statistics on edge coverage behavior~\cite{bohme2017coverage,lemieux2017fairfuzz} misses many local input-specific variations in edge coverage, while taint-tracking based strategies are known to suffer from high false positives/false negatives~\cite{she2018neuzz,she2019neutaint}. 

% % %They may not generalize well across different programs or even across different regions of the same programs.

% % Machine learning-based fuzzers have shown that they can approximate the hot-byte locations more effectively than existing methods. They do so by predicting how input bytes affect coverage measures such as \ec. In order to accuarately make these predictions, ML-based fuzzers would require a large number of training examples. However, obtaining sufficient training examples can be costly, if not prohibitively expensive. When adequate number of training examples are not available, the hot-byte approximations of ML-based fuzzers tend to be localized to what can be infered from the available training inputs. As a result, their hot-byte approximations do not generalize well across different regions of the same programs, \ie, the approximation of hot-byte distribution does not reflect the unseen regions of the program space.  

% % Since obtaining sufficient number of inputs to train an ML-based fuzzer is hard, 
% This paper makes a case for reusing existing inputs instead of gathering more input samples. For the existing inputs, we may measure additional aspects of program behavior that are not fully conveyed by \ec alone~\cite{chen2018angora, Wang2019Be, GREYONE}. Note that, some preliminary evidence has alluded to the possible benefits of using additional information sources such as \ctx~\cite{Wang2019Be, chen2018angora} and \softlabel~\cite{McMinn2004, arcuri2010does, mcminn2011search, pachauri2013automated}. However, how best to incorporate these additional information sources for fuzzing is still an open problem that this paper attempts to address. 

% We develop a novel fuzzing framework using Multi-task Neural Networks to incorporate these additional information sources. We use to notion of ``tasks'' to model the following three information sources: 
% \begin{inparaenum}[(i)]
% \item \ec: to measure the number of unique control-flow edges taken by a test-input~\cite{zalewski2017american} (see \tion{ec}); %: One or two lines about edge coverage. Ref. to the section for detail.
% \item \ctx: to distinguish between inputs that invoke the same control-flow edges but via new internal states~\cite{chen2018angora,Wang2019Be} (see \tion{ctx}); and  %: One or two lines about call context. Ref. to the section for detail.
% \item \softlabel: to measure the proximity of a generated input to triggering specific control-flow edges~\cite{McMinn2004, arcuri2010does, mcminn2011search, pachauri2013automated} (see \tion{sl}). %: One or two lines about approach. Ref. to the section for detail.
% \end{inparaenum}


% The rest of this section discusses Multi-task Neural Networks in detail demonstrating how, with no additional training inputs, it can: (a) prevent overfitting (enabling generalization) and (b) provide a compact embedding (mitigating the effect of sparse input space). In \tion{gradients}, we discuss our gradient-guided hotbyte discovery and mutation strategy.

%\end{comment}



\subsection{Multi-task Neural Networks}
\label{sect:multitask_learning}
Multi-task neural networks (or MTNN for short) are prevelantly used in several domains such as machine learning~\cite{argyriou2008convex, gong2014efficient}, natural language processing~\cite{collobert2008unified, Binge2017}, and computer vision~\cite{standley2019tasks} communities. MTNN draws inspiration from human learning where it is common for one to learn multiple related tasks more easily than it is to learn them in isolation.%, \eg, \{\textsc{a good example here with citation}\}.

The key intuition behind MTNN is that it is useful for multiple learning tasks to be learned jointly so that each task can leverage the knowledge available in the other tasks~\cite{caruana1996algorithms,caruana1997multitask}. Each individual task may fall under any machine learning paradigm, \eg, supervised learning (classification/regression)~\cite{yin2017multi, mtl_regression_1}, unsupervised learning~\cite{mtl_unsuper}, etc. It is most beneficial, when all the tasks, or at least a subset of the tasks, are related to each other~\cite{standley2019tasks,zamir2018taskonomy}. 

More formally, the objective of a multi-task neural network may be defined as follows:
\begin{definition}
    Given a set of training instances $\mathrm{X}=\{x_1, x_2, ..., x_n\}$ and $\mathit{m}$ tasks $\mathcal{T}=\{\tau_1, \tau_2, ..., \tau_m\}$, where all (or a subset) of the $\mathit{m}$ tasks are related, a \textit{multi-task neural network} aims to learn a mapping function $f:X\rightarrow\mathcal{T}$ that maps the input $\mathrm{X}$ to all the m tasks in $\mathcal{T}$.    
\end{definition}

The architecture of the MTNN used in this paper comprises of two groups of layers. First, a set of initial layers that are shared among all the tasks. Next, we have several individual task-specific layers output layers. This architecture, also known as the \textit{hard parameter sharing} model~\cite{caruana1997multitask}, is most the widely used approach to MTNN\footnote{For other modalities of MTNN, we guide the interested readers to \cite{zhang2017survey, ruder2017overview}}~\cite{kokkinos2017ubernet,standley2019tasks,ruder2017overview}. The following remarks may be made regarding the two sets of layers:
\be
\item \textit{Shared initial layers}:~The goal of the shared initial layers is to \textit{generate a common embedding} that may be shared by all the tasks. This enables the MTNN to \textit{find a representation} that captures information \textit{common} to all tasks. %thereby reducing the chance of the model overfitting to one task. 
\item \textit{Task specific layers}:~The goal of the task specific layers is to generate predictions for each individual task using the encoding offered by the shared initial layers.   
\ee

\noindent\textbf{Training MTNN.} The training of MTNN is formulated as under a supervised learning paradigm since it is most relevant to this work. Under this setting, we assume that we have access to a training dataset $\mathcal{D}$ , such that $\mathcal{D}=\{\mathrm{X}, \mathrm{Y}^{\tau_1}, \mathrm{Y}^{\tau_2}, ..., \mathrm{Y}^{\tau_m}\}$ where $\mathrm{X}=\{x_1, x_2, ..., x_n\}$ is the training set consisting of $\mathit{n}$ training samples and $\mathrm{Y}^{\tau_i}=\{y^{\tau_i}_1, y^{\tau_i}_2, y^{\tau_i}_3, ...\}$ represents the output labels for the task $\tau_i \in \mathcal{T}$
%\{\tau_1, \tau_2, ..., \tau_m\}$
; here $y^{\tau_i}_j$ represents the $\mathit{j}^\mathit{th}$ label in the $\tau_i^\mathit{th}$ task. We train the MTNN as a regular feed-forward neural network.

\noindent\textbf{Multi-task Loss.}~Training an MTNN is guided by a \textit{multi-task loss function}, denoted by $\mathcal{L}$. Each individual task $\tau_i$ in the set of tasks $\mathcal{T}=\{\tau_1, \tau_2, ..., \tau_m\}$ is associated with a corresponding loss function $\mathcal{L}_i$, \ie, for $\mathit{m}$ tasks, we would have a $\mathit{m}$ corresponding losses. Then, the multi-task loss is computed as the weighted sum of each individual task loss. More formally, 
\begin{equation}
    \label{eq:multitask_loss}
    \mathcal{L}=\sum^{m}_{i=1}\alpha_i\cdot\mathcal{L}_i
\end{equation}   

In the above equation, $\alpha_i$ represents the weight assigned for each individual task. This is a prominent approach to task weighting. It has shown much promise in several diverse applications~\cite{uhrig2016pixel, teichmann2018multinet, liao2016understand}. 

In general, the goal of training an MTNN is to \textit{reduce} the overall loss. In doing so, the shared layer is forced to learn the most more general representation of the input, \ie, a representation that is most applicable to all tasks. 

The shared-layer offers two practical benefits:
\be 
\item It can \textit{maximize generalizability}. Theoretical results have demonstrated that the overall risk of overfitting reduces by an order of $m$ (where $\mathit{m}$ is the number of tasks) compared to single task models~\cite{baxter1997bayesian}. Intuitively, the more tasks an MTNN has to learn concurrently, the more general the required representation has to be so that we capture essence of all the tasks. This would prevent the representation from overfitting to one task. 
\item It can \textit{reduce sparsity}. This arises due the \textit{compactness} of the shared embedding layer. The shared embedding layer usually requires far fewer nodes compared to the input layer to retain the same expressive power of the input.  
\ee

% \input{tex/background_fig_1.tex}
% % 
% % \subsubsection{Benefits over current ML-based fuzzers}~
% % The properties of MTNN listed above are very useful in addressing the challenges with current ML-based fuzzers. 
% % Specifically, 
% % \be
% % \item Current ML based fuzzers only use one information source (\ie, edge coverage) to reason about how an input interacts with the program-states, MTNN can model multiple tasks. Each additional task (\eg, in the form of additional coverage measures) assist MTNN-based fuzzers in reasoning about various aspects of the program-state space. This will allow MTNN
% % \item 
% % 
% \subsection{Compact Embedding}
% \label{sect:compact}

% % \subsection{Identifying Hot-bytes}
% % \label{sect:gradients}

% % The goal of ML-based fuzzers is to effectively identify the byte offsets in the input that needs to be mutated so that we may maximize the overall coverage of the program space~\cite{lemieux2017fairfuzz,chen2018angora,zalewski2017american}. Traditional ML-based methods usually operate on the sparse and high-dimensional input space~\cite{she2018neuzz,rajpal2017not,Saavedra2019}. As a result, their mutations tend not to generalize well to unseen regions of the program space~\cite{she2018neuzz,You2019SLFFW,rajpal2017not}.

% % MTNN offers a useful alternative to address this problem. 

% The compact embedding layer of MTNN is a dense and a feature rich representation of the sparse input space (see \fig{bg_fig_1}). It captures all the semantically meaningful factors in the inputs with a substantially lower number of dimensions, \ie, it contains all the information present in the inputs  
% but in a compact and an interpretable manner~\cite{chen2016, kulkarni2015, Bengio13} while discarding other spurious information~\cite{kumar2017variational}.

% Formally, we can represent the input as a byte vector $xb=\{xb^1, xb^2, ..., xb^q\}\in\mathrm{\left[0, 255\right]^n}$, where $xb^i$ is the $i^{\text{th}}$ byte in $xb$ and $q$ represents the input dimensions (\ie, number of bytes or features). Then, once the MTNN has been trained, we can extract a transformation function $\mathrm{F}: xb\rightarrow z$, where $\mathbf{z}=\{z^1, z^2, ..., z^p\}$ is the \textit{compact embedding} of the input $\mathbf{xb}$ of size $\mathit{p}$ nodes such that, $\mathit{p} < \mathit{q}$. In other words, $\mathbf{z}=\mathrm{F}\left(\mathbf{xb}\right)$, is a low-dimensional representation of the input bytes in $\mathbf{xb}$ expressed with the help of a function $\mathrm{F}$. This is illustrated in \fig{bg_fig_1}.

% % In the context of this paper, the input $\mathbf{xb}$ represents a binary file format. Hence, a \textit{feature} refers to the input bytes and each of the $p$ features represents a byte. 

% An important property of the compact embedding is that, for every byte that changes in $\mathbf{xb}=\{xb^1,...,xb^q\}$, we obtain a corresponding change in every node in $\mathbf{z}=\{z^1, ..., z^p\}$. The extent of the change is determined by how influential each of the $q$ bytes in the input $\mathbf{xb}$ are to the overall MTNN model, \ie, the \textit{more influential} bytes produce \textit{larger} changes to $\mathbf{z}$ compared to less influential bytes. % In theory, if we can measure the magnitude of the 

% \subsection{Gradient guided mutation}
% \label{sect:gradients}

% We propose the use of \textit{gradients} to compute the importance of each byte in $\mathbf{xb}$ to the MTNN model. Gradient computation is supported by a rich literature on techniques such as \textit{automatic differentiation}~\cite{wengert1964simple,block1991siam,baydin2018automatic}. In this paper, we compute the gradient between the nodes in the compact embedding layer ($\mathbf{z}$) \wrt to the input bytes ($\mathbf{xb}$). More formally, we compute the \textit{Jacobian Matrix} given below: 
% % 
% % \begin{equation}   
% %     \label{eq:jacobian0}
% %     \mathbf J = \begin{bmatrix}
% %         \dfrac{\partial z^1}{\partial xb^1} & \cdots & \dfrac{\partial z^1}{\partial xb^q}\\
% %         \vdots & \ddots & \vdots\\
% %         \dfrac{\partial z^p}{\partial xb^1} & \cdots & \dfrac{\partial z^p}{\partial xb^q} 
% %     \end{bmatrix}
% % \end{equation}
% % More succinctly, we may express \eq{jacobian0} as:
% % \begin{equation}
% %     \label{eq:jacobian}
% %     \mathbf J = \begin{bmatrix}
% %     \dfrac{\partial \mathbf{z}}{\partial xb^1} & \cdots & \dfrac{\partial \mathbf{z}}{\partial xb^q} \end{bmatrix}  
% % \end{equation}
% % 
% \begin{equation}
%     \label{eq:jacobian}
%     \mathbb{J} = \begin{bmatrix}
%     \dfrac{\partial \mathbf{z}}{\partial xb^1} & \cdots & \dfrac{\partial \mathbf{z}}{\partial xb^q} \end{bmatrix}  
% \end{equation}
% The above Jacobian matrix has a dimensionality of $p\times q$, where each column ($\partial \mathbf{z}/\partial xb^i$) is a $\mathit{q-dimensional}$ column vector that represents the gradient of all the nodes in the compact-embedding layer $\mathbf z$ with respect to the $i$-th byte, \ie, the first column measures the gradients of each of the nodes in the compact-embedding layer with respect to the first byte in the input ($xb^1$), the second column with respect to the second byte in the input ($xb^2$), and so on for all $q$ bytes in the input.
% For example, the $i$-th column of \eq{jacobian} (\ie, $\partial \mathbf{z}/\partial xb^i$) is represented by the column vector, given by:
% \begin{equation}
%     \label{eq:jacobian_2}
%     \dfrac{\partial \mathbf{z}}{\partial xb^i} = J_z(xb^i) = \begin{bmatrix}
%     \dfrac{\partial z^1}{\partial xb^i} & \cdots & \dfrac{\partial z^p}{\partial xb^i} \end{bmatrix}^\mathbf{T}  
% \end{equation}


% In order to infer the importance of each byte $xb^i\in xb$ using \eq{jacobian}, we compute the \textit{saliency map}, represented by $\mathrm{S}(\mathbf{xb})$. It is given by, 
% \begin{equation}
%     \label{eq:hot_byte}
%     \mathrm{S}(\mathbf{xb}) = \begin{bmatrix}
%     \sum{\left|J_z (xb^1)\right|} & \cdots & \sum{\left|J_z (xb^q)\right|} \end{bmatrix} 
%     % = \begin{bmatrix}
%     % \sum_{i=1}^{p}{\dfrac{\partial \mathbf{z^i}}{\partial xb^1}} & \cdots & \sum_{i=1}^{p}\dfrac{\partial \mathbf{z^i}}{\partial xb^q} \end{bmatrix}  
% \end{equation}
% Here, $\mathrm{S}(\mathbf{xb})$ is a vector of length $\mathit{q}$. The $i$-th element in $\mathrm{S}(\mathbf{xb})$ represents the sum of all the gradients of the compact-embedding nodes ($\mathbf{z}$) \wrt the  $i$-th input byte $xb^i$.
% Note that, 
% \bi 
% \item The $\mathit{i}^{th}$ element in $\mathrm{S}(\mathbf{xb})$ measures the \textit{average influence} the $\mathit{i}^{th}$ input byte ($xb^i$) has on \textit{all} the nodes in the compact layer. 

% \item The numeric value of each of the $\mathit{q}$ elements in $\mathrm{S}(\mathbf{xb})$ determines the hotness of each of the bytes. The larger the value, the more likely it is that the byte is potentially a \textit{hot-byte}.
% \ei 

% \input{tex/hot_bytes.tex}

% Using the \textit{saliency map} ($\mathrm{S}(\mathbf{xb})$) from~\eq{hot_byte} we can now mutate the existing inputs to generate new ones using \textit{gradient ascent}. Given an initial input $xb^{t}$, we can now generate the next input  $xb^{t+1}$ as $xb^{t+1} = xb^{t} + \alpha \cdot \sum{\left|J_z (xb_t^i)\right|}$, where $\alpha$ is the step-size of the mutation. In fact, each input byte can be mutated as:
% {
% \setlength{\abovedisplayskip}{0pt}
% \setlength{\belowdisplayskip}{0pt}
% \begin{equation}
%     \label{eq:eq_5}    
%     xb_{t+1}^i = xb_{t}^i + \alpha \cdot \sum{\left|J_z (xb_t^i)\right|}\hspace{1em}\forall xb_t^i\in~xb_t
% \end{equation}
% }
% From~\eq{eq_5}, we see that when $\sum{J_z (xb_t^i)}$ is \textit{large}, that byte location is mutated by a larger extend compared to when $\sum{J_z (xb_t^i)}$ is \textit{small}. In other words, the more \textit{hot} a byte-location is, the more it is mutated.

% As an example, we inspect the extent of mutation at each byte location is mutated in ELF binaries (see \fig{hotbytes}). We find that the key regions such as \textit{ELF header} and \textit{Section header} are mutated to the greatest extent. Intuitively, this make sense because these regions play a major role in triggering unique program behaviors as compared to other regions. 

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \subsubsection{Distribution of Hot-bytes}
% % \label{sect:hotbytes}
% % In order to define \textit{hot-bytes} formally, let us represent a test input $x$ of length $n$ as a set of bytes $x=\{x_1, x_2, x_3, ..., x_n\} \in \{0, 255\}^n$. Each byte $x_i$ in $x$ is in-turn comprised of 8 bits. This means that a byte $x_i$ is a boolean function $x_i\equiv f:\{0, 1\}^p$ where $p$ is called the \textit{arity} of the boolean function $f$. Since a byte contains 8 bits, $p=8$, i.e., $x_i\equiv f:\{0, 1\}^8$. If a byte $x_i$ is ``hot'', then a change in at least one of the bits in $x_i$ will lead to a corresponding change in the edge coverage $Y$. This allows us to define a ``probability
% % that the $j^{th}$ bit in $x_i$ affects the number of edges invoked $\mathrm{Y}$''. This probability is known as the \textit{influence} function $\operatorname{Inf_j}(\cdot)$~\cite[p.~46, \S~2.2]{o2014analysis}:
% % %
% % \begin{equation}
% %     \operatorname{Inf}_j[x_i] = \mathbb{P}(\mathrm{Y}~|~x_{i,~j}=1)
% % \end{equation}
% % %
% % Here, $x_i$ is a byte in the input $x$, and the $j^{th}$ bit in $x_i$ is represented as $x_{i,~j}$. To measure if the whole byte $x_i$ is a ``hot-byte'', we need to aggregate the influence $\operatorname{Inf_j}(\cdot)$ for all the 8 bits in $x_i$. This measure is called the total influence $\operatorname{I}(\cdot)$ in boolen algebra~\cite[p.~49, \S~2.3]{o2014analysis}, it is defined as follows:
% % %
% % \begin{equation}
% %     \label{eq:total_influence}
% %     \operatorname{I}(x_i) = \sum_{j=1}^{8}\operatorname{Inf}_j[x_i] = \sum_{j=1}^{8}\mathbb{P}(\mathrm{Y}~|~x_{i,~j}=1)
% % \end{equation}
% % %
% % From the context of hot-bytes, the \textit{total influence} measure $\operatorname{Inf_j}(\cdot)$ can be understood as follows:
% % %
% % \be[leftmargin=*]
% % \item $\operatorname{I}(x_i) = 0$: The total influence of a byte $x_i$ is zero. This means that, regardless of which bit $j$ in $x_i$ is changed, it has no impact on the edge coverage $Y$. Therefore this byte will not be a ``hot-byte''.
% % \item $\operatorname{I}(x_i) > 0$: The total influence of a byte $x_i$ is positive. This means that, when one or more bits $j$ in $x_i$ are changed, there is a \textit{non-zero impact} on the edge coverage $Y$. Therefore this byte will potentially be a ``hot-byte''. Note that, the \textit{larger} the value of $\operatorname{I}(x_i)$, the \textit{more likely} the byte $x_i$ is a ``hot-byte''. 
% % \ee
% % %
% % Now, it is possible to obtain all the hot-bytes in an input $x={x_1,~x_2,~x_3,~...~,~x_n} \in \{0,~255\}^n$. To do this, let us partition the set of input bytes $x_i \in x$ into two disjoint subsets $A\subset x$ and $B\subset x$ such that $A\cap B=\varnothing$ and $A\cup B=x$. Then $A$ would represent all the \textit{hot-bytes} in $x$ if:
% % \begin{equation}
% % \label{eq:eq_3}
% %     \operatorname{I}(x_p) > \operatorname{I}(x_q)\hspace{1em} \forall x_p\in A,~x_q\in B    
% % \end{equation}
% % Guiding fuzzing towards these \textit{hot-bytes} can be achieved trivially if the conditional distribution of $P(\mathrm{Y}~|~x)$ is known. All that would have to be done is: 
% % %
% % \be[leftmargin=*]
% % \item Partition the input bytes according to~\eq{eq_3};
% % \item For each byte $x_p$ in the set of hot-bytes $A$, we set the bits $j$ in $x_p$ such that~\eq{total_influence} is satisfied. 
% % \ee
% % Performing the above two steps with ensure that~\eq{eq_1} is satisfied. Unfortunately, it is not possible to know $P(\mathrm{Y}~|~x)$ before hand and therefore, evolutionary greybox fuzzers like AFL resort to performing random mutations over the bytes in the input. At each iteration they only retain those mutated inputs that achieve new edge coverage. Since hot-bytes are most likely to increase coverage, these newly generated test inputs are most likely to have had mutations performed on the locations corresponding to these hot-bytes. Consequently, over a large number of iterations, greybox fuzzers gradually focus the mutations on these ``hot'' byte locations. 

% % \input{tex/hot_bytes.tex}

% % \fig{hot_bytes} illustrates the distribution of hot-bytes in \textit{readelf} (one of our test programs). This figure was obtained after running AFL for 1 hour and gathering the byte-location of the mutations and the corresponding edge coverage. Notice that the locations highlighted in red have significantly higher probability of invoking new edges as compared to the rest; these locations represent the \textit{hot-bytes}.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% % The goal of \textit{mutational greybox fuzzers} (hereafter \GF) is to maximize edge coverage (\ie, the number of  control flow edges) given a fixed amount of resource (e.g., time). Therefore, \GF can be thought of an optimization problem, where it searches over the entire input space to maximize edge coverage . 
% % Thus, if \allx is the space of all possible inputs to a program, a \GF tries to search over \allx to maximize the total edge coverage (\ally) within a fixed budget, say $\mathcal{T}$. 
% % More formally, if $E_t$ is the set of edges covered by input $x_t\in\mathcal{X}$ at fuzzing step $t$, and function $f: x_t\rightarrow E_t$ maps program inputs ($x_t$) to the covered edges $E_t$, then \gf can be formally represented as:
% % % 
% % \begin{equation}
% %     \setlength{\abovedisplayskip}{0pt}
% %     \setlength{\belowdisplayskip}{0pt}
% %     \label{eq:formal_main_0}
% %     \mathcal{Y_\mathcal{T}} =
% %     \max\norm{~\bigcup_{t=1}^\mathcal{T} E_t  }
% %                 = \max_{x_t\in\mathcal{X}}\norm{~\bigcup_{t=1}^\mathcal{T} f(x_t)}
% % \end{equation}
% % % 
% % Here $\|\cdot\|$ represents the norm and $\bigcup(\cdot)$ represents the union of all elements.~\eq{formal_main_0} indicates that maximization the union of $f(x)$ happens over all possible inputs. % and the norm takes the aboslute value of the union
% % Since the input space \allx of real-world programs is typically large, an exhaustive search to maximize \eq{formal_main_0} is infeasible. 
% % Instead, one needs to identify and focus the search on promising regions that will maximize edge-coverage. 
% % To identify such promising inputs, most \GF generates  mutated inputs using the following {mutation parameters}: 
% % (i) \textit{Input ($x\in$\allx)}: the input to mutate; 
% % (ii) \textit{Mutation location ($ml$)}: which byte location (offset) will be mutated, and 
% % (iii) \textit{Mutation operator ($mo$)}: the mutation operation to perform on those byte locations. 

% % Thus, given an input $x_{t-1}$ at step $(t-1)$, the next generated
% % input $x_{t}$ depends on $x_{t-1},m_l,m_o$.
% % The set of edges $E_t$ covered by $x_t$ can be represented as a function ($F$) of these three fuzzing parameters, i.e.,~$E_t=F(x_{t-1},m_l,m_o)$. Thus,~\eq{formal_main_0} can be written as: 
% % {
% % \setlength{\abovedisplayskip}{0pt}
% % \setlength{\belowdisplayskip}{0pt}
% % \begin{equation}
% %     \label{eq:formal_main}
% %     %\vspace{-2mm}
% %     \mathcal{Y_\mathcal{T}} 
% %     %= \maximize_{x,ml,mo}\norm{~\bigcup_{t=1}^\mathcal{T} E_t}  
% %     = \max_{x_{t-1},ml,mo}\norm{~\bigcup_{t=1}^\mathcal{T}F(x_{t-1},ml,mo)~}
% % \end{equation}
% % }

% % Note that, in the above equation, $x_0$ is an initial seed input.
% % In the rest of this section, we will discuss how the current state-of-the-art fuzzers realize this optimization (\eq{formal_main}), their limitations, and how our framework can help address these issues.


% % \subsection{Parameterized Mutation} 
% % \label{sec:egf}
% % % \smallskip
% % % \noindent
% % % \textbf{Evolutionary Fuzzing.} 
% % Graybox fuzzers applies mutations iteratively starting from all the initial seeds until the budget is exceeded. Different mutation strategies target different information sources, \eg input formatting~\cite{godefroid2017learn}, rare-edges~\cite{lemieux2017fairfuzz}, \etc, to improve these fuzzers. 
% % All tend to find promising input regions (i.e., byte locations), typically called \textit{hot-regions}, that need to be mutated for increasing edge-coverage. 

% % % It has been observed by several researchers in the past that, for real-world target programs, certain inputs regions (i.e., byte locations) tend to be far more likely to invoke new edge coverage compared to other regions~\cite{taintscope, rajpal2017not,lemieux2017fairfuzz,chen2018angora,vuzzer}. These byte locations are called \textit{hot-regions}. \fig{hot_bytes} shows the hot regions for \textit{readelf}, one of our target programs. The hot regions of the input (highlighted in red) have significantly higher probability of invoking new edges (see the edge coverage histogram) as compared to the rest.

% % % \input{tex/hot_bytes.tex} 

% % %Different graybox fuzzers use 
% % The mutation strategies, in general, involve 
% % program analysis or different types of aggregate statistics to identify the hot regions. 
% % Once identified, these fuzzers use this information to set some mutation parameters to focus more on the hot regions. There are three main types of parameters in the literature: seed inputs, mutation locations, and mutation operations. 
% % Table~\ref{tab:who_does_what} shows previous work involving different mutation strategies and parameters. %Significant research effort has been focused on developing different heuristics to select these parameters. 
% % We provide a brief summary below:
% % \input{tex/heursitics.tex}

% % \mybullet \textit{Input selection}: In AFLFast~\cite{bohme2017coverage}, B\"{o}hme et al. propose the use of heuristics such as power schedules in conjunction with Markov chains to assist in prioritizing the input queue for mutation.

% % \mybullet \textit{Mutation location selection}: FairFuzz~\cite{lemieux2017fairfuzz}, ProFuzz~\cite{You2019ProFuzzerOI} and SLF~\cite{You2019SLFFW} modify the mutation strategy of AFL by using aggregate statistics to identify which input regions are most likely to trigger ``rare-branches''. In contrast, Vuzzer~\cite{vuzzer}, Steelix~\cite{steelix} and Angora~\cite{chen2018angora} use dynamic taint analysis to identify hot regions and focus on mutating them more. 

% % \mybullet \textit{Mutation operator selection:} Angora~\cite{chen2018angora} %and NeuZZ by She et al.~\cite{she2018neuzz}
% % uses coordinate decent to guide mutations, while Vuzzer~\cite{vuzzer} uses a hybrid approach involving static analysis to identify promising mutation operations.

% % However, these approaches are usually used in ad hoc manner on top of AFL and may not generalize well across different programs or even across different regions of the same programs. For example, the approaches based on aggregated statistics on edge coverage behavior~\cite{bohme2017coverage,lemieux2017fairfuzz} misses many local input-specific variations in edge coverage, while taint-tracking based strategies are known to suffer from high false positives/false negatives~\cite{she2018neuzz,she2019neutaint}. 

% % %They are either based on aggregated statistics on edge coverage behavior~\cite{bohme2017coverage,lemieux2017fairfuzz}, 
% % %or depends on static/dynamic program analysis approaches like taint tracking.
% % %While the former misses many local input-specific variations in edge coverage, the latter are known to suffer from 
% % %high false positives/false negatives~\cite{she2018neuzz,she2019neutaint}. 

% % \subsubsection{Modeling mutations with NN. }~In this paper, we argue that an alternative way to approximate the function in~\eq{formal_main} is to use a neural network (NN) as the \textit{universal approximation theorem} states that ``A feed-forward network with one or more hidden layers, containing a finite number of neurons, can approximate any non-linear, non-convex, or a bounded discontinuous function~\cite{funahashi1989approximate, csaji2001approximation, anil2018sorting}. An added advantage of such NN-based approximation would be to directly use gradient guided approach to solve the optimization problem of fuzzing.  The latter is particularly enticing over the traditional evolutionary approaches due to its efficiency and better convergence guarantees~\cite{Maheswaranathan2018, sra2012optimization, juditsky2011first}.
% % Following the universal approximation theorem, we can cast the fuzzing problem as a learning problem where the goal is to use NN 
% % to learn an approximate function that can map the program input space to the probability of each edge in the corresponding control flow graph being taken. 

% % More formally, given \allx represents the space of all possible 
% % inputs to a program, and $\mathrm{xb}\in\mathcal{X}$ denotes a single 
% % input byte of length $n$-bytes, 
% % $xb$ can be represented as byte vector $xb=\{xb^1, xb^2, ..., xb^n\}\in\mathrm{\left[0, 255\right]^n}$, where $xb^i$ is the $i^{\text{th}}$ byte in $xb$. 
% % Let us further assume that $\mathrm{E}=\{e^1, e^2, ..., e^n\}\in\mathrm{\left[0, 1\right]^m}$ represents an edge-vector, where a positive value denotes the probability of the edges invoked by $xb$, and $0$ otherwise;
% % %the edge coverage can be measured by the norm of the edge vector, \ie $y=\norm{E}$.
% % With this, we can construct a neural network (NN) which  takes $xb$ as input and  predicts $\mathrm{E}$ as output. 

% % Such an NN directly tries to learn the mapping function $F$ between input and  edge invocation probability (see \eq{formal_main}).
% % Once \tool is trained with a set of inputs and their corresponding edge vectors, we can extract from the NN the 
% % conditional probability ${P}(e^j~|~xb^i)$, 
% % \ie, the probability of invoking edge $e^j$ by input byte $xb^i$. 
% % Note that, such probability is an approximation of the actual 
% % dependency between $xb^i$ and $e^j$ based on the observed branching behavior in the training data. 

% % \subsubsection{Gradient-guided parametric Mutation.}~
% % An important property of \tool is that it allows efficient computing of first-order derivatives. 
% % %Specifically, it is possible for us to algorithmically evaluate the derivative of $\hat{P}(\mathrm{Y}~|~x)$ with respect to $x$. 
% % There is a rich literature on techniques such as \textit{automatic differentiation} which have been used extensively 
% % for computing derivatives of the parameters in an artificial neural network~\cite{wengert1964simple,block1991siam,baydin2018automatic}. 
% % Let $G(x)$ represent the function computed by \tool, 
% % \ie, output edges $\mathrm{E}$ exercised by input bytes $xb$. 
% % We can then compute the gradients of $G$ \wrt 
% % the input bytes $xb$ as: %. That is, we can obtain:
% % {
% % \setlength{\abovedisplayskip}{0pt}
% % \setlength{\belowdisplayskip}{0pt}
% % \begin{equation}
% %     \label{eq:eq_5}
% %         \nabla\mathrm{G(xb)} = \left[\frac{\delta\mathrm{G}}{\delta xb^1},~\frac{\delta\mathrm{G}}{\delta xb^2},~\frac{\delta\mathrm{G}}{\delta xb^3},~...~,~\frac{\delta\mathrm{G}}{\delta xb^n}  \right]
% % \end{equation}
% % }
% % The gradient values help us to understand how individual input byte affects the edge coverage, and thus, can locate the {\em hot-bytes}. For each input byte $xb^i \in xb$, there are two possibilities:
% % \squishlisttwo
% % \item[] (1) $\left| {\frac{{\delta G(xb)}}{{\delta {xb^i}}}} \right| > 0$:
% % If the absolute value of the gradient %$\nabla_{xb^i}G(xb)$ 
% % is \textit{non-zero}, then a change in $xb^i$ is likely to result in some change in the covered edges $\mathrm{E}$.
% % \item[] (2) ${\frac{{\delta G(xb)}}{{\delta {xb^i}}}} = 0$: 
% % If the gradient %$\nabla_{xb^i}G(xb)$ 
% % is \textit{zero}, then a change in $xb^i$ \textit{is unlikely to} result in a change in the covered edges $\mathrm{E}$.
% % \squishend
% % % It can be observed that, conceptually, the value of the gradients resembles the distribution of \textit{hot-bytes} discussed previously. Our results demonstrate that this is indeed the case. For example, in~\fig{hot_bytes} we plot the distribution of gradients for readelf along with the hot-bytes obtained from AFL. 
% % \noindent
% % These gradient values resemble the \textit{hot-byte} distributions, \ie, higher the absolute value of a gradient, 
% % the higher the hotness of the corresponding byte. 
% % %Our results in~\fig{hot_bytes} demonstrate that this is indeed the case\textemdash  the hot-byte distribution obtained from AFL closely resembles the gradient values computed at those byte locations. 
% % %Thus, the gradients of \tool can be used to identify the 
% % %represents the distribution of hot-bytes.

% % %\input{tex/ga_vs_gd.tex}

% % Using the gradients from~\eq{eq_5} we can now solve the original 
% % \gf problem (see~\eq{formal_main}) using a simple \textit{gradient ascent} method. Remember that the success of \gf depends on three fuzzing parameters: (i) initial inputs, (ii) mutation location ($ml$), and (iii) mutation operations ($mo$).  
% % Given an initial input $xb^{t}$ to \tool, we can now generate the next input  $xb^{t+1}$ as $xb^{t+1} = xb^{t} + \alpha \cdot \nabla G(xb^{t})$, where $\alpha$ is the step-size of the mutation.
% % In fact, each input byte can be mutated as:
% % {
% % \setlength{\abovedisplayskip}{0pt}
% % \setlength{\belowdisplayskip}{0pt}
% % \begin{equation}
% %     \label{eq:eq_7}    
% %     xb^{t+1}^i = xb^{t}^i + \alpha \cdot \frac{\delta\mathrm{G}}{\delta xb^{t}^i}\hspace{1em}\forall xb^t^i\in~xb^t
% % \end{equation}
% % }
% % From~\eq{eq_7}, we see that when $\nabla_{xb^i}G(xb)$ is \textit{non-zero}, that byte location is mutated by the step-size $\alpha$ and when $\nabla_{x_i}G(x)$ is \textit{zero}, we make no change to that byte. Thus, \wrt \eq{formal_main}, mutation location ($ml$) can be detected by such non-zero gradients and the corresponding mutation operation ($mo$) can be determined by step-size. In such framework, 
% % the original fuzzing equation of \eq{formal_main} can be rewritten as:
% % $\mathcal{Y_\mathcal{T}} \equiv\max_{xb^{t}\in\mathcal{X}}\norm{~\bigcup_{t=0}^{\mathcal{T}-1}G(xb^{t} + \alpha \cdot \nabla G(xb^{t})~}$.


% % \input{tex/eq_fig.tex}


% % To further incorporate the dependency of \gf on the inputs, 
% % we introduce a \textit{selection operator} $C(\mathcal{X})$ that selects the most salient inputs from the original input space \allx. Thus, in \tool framework, we can reformulate the optimization problem as:
% % {
% % \setlength{\abovedisplayskip}{0pt}
% % \setlength{\belowdisplayskip}{0pt}
% % \begin{equation}
% % %\label{eq:formal_main_final}
% % \label{eq:eq_8}
% %     \mathcal{Y_\mathcal{T}} 
% %     \equiv\max_{xb \in C(\mathrm{X})}\norm{~\bigcup_{t=0}^{\mathcal{T}-1}G(xb^{t} + \alpha \cdot \nabla G(xb^{t})~}
% % \end{equation}
% % }
% % % \begin{equation}
% % %     \label{eq:eq_8}
% % %     \text{Fuzzing}~\equiv~\max_{x \in C_p(\mathrm{X})}\left[\sum_{i=1}^{n}G(x_i)\right]
% % % \end{equation}
% % \subsubsection{Adapting mutation strategies.}~It is worth noting that solving~\eq{eq_8} with gradient ascent is an inherently adaptive framework. It lends itself neatly to incorporating a number of mutation strategies that can target different information sources, as discussed in 
% % Section~\ref{sec:egf}.  These information sources manifest themselves as parameters of the optimization problem. 
% % By carefully choosing these parameters, we can guide the fuzzing towards the most desirable regions of the input that will increase the edge-coverage. This is illustrated in~\fig{optimization_parameters}:

% % \be[leftmargin=*]
% % \item \textit{On input selection}: 
% % In \subfig{4_a}, \circled{1} shows that the optimization occurs over the space defined by the \textit{selection operator} $C(\mathrm{X})$. 
% % This parameter is similar to the input selection strategies of B\"{o}hme et al.~\cite{bohme2017coverage}. 
% % Our selection operator is detailed in \tion{seed_selection}.

% % \item \textit{On mutation location selection}: 
% % In \subfig{4_b}, \circled{2} shows that the gradients are used to make updates to the specific byte locations\textemdash zero gradient means no updates. This parameter is comparable to the studies related to mutation location selection strategies~\cite{lemieux2017fairfuzz}. 
% % See \tion{offset_selection} for details. 
% % %, we discuss in detail how we can train neural networks to perform gradient guided fuzzing.

% % \item \textit{On mutation operation selection}: 
% % In \subfig{4_b}, \circled{3} represents the step-size of the mutation. By modifying this parameter, we can control how the mutation operator is implemented. % This is analogous to the heuristics proposed by Angora~\cite{chen2018angora}.% In \tion{opertaion_selection}, we discuss how to choose this parameter.
% % \ee

% % To incorporate different source of information (\eg branch coverage, rare-edges, \etc), 
% % it is also possible to encode training data with different information source or modify the loss function of NN.
% % For example, in~\tion{soft_label}, we show how to encode output variable $E$ to incorporate branch distance.
% % ~\tion{offset_selection} further shows how we can modify loss function to incorporate rare-edge information. In such cases, \tool will learn a new approximate function, say $G'$. \circled{4} in \subfig{4_b} represents this step. 

% % % In fact, it is also possible to replace the dependent variable $E$ (which represents covered edges) with alternatives such as \textit{branch distance} to further guide fuzzing towards \textit{hard-to-reach} sections of the code (see~\tion{soft_label} for details). In such case \tool will learn a new approximate function, say $G'$. \circled{4} in \subfig{4_b} represents this step. 

% % %We show in \tion{soft_label} that, with our neural framework,

% % % Finally, \circled{4} in \subfig{4_b} represents a novel contribution of this paper. We show in \tion{soft_label} that, with our neural framework, it is possible to replace the dependent variable $Y$ (which represents edge coverage) with alternatives such as \textit{branch distance} to further guide fuzzing towards \textit{hard-to-reach} sections of the code. 

% % % \input{tex/intro_fig.tex} 



% % %Here, blocks highlighted in \colorbox{lightgray}{gray} to represent the mutation parameters that we choose to address the common challenges faced by the current state-of-the-art fuzzers. 








% % % We may expand~\eq{eq_6}, for each byte $x_i\in x$ as follows: 
% % % \begin{equation}
% % %     \label{eq:eq_7}    
% % %     x^{t+1}_i = x^{t}_i + \alpha \cdot \frac{\delta\mathrm{G}}{\delta x_i}\hspace{1em}\forall x_i\in~x
% % % \end{equation}
% % % From~\eq{eq_7}, we see that when $\nabla_{x_i}G(x)$ is \textit{non-zero}, that byte location is mutated by the step-size $\alpha$ and when $\nabla_{x_i}G(x)$ is \textit{zero}, we make no change to that byte. This ensures that bytes that have some effect on invoking edge coverage (i.e., \textit{hot-bytes}) are mutated while the remaining bytes remain unchanged.

% % % \subsubsection{Constructing an adaptive framework}
% % % \label{sect:adaptive_framework} 
% % % In theory, the above formulation (\eq{formal_main_g}) for solving fuzzing as a gradient based optimization can ensure strong convergence guarantees~\cite{Maheswaranathan2018}, in practice however, it may take prohibitively long to converge. It is therefore advisable to incorporate additional parameters to the optimization in form of budget constraints. 
% % % \input{tex/eq_fig.tex}
% % % According to~\eq{eq_4}, the input samples $x$ belonged to the space of all possible samples $\mathrm{X}$ (i.e., $x\in X$). This space is combinatorially large and for practical purposes it may not be possible to exhaustively explore the whole space. Therefore, we introduce a optimization budget $K$ that limits the number of samples we choose from the space of $\mathrm{X}$. We introduce a \textit{selection operator} $C_p(\mathrm{X})$ that selects the $K$ most salient samples from the original space of $\mathrm{X}$. Now, we may reformulate the original optimization problem as:
% % % \begin{equation}
% % %     \label{eq:eq_8}
% % %     \text{Fuzzing}~\equiv~\max_{x \in C_p(\mathrm{X})}\left[\sum_{i=1}^{n}G(x_i)\right]
% % % \end{equation}

% % % It is worth noting that solving~\eq{eq_8} with gradient ascent is an inherently adaptive framework. It lends itself neatly to incorporating a number of heuristics. We see that the heuristics discussed in \tion{heuristics} manifest themselves as parameters of the optimization problem. By carefully choosing these parameters, we can guide the fuzzing towards the most desirable regions of the input. This is illustrated in~\fig{optimization_parameters},
% % % \be[leftmargin=*]
% % % \item In \subfig{4_a}, \circled{1} shows that the optimization occurs over the space defined by the \textit{selection operator} $C_p(\mathrm{X})$. This parameter is similar to the input selection strategies of studies like that of B\"{o}hme et al.~\cite{bohme2017coverage}. Our selection operator is detailed in \tion{seed_selection}.
% % % \item In \subfig{4_b}, \circled{2} shows that the gradients are use to make updates to the specific byte locations. If, at a specific byte, the gradient is zero, then no update happens there. This is comparable to the mutation location selection strategies of studies like that of FairFuzz\cite{lemieux2017fairfuzz}. In \tion{offset_selection}, we discuss in detail how we can train neural networks to perform gradient guided fuzzing.
% % % \item In \subfig{4_b}, \circled{3} represents the step-size of the mutation. By modifying this parameter, we can control how the mutation operator is implemented. This is analogous to the heuristics proposed by Angora~\cite{chen2018angora}. In \tion{opertaion_selection}, we discuss how to choose this parameter.
% % % \item Finally, \circled{4} in \subfig{4_b} represents a novel contribution of this paper. We show in \tion{soft_qabel} that, with our neural framework, it is possible to replace the dependent variable $Y$ (which represents edge coverage) with alternatives such as \textit{branch distance} to further guide fuzzing towards \textit{hard-to-reach} sections of the code. 
% % % \ee


==> body/3_methodology_bck.tex <==
\section{Methodology}
\label{sect:our_method}
% -=--=--=--=--=- Version 3 -=--=--=--=--=-
%The goal of any grey box fuzzers is to maximize code coverage within a fixed computation budget. In general,~\textit{code coverage} measures how many code elements (\eg edge, path, call site, etc.)  in the program are executed by a given test input.
This section presents a brief overview of \tool that aims to maximize \ec with the aid of two additional coverage measures: \ctx and \softlabel using multi task learning.~\Cref{fig:intro_fig} illustrates an end-to-end workflow of the proposed approach. The first stage trains an MTNN to produce a compact embedding of an otherwise sparse input space while preserving information about the hot bytes \ie, the input bytes have the highest likelihood to impact code coverage~(\Cref{sect:stage-1}). %These {\em hot-bytes} are  metrics.
The second stage identifies these hot bytes and focuses on mutating them~(\Cref{sect:stage-2}). Finally, in the third stage, the seed corpus is updated with the mutated inputs and retains only the most interesting new inputs~(\Cref{sect:stage-3}).
%To identify the hot-bytes, we use {\em saliency score} that measures the extent to which each input byte affects the compact embedding by computing impact of change in the input byte to the embedding\textemdash the hot-bytes should have the largest impact. \tool then mutates the hot-bytes with all possible permissible values. 
% \begin{goal}
%     {\normalfont\textsc{Definition 2:}}~The input bytes that have the highest likelihood of having an effect on code coverage metrics are referred to as ``hot-bytes''. 
% \end{goal}

% This achieved by training a multitask neural network (MTNN) to predict for the relationship between the inputs and three related tasks (or code coverage measures) namely, (a) \ec, (b) \ctx, and (c) \softlabel. Each task complements one another other by offering some additional information about how the input interacts with the program (discussed further in~\tion{tasks}). For example, while \ctx accounts for the changes to program's internal states caused by an input, \softlabel measures how close an input was to invoking an edge that was not previously triggered. Predicting for all these tasks simultaneously enables the MTNN to generate a compact embedding of the input that discards any task-specific variations and focuses on the sections of the input most relevant to all the tasks. In \tion{stage-1}, we discuss our MTNN in greater detail. 

% The goal of the second stage is to mutate the inputs on the most influential byte locations, \ie hot-bytes. Focusing mutations on these hot-bytes tends to result in significantly more code coverage. To identify the hot-bytes, we measure the extent to which each byte in the input affects the compact embedding layer. The hot-bytes usually have among the largest impact on the embedding layer. We measure the extent of the impact by computing the gradients of the embedding layer \wrt the input bytes. The locations in the input corresponding to the hot-bytes have the largest gradient values. The mutations are focused at these hot-byte locations. We discuss this in greater detail in \tion{stage-2}.

% that result in increased coverage. 
%. A newly generated seed input is deemed interesting if it reaches a previously unseen region of the program space. By selecting only the most interesting new inputs, we keep the corpus from growing uncontrollably in size. 

% In the rest of the section we first introduce the tasks we are modeling and then describe \tool's methodology in details.

% To quantify this, we define a \textit{saliency score} which is obtained by computing the gradients of the embedding layer \wrt the input bytes. The locations in the input corresponding to the hot-bytes have the largest gradients and therefore larger saliency scores. Therefore, the mutations are focused at those  We discuss this in greater detail in \tion{stage-2}.

% Why does this stage come first . . .
% Briefly, how does it work . . .
% What value does it add to the subsequent stages . . .

% % -=--=--=--=--=- Version 2 -=--=--=--=--=-
% In this section we present a brief overview of the \tool framework.~\fig{intro_fig} illustrates an end-to-end workflow of the proposed approach comprising of three stages: (i)~multi-task training; (ii)~gradient guided mutation; and (iii)~incremental learning.

% % Multitask }learning- what and why?
% In the first stage, we use the inputs from a seed corpus (far left in \fig{intro_fig}) to train a multi-task feed-forward neural network (MTNN) detailed in \tion{stage-1} to predict for three \textit{related} tasks (coverage measures) namely, (a) \ec, (b) \ctx, and (c) \softlabel. 
% Each task complements the others by offering some additional information about how the input interacts with the program (discussed further in~\tion{tasks}). \Red{for example...} Training for the tasks jointly enables the MTNN to discard any task specific noise and learn a more general representation of the input. 


% In the second stage, we make use of the shared embedding layer of the trained MTNN to infer the \textit{hot-bytes}. We compute the partial derivatives of the embedding layer \wrt the input layer (called the \textit{saliency score}) to find the influential input bytes. Bytes with the \textit{largest} saliency scores will be mutated. We discuss this in greater detail in \tion{stage-2}.

% In the third stage, we inspect the mutated seeds by running them on the instrumented program. We then update the seed corpus with only the most interesting new seeds. Selecting only the most interesting new inputs keeps the corpus from growing uncontrollably in size. The proposed selection strategy is discussed in detail in \tion{stage-3}. 

% -=--=--=--=--=- Version 1 -=--=--=--=--=-

% After training, the MTNN consists of two partitions of layers--- a set of shared intermediate layers and three task specific layers. 
% We begin with a set of seed inputs...
% For each of the inputs we assess how they impact the code coverage in terms of three coverage measures (a) Edge coverage, (b) Context sensitive branch coverage, and (c) approach level. We use a light-weight instrumentation to collect these. Next, we train a multi-task neural network to predict for each of the above coverage measures simultaneously.
% 
% \paragraph{Gradient guided mutation (Stage-II)}
% The shared intermediate layers results in providing a compact-embedding of the inputs. This embedding is a more general representation of the input that improves the overall predictive power for each of the three tasks. 
% Accordingly, more influential input bytes are expected to have a \textit{larger} impact on the compact embedding. In order to quantify the extent of this impact, we make use of gradients. Specifically, if we have \inlinemathit{q} input bytes and \inlinemathit{p} node in the compact-embedding layer, then we:
% \begin{inparaenum}[(i)]
%     \item compute the gradient of each of the \inlinemathit{p} nodes in the compact-embedding \wrt the each of the \inlinemathit{q} input bytes, and    
%     \item compute the sum of the gradients \wrt each of the \inlinemathit{q} input bytes. 
% \end{inparaenum} We call this sum the \textit{saliency} of the input byte. If the byte is more influential, then the saliency of that byte will be \textit{large}. Saliency score informs the fuzzer how to mutate-- bytes with greater saliency value will be mutated to greater extent. We discuss this greater detail in \tion{stage-2}.
% 
% \paragraph{Incremental learning (Stage-III)}
% After seed selection, Stage-I and Stage-II are repeated with the updated seed corpus. The whole process terminates after the allocated fuzzing budget has been exhausted. 

% We retain newly generated that result in ``rare'' behaviors they trigger, \eg, if an input invokes a rare control-flow edge or if it triggers a new internal state. 

\subsection{Modeling Coverage as Multiple Tasks}
\label{sect:tasks}

The goal of any ML-based fuzzers, including \tool, is to learn a mapping between input space and code coverage. The most common coverage explored in the literature is \ec, which is an effective measure and quite easy to instrument. However, it is coarse-grained and misses many interesting program behavior (\eg, explored call context) that are known to be important to fuzzing. One workaround is to model path coverage by tracking the program execution path per input. However, keeping track of all the explored paths can be computationally intractable since it can quickly lead to a state-space explosion on large programs~\cite{Wang2019}. As an alternative, in this work, we propose a middle ground: we model the \ec as the primary task of the MTNN, while choosing two other fine-granular coverage metrics (\softlabel and \ctx) as auxiliary tasks to provide useful additional context to \ec. %while still preventing state-space explosion. 

% To learn how various inputs interact with the program's state space, we use a machine learning model to learn a mapping between the inputs and the various regions of the program space that are reached by those inputs. One possible way to build this ML-model is by predicting for edge coverage, \ie, predicting edges in the control-flow graph are explored by the inputs. 
% This approach reasonably effective and quite easy to instrument. However, it tends to be too coarse an estimation. Monitoring the edges in isolation does not account for several crucial of the program behavior. Therefore, training a machine learning model that just learns to predict for edge coverage is inadequate. 

% Alternatively, we may increase the granularity by predicting for the path-coverage, \ie, which execution paths in the program's control-flow graph are traversed by the inputs. However, enumerating all the possible paths in the control-flow graph is computationally intractable since keeping track of all the explored code paths, especially for large programs can quickly lead to an explosion of the state space~\cite{Wang2019}.

% Thus, as an alternative to path coverage, we increase the granularity of prediction by selecting two additional coverage metrics. These metrics augment edge coverage by adding more contextual information to triggered each edge. To account for the distance between an explored and unexplored edges we use \softlabel (\tion{softlabel}). To account for other internal states that were involved when an edge is triggered, we use \ctx  (\tion{ctx}). These measures, when used in conjunction with edge-coverage, provide useful addition information while preventing state-space explosion. 

% To learn how various inputs interact with the program's state space, we use a  
% machine learning model to learn a mapping between the inputs and the various regions of the program space that are reached by those inputs. One possible way to build this ML-model is by predicting for which execution paths in the program's control-flow graph are traversed by the inputs, \ie, predicting for path-coverage. However, enumerating all the possible paths in the control-flow graph can quickly lead to an explosion of the state space, therefore being computationally intractable.

% As alternative to path-coverage, we may model the which edges in the control-flow graph are explored by the inputs. This approach reasonably effective and quite easy to instrument. However, it tends to be too coarse an estimation. It does not account for several crucial of the program behavior such as--- how far an input is from an unexplored edge, or what other internal states were invoked. Therefore, training an machine learning model that learns to predict only for edge coverage inadequate. 

% We Measure at the program states exercised by an input at different levels of granularity 

% . Further, the state space often explodes to .%\rahul{good to have a citation here.}

% Thus, as an alternative to path coverage, we increase the granularity of prediction by selecting two additional coverage metrics. These metrics augment edge coverage by adding more contextual information to triggered each edge. To account for the distance between an explored and unexplored edges we use \softlabel (\tion{softlabel}). To account for other internal states that were involved when an edge is triggered, we use \ctx  (\tion{ctx}). These measures, when used in conjunction with edge-coverage, provide useful addition information while preventing state-space explosion. 

% However, it is less precise than using path coverage, as edge coverage gives an aggregate statistic of the individual edges in all the explored code paths. 

\subsubsection{Edge coverage:~Primary Task.~}%\hfill
\label{sect:ec}

Edge coverage measures how many unique control-flow edges are triggered by a test input as it interacts with the program. 
It has become the de-facto code coverage metric~\cite{zalewski2017american,she2018neuzz,lemieux2017fairfuzz,You2019SLFFW} for fuzzing. 
We model edge coverage prediction as the {\em primary task} of our multi-task network, which takes a binary test case as input and predicts the edges that could be covered by the test case. 
For each input, we represent the edge coverage as an \textit{edge bitmap}, where value per edge is set to \texttt{1} or \texttt{0} depending on whether the edge is exercised by the input or not. 

In particular, in the control-flow-graph of a program, an edge connects two basic blocks (denoted by \texttt{prev\_block} and \texttt{cur\_block})~\cite{zalewski2017american}. A unique $edge\_id$ is obtained as: $hash(\texttt{prev\_block}, \texttt{cur\_block})$.  %$hash(\texttt{prev\_block},\-\texttt{cur\_block).
% An unique $edge\_id$ is obtained as follows:% $hash(\texttt{prev\_block}, \texttt{cur\_block)$. That is,
% {
% %  \setlength{\abovedisplayskip}{1pt}
% \setlength{\abovedisplayskip}{0pt}
%  \setlength{\belowdisplayskip}{0pt}
% \begin{equation}
% \label{eq:edge_id}
% edge\_id = hash(prev\_block\_id, cur\_block\_id)
% \end{equation}  
% }
For each $edge\_id$, there is a bit allocated in the bitmap. For every input, the \edgeids in the corresponding edge bitmap are set to \texttt{1} or \texttt{0}, depending on whether or not those edges were triggered. 

% Edge coverage measures how many unique control-flow edges are triggered by a test input as it interacts with the program. It is one of the most widely used code coverage metrics~\cite{zalewski2017american,she2018neuzz,lemieux2017fairfuzz,You2019SLFFW}. We model edge coverage prediction as the {\em primary task} in our multi-task network, which takes in test cases as input and outputs edge coverage metric. 

% % What does this measure, how is it instrumented, what it's missing
% Edge coverage measures how many unique control-flow edges are triggered by a test input as it interacts with the program. It is one of the most widely used code coverage metrics~\cite{zalewski2017american,she2018neuzz,lemieux2017fairfuzz,You2019SLFFW}. We model edge coverage prediction as the {\em primary task} in our multi-task neural network to reason about which input bytes are most likely to trigger specific edges in the \cfg. 
% %This will help quickly rule out all those bytes in the inputs that do not influence edge coverage in any way.

% %Incorporating edge coverage prediction as an individual task enables the multi-task neural network to reason about which input bytes are most likely to trigger specific edges in the \cfg. This will help quickly rule out all those bytes in the inputs that do not influence edge coverage in any way.

% This task falls under a multi-class classification paradigm where the MTNN attempts to predict all the unique \cfg edges triggered by the input. During training, the MTNN is provided with the edge coverage corresponding to each input in the form of an \textit{edge bitmap}. This edge bitmap contains a unique identifier for each edge (denoted by $edge\_id$). %In accordance with current practice~\cite{zalewski2017american}, 
% An edge is modeled transition between a pair of basic blocks (denoted by \texttt{prev\_block} and \texttt{cur\_block})~\cite{zalewski2017american}. The unique $edge\_id$ is obtained as follows:% $hash(\texttt{prev\_block}, \texttt{cur\_block)$. That is, 
% \begin{equation}
% \label{eq:edge_id}
% edge\_id = hash(prev\_block, cur\_block)
% \end{equation}  
% For every input, the \edgeids in the corresponding edge bitmap are set to \texttt{1} or \texttt{0} depending on whether those edges were triggered or not respectively. 

%An ML-model that only predicts for edge coverage would fall short because such a model would be too coarse grained. For edges that were not triggered, it would lack a distance measure to indicate how close an input was to triggering those edges. For the edges that are triggered, it would lack additional context pertaining to internal program states that were involved in triggering those edges.



% Given that an edge is transition between a pair of basic blocks (denoted by \texttt{prev\_block} and \texttt{cur\_block}), the unique $edge\_id$ may be obtained as follows:% $hash(\texttt{prev\_block}, \texttt{cur\_block)$. That is, 
% \begin{equation}
% \label{eq:edge_id}
% edge\_id = hash(prev\_block, cur\_block)
% \end{equation}  

% This task falls under multi-class classification paradigm where for each input the MTNN attempts to predict for all the unique edges triggered in the \cfg. 
% 
% 
% Trained on inputs to predict for 
% each input is paired with it corresponding edge coverage. 
% 
% 
% not know anything about the unseen edges in the \cfg. 
% Predicting for \ec falls under a multi-class classification paradigm with one class label for each unique edge in the \cfg. Trained on inputs to predict for 
% 
% An edge is transition between pairs of basic blocks (denoted by \texttt{prev\_block} and \texttt{cur\_block}). 
% To obtain an ID unique of each edge, we track all the conditional statements in the program and record the code blocks before and after each of conditional statements. 
% These code blocks are denoted by \texttt{prev\_block} and \texttt{cur\_block}, respectively. 
% An \textit{edge}, then, is a transition between two code blocks and it is represented as a tuple \texttt{(prev\_block, cur\_block)}. An \texttt{edge\_id} is assigned by encoding each tuple using a hash function $hash(\cdot)$. That is, 
% \begin{equation}
% \label{eq:edge_id}
% edge\_id = hash(prev\_block, cur\_block)
% \end{equation}  

% All the $edge\_id$s from \eq{edge_id} are stored in a global \textit{edge count} which maintains all the previously seen \inlinemath{edge\_id}s over several runs. 
% All the \edgeids are stored in an \textit{edge bitmap}. Every time a test input triggers a new \inlinemath{edge\_id} (unseen in the previous runs), the corresponding \edgeid in bitmap is marked as \texttt{1}. Otherwise, it is marked as 





\subsubsection{Approach-Sensitive Edge Coverage:~Auxiliary Task 1.~}%\hfill
\label{sect:softlabel}
\begin{wrapfigure}[16]{R}{0.45\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/approach_eg.pdf}
    % \vspace{-4mm}
    \caption{\small Approach Bitmap vs. Edge Bitmap. The edge `d' has a visited parent edge `b' and is thus marked 0.5 in the approach bitmap.}
    \label{fig:sl_eg}
    % \vspace{-3mm}
\end{wrapfigure}For an edge that is not exercised by an input, we measure how far off the edge is from getting triggered. Such a measure provides additional contextual information of an edge. For example, if two test inputs failed to trigger an edge, however one input reached ``closer'' to the unexplored edge than the other,  traditional  edge coverage would treat both inputs the same. However, using a proximity measure, we can discern between the two inputs and mutate the closer input so that it can reach the unexplored edge. 
To achieve this, \softlabel extends \ec by offering a distance measure that computes the distance between an unreached edge and the nearest edge triggered by an input. This is a popular measure in the search-based software engineering literature~\cite{McMinn2004,mcminn2011search,arcuri2010does}, where  instead of assigning a binary value (0 or 1), as in edge bitmap, \textit{approach level} assigns a numeric value between 0 and 1 to represent the edges~\cite{Phil2004Hyber}; if an edge is triggered, it is assigned \texttt{1}. However, if the edge is \textit{not} triggered, but one of its parents are triggered, then the non-triggered edge is assigned a value of $\beta$ (we use $\beta=0.5$). If neither the edge nor any of its parents are triggered, it is assigned $0$. This is illustrated in \fig{sl_eg}. Note that, for a given edge, we refrain from using additional ancestors farther up the \cfg to limit the computational burden. The approach sensitive coverage is represented in an \textit{approach bitmap}, where for every unique $edge\_id$, we set an approach level value, as shown in \fig{sl_eg}. We model this metric in our \MTNN as an auxiliary task, where the task takes binary test cases as inputs and learn to predict the corresponding approach-level bitmaps. 





% Approach-sensitive edge coverage extends \ec by offering a distance measure to all the edges % that are triggered and 
% % 
% % Edge coverage marks an edge as 1 if it is taken during runtime or 0, otherwise. 
% % When an edge is marked as 0, it does not 
% indicating \textit{how close} a given test input was to triggering those edges. For example, if two test inputs failed to trigger an edge, however one input was ``closer'' to the unexplored edge than the other, edge coverage would treat both inputs the same. However, using a distance measure, we can discern between inputs that are closer to unexplored edges and those that farther away. 

% Specifically, by including a task in the MTNN to estimate how close inputs are to non-triggered edges, we can discover the specific input bytes that are most likely to trigger the non-triggered edges in the \cfg.
% With further mutations to these bytes, we increase the chances of eventually triggering the edges. This would, in essence, augment the edge coverage by providing additional context (in the form of a proximity score) to the edges they were not triggered, \ie, those edge that were labeled \texttt{0} by edge coverage. 

% In this paper, we use $approach~level$. It measures the distance between an unreached edge and the nearest edge triggered by the input. This measure is popularly used in the search-based software engineering literature~\cite{McMinn2004,mcminn2011search,arcuri2010does}. Instead of assigning a binary value (0 or 1) as in the case of edge coverage, \textit{approach level} provides a numeric value between 0 and 1 to represent the edges~\cite{Phil2004Hyber}. 

% In approach level, the numeric value assigned to an edge depends on its parent edges. If an edge is triggered, it is assigned a value of \texttt{1}. However, if the edge is \textit{not} triggered, but one of it's parents are triggered, then the non-triggered edge is assigned a value of $\beta$ (we use $\beta=0.5$). If neither the edge nor any of it's parents are triggered, then it is assigned an value of $0$. This is illustrated in \fig{sl_eg}. Note that, for a given edge, we refrain from using additional ancestors farther up the \cfg to limit the computational burden. %Our findings suggest that using the parent (the first ancestor)  

% The approach level for each edge is maintained in an \textit{approach bitmap}. Similar to edge bitmap,  approach bitmap contains a unique identifier for each edge denoted by $edge\_id$ (computed according to \eq{edge_id}). For every input, the \edgeids in the approach bitmap are set to the approach level of corresponding edges (see \fig{sl_eg} for an example of an \textit{approach bitmap}). 

% works as follows:
% \beq
% \label{eq:eq_sl}
% appraoch\ level=\left\{
% \begin{array}{ll}
% 1                      & \text{The edge was triggered.}\\
% \multirow{2}{*}{\beta} & \text{The edge was \textit{not} triggered,} \\
%                       & \text{but one of the parent edges were triggered.}\\
% \multirow{2}{*}{0}     & \text{Neither the edge,} \\
%                       &  \text{nor its parents were triggered.}
% \end{array}
% \right.
% \eeq


% Since edge coverage is a binary mearure 

% Including distance measure  edge coverage prediction as an individual task enables the multi-task neural network to reason about which input bytes are most likely to trigger specific edges in the \cfg. This will help quickly rule out all those bytes in the inputs that do not influence edge coverage in any way.

% because we can guide mutations on the inputs to \textit{reduce the proximity} to the unexplored edges.


% \be
% \item If an edge has been reached, it is assigned a value of 1. 
% \item If the parent of the edge is reached but not the edge itself, then we assigned a value of \inlinemath{\beta} (0.5 in our case) to indicate that the parent was taken but not the current edge. 
% \item If the parent was not triggered by the input, then the current edge is assigned a value of 0.
% \ee

% In our multi-tasking framework, we model the task of predicting approach level\textemdash given a binary input, the output is the approach-level bitmap (see~\fig{sl_eg}). Such a model can learn to identify inputs closer to triggering an edge, and focus mutations on the input bytes that are likely to change the approach levels. %The ML-models trained to predict only \ec cannot provide such fine-granular information.

% In our multi tasking framework, we model the task of predicting approach level\textemdash given a binary input, the output is the approach-level bitmap (see~\fig{sl_eg}). 
% By training Machine Learning models to predict for the approach level, they can learn to distinguish between inputs that more likely to trigger an edge. For example, an ML model can learn which input bytes  affect the approach levels of various edges so as to focus mutations more on those bytes. ML-models trained to predict only \ec cannot provide this information.
% \begin{equation}
% \label{eq:dist_edge}
% dist\_edge=
%     \begin{cases}
%     1, & \text{if the edge is taken} \\ 
%     \beta, & \text{if}\ approach\ level =0 \\
%     0, & \text{if} \ approach\ level >0\\
% \end{cases}
% \end{equation}



% \subsection{Stage-I: Multi-task Training}
% \label{sect:stage-1}
% This phase builds a multi-task neural network (MTNN) to learn how the inputs in the seed corpus interact with the control-flow edges of the test program. The MTNN is designed such that, each input byte corresponds to one input node (as shown in \fig{bg_fig_1}). 
% \paragraph{Architecture} The MTNN is architectured such that there is an \textit{encoder} (shared among all the tasks) and three \textit{decoders} (one for each task). 
% \bi
% \item \textit{Encoder.} Comprises of one input layer followed by three \textit{progressively narrower} intermediate layers. The total number of nodes in the input layer is equal to the total number of bytes in the largest input in the seed corpus. All shorter inputs are padded with \texttt{0x00} for consistency. %Note, the layers in the encoder are \textit{shared} among all the tasks. 
% The last layer of the encoder is the most compact representation of the input that will be used by the tasks (highlighted \colorbox{greenish!80}{green} in \fig{bg_fig_1}). 
% \item \textit{Decoders.} There are three \textit{task-specific decoders} (shown in \colorbox{lavender}{violet} in \fig{bg_fig_1}). Each task specific decoder consists of three intermediate layers that grow \textit{progressively wider}. The last layer of each of the decoder is the output layer. Each node in the output layer corresponds to one output label of that task, \eg, for \ec task there is one node for each unique edge id, likewise for \ctx and \softlabel.
% \ei 
% \paragraph{Training}
% The MTNN is trained to predict for how inputs change the outcomes of each of the tasks. In order to train a MTNN, we must define a \textit{loss function}. 
% We define a multitask loss \inlinemathcal{L} for all three tasks as follows:
% \begin{equation}
%     \label{eq:adap_total}
%     \displaystyle
%     \mathcal{L} = -\sum\alpha_{\tau}\mathcal{L}_{\tau} \hspace{1em} \tau\in\{\tau_1, \tau_2, \tau_3\}
% \end{equation}
% This is a weighted sum of the loss $\mathcal{L}_{\tau}$ for each individual task. During the training phase, the MTNN attempts to minimize the multitask loss \inlinemathcal{L}.

% \subsubsection{Loss functions}\hfill%\newline\indent 
% \label{sect:adaptive_loss}

% The loss functions play a major role in 
% In our architecture, we have 3 tasks namely, \ec, \ctx, and \softlabel. Among these, \ec and \ctx are trained as a classification task, while \softlabel is trained as a regression task. Accordingly, we use the following loss functions for each of them:
% \be
% \item \textit{Loss function for classification:} This applies to \ec and \ctx. 
% Exhibit a lot of rare behaviour 
% Defining a loss-function for classification tasks need to account for the class imbalances, \ie while some classes (edge ids or call-stack ids) are invoked very often (mostly 1 value), some others are invoked rarely (mostly 0 value). Due this imbalance, MTNN that uses off-the-shelf loss functions such as cross entropy is ill suited for fuzzing, because they are prone to both (a)~\textit{Type-I errors} (or false positive errors) and (b)~\textit{Type-II errors} (or false negative errors). In order to accurately train an MTNN, we ought to mitigate for these errors. Thus we use the \textit{weighted cross entropy loss}, given as:
% % The binary cross entropy loss function, is formulated as:
% % 
% %p is a binary value. 1 means the edge was actually taken, 0 means it was not taken.
% % In order to classify the edges accurately, we must define a \textit{loss function}. 
% % A program's edge coverage is subject to a number of peculiarities. Specifically, we find that while some edges are invoked very often, some other edges are invoked very rarely. This is especially true for new inputs that invoke edges that have never been invoked before. Due to this imbalance, a neural network trained with off-the-shelf loss functions such as cross entropy are ill suited for this fuzzing, because they are prone to both (a)~\textit{Type-I errors} (or false positive errors) and (b)~\textit{Type-II errors} (or false negative errors). The binary cross entropy loss function, is formulated as:
% % {
% % % \setlength{\abovedisplayskip}{0pt}
% % % \setlength{\belowdisplayskip}{0pt}
% % \begin{equation}
% %     \label{eq:xent}
% %     \mathcal{L}  = -\sum_{~\text{edge}}\left[p\cdot log(\hat{p}) + (1 - p)\cdot log(1-\hat{p})\right]
% % \end{equation}
% % }
% % Here, $p\in \{0,1\}$ is the {\em true} edge-invocation value: 1 means the edge was actually taken, and 0 means it was not taken, and $\hat{p}$ indicates the corresponding prediction probability. 
% % 
% % % To illustrate why the above loss function is not suitable for fuzzing, consider the example in \fig{class_imbalance}. Here we highlight two edges labeled \textit{a} and \textit{b}. Edge \textit{a} is invoked 99\% of the times; therefore, wrongly classifying it as 1 for 1\% of the time does not adversely affect the loss in~\eq{xent}. Likewise, edge \textit{b}, a rare edge, is invoked only 1\% of the time and wrongly classifying it as 0 would again not adversely affect the loss in~\eq{xent}. 
% % % %However, the latter miss-classified edges is often among the rarest of edges, and it is precisely these edges that need to be correctly classified for better fuzzing performance. 
% % % However, these miss-classified edges are often important ones that influence fuzzing performances. 
% % % For example, in~\fig{class_imbalance}, edge {\it b} is a rare edge, and we should focus fuzzing towards it, while edge {\it a} is already covered so many times that it might be fine not to cover it any longer. 
% % \ee
% % 
% % \begin{figure}[tbp!]
% %     \centering
% %     \includegraphics[width=\linewidth]{figures/class_imbalance.pdf}
% %     \caption{A typical example of imbalance in edges invoked.}
% %     %\caption{Class Imbalance Example}
% %     \label{fig:class_imbalance}
% % \end{figure}
% % {
% % \setlength{\abovedisplayskip}{0pt}
% % \setlength{\belowdisplayskip}{0pt}
% % \begin{equation*}
% %     \text{Penalty}_\text{edge} = \beta_\text{edge} = \frac{\text{\# times an edge is \textit{not} invoked}}{\text{\# times an edge is invoked}}
% % \end{equation*}
% % With this, we compute the loss as follows:
% % 
% \begin{equation*}
%     \label{eq:adap_ent}
%     \displaystyle
%     \mathcal{L}_{adaptive} = -\sum_{\text{edge}}\left(\beta_\text{edge}\cdot p\cdot log(\hat{p}) + (1 - p)\cdot log(1-\hat{p})\right)
% \end{equation*}
% Here, penalize both false positive (Type I) and false negative (Type II) errors and such that these errors would significantly increase the overall loss. To do this, we introduce a parameter called \textit{penalty} (denoted by $\beta$) to penalize these miss-classification. For each edge, the penalty is the ratio of the number of times it is not invoked over the number of times it is invoked. That is, 

% \setlength{\abovedisplayskip}{0pt}
% \setlength{\belowdisplayskip}{0pt}
% \begin{equation*}
%     \text{Penalty}_\text{edge} = \beta_\text{edge} = \frac{\text{\# times an edge/call-stack is \textit{not} invoked}}{\text{\# times an edge/call-stack is invoked}}
% \end{equation*}

% % For each of the edges, the penalty ($\beta_\text{edge}$) takes 3 possible values:
% % \squishlisttwo
% % \item $\beta_\text{edge}>1$: This means the edge is very rarely invoked. Therefore, we penalize $p\cdot log({\hat{p}})$, representing false negatives (Type II), a lot more.
% % \item $\beta_\text{edge}=1$: This means the edge is invoked and not invoked equal number of times. Here, we penalize both false positives and false negatives equally.
% % \item $\beta_\text{edge}<1$: This means the edge is invoked more often than not. Here, we penalize $(1-p)\cdot log({1 - \hat{p}})$, representing false positives (Type I), a lot more.% \note{RAHUL: Tie this better with gradients}
% % \squishend

% \item \textit{Loss function for regression:} This applies to \softlabel. Recall that, unlike \ec and \ctx, \softlabel measures how close an input was from an edge that was not triggered using a \textit{continuous value} between 0 and 1 used to indicate. Therefore, we use a \textit{mean squared error loss} for this task. The \textit{mean squared error loss} is given by:
% \begin{equation}
% \label{eq:mse_loss}
%     \operatorname{MSE}=\frac{1}{n}\sum_{i=1}^n(Y_i-\hat{Y_i})^2.
% \end{equation}
% \ee

% % Note that, for each edge, $\beta$ is dynamically evaluated\textemdash as fuzzing progresses, a rare edge can become frequent edge and vice-versa and thus, the value of $\beta$ must be evaluated at every round of fuzzing to account for this change. Such adaptiveness is particularly desirable due to fuzzing's online learning setting. Finally, we compute the total loss for our multi-task NN model with $K$ tasks as:
% % \begin{equation*}
% %     \label{eq:adap_total}
% %     \displaystyle
% %     \mathcal{L}_{total} = -\sum_{i=1}^K\alpha_{i}\mathcal{L}_{i} 
% % \end{equation*}
% % This is the weighted sum of the adaptive loss $\mathcal{L}_{i}$ for each individual task.


\subsubsection{Context-sensitive Edge Coverage:~Auxiliary Task 2.~}
\label{sect:ctx}

Edge coverage cannot distinguish between two different test inputs triggering the same edge, but via completely different internal states (\eg, through the same function called from different sites in the program). This distinction is valuable since reaching an edge via a new internal state (\eg, through a new function call site) may trigger a vulnerability hidden deep within the program logic. Augmenting edge coverage with context information regarding internal states of the program may help alleviate this problem~\cite{chen2018angora}.

% sequence of function calls that lead up to the edge would act as a surrogate 

% Encoding the entire path leading up to an edge is impractical. Therefore, we obtain a estimation of program state by reflecting on 
% The same edge reached from two different call sites would have different internal state 

% In our multi-tasking framework, the \ctx ``task'' is trained to predict the mapping between the inputs and the corresponding $call\_trace\_id$s  bitmaps. This can enable us to learn the difference between two inputs in a more granular fashion. For example, an ML model can learn that under certain circumstances, the second input byte (\texttt{input[1]} in~\fig{ctx_eg}) can cause crashes. This information cannot be learned by training to predict for \ec alone since both inputs will have the same edge coverage (as shown in~\fig{ctx_eg_2}).

% In our multi-tasking framework, the \ctx ``task'' is trained to predict the mapping between the inputs and the corresponding $call\_trace\_id$s  bitmaps. This can enable us to learn the difference between two inputs in a more granular fashion. For example, an ML model can learn that under certain circumstances, the second input byte (\texttt{input[1]} in~\fig{ctx_eg}) can cause crashes. This information cannot be learned by training to predict for \ec alone since both inputs will have the same edge coverage (as shown in~\fig{ctx_eg_2}).

% Edge coverage uses an \textit{edge bitmap} to count the number edges triggered by an input. However, it cannot discern between inputs that trigger the same edge, but under different contexts. %These internal states are referred to as a context.
% For example, if calls to the same function appears at different sites in the program, \ec cannot fully distinguish between them. 
\begin{figure}[t!]
    \centering
    % \inputminted[xleftmargin=15pt, numbersep=10pt, linenos=true,fontsize=\small,fontfamily=tt]{c}{code/ctx_eg.c}
    \includegraphics[width=\linewidth]{figures/ctx_eg_code.pdf}
    \vspace{-0.4cm}
    \caption{\small An example C-code to demonstrate the usefulness of using context-sensitive measures. Measures such as \ec will fail to detect a possible bug in \texttt{strncpy($\cdot$)}}
    \label{fig:ctx_eg}
     \vspace{-3mm}
\end{figure}
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.55\linewidth]{figures/ctx_eg.pdf}
    \vspace{-0.4cm}
    \caption{\small The tuple in \ec does not differentiate between the \colorbox{blueish!63}{clean} input and the \colorbox{red!36}{buggy} input, while of \ctx (labeled `Call Ctx') does.}
    \label{fig:ctx_eg_2}
    \vspace{-3mm}
\end{figure}

Consider the example %provided by~\cite{chen2018angora} 
in \fig{ctx_eg}. Here, for an input \texttt{[1, 0]}, the first call to function \texttt{foo()} appears at site \texttt{line 12} and it triggers the if condition (on \texttt{line 2}); the second call to \texttt{foo()} appears on site \texttt{line 14} and it triggers the else condition (on \texttt{line 5}). As far as \ec is concerned, both the edges of the function \texttt{foo()} (on lines 2 and 5) have been explored and any additional inputs will remain uninteresting. However, if we provide a new input say \texttt{[0, 8]}, we would first trigger \texttt{line 5} of \texttt{foo} when it is called from \texttt{line 12}. Then we trigger \texttt{line 2 } of \texttt{foo} from \texttt{line 14} and further cause a buffer overflow at \texttt{line 3} because a 12 bytes string is written into a 8 bytes destination buffer \texttt{buf}. Moveover, the input \texttt{[0, 8]} will not be saved by \ec fuzzer since it triggers no new edges. Frequently called functions (like \texttt{strcmp}) may be quite susceptible such crashes~\cite{Wang2019}. 



In order to overcome this challenge, Chen \etal~\cite{chen2018angora} propose keeping track of the \textit{call stack} in addition to the edge coverage by maintaining tuple: 
% of the \textit{call\_stack}, \textit{prev\_block}, and \textit{cur\_block}, \ie 
$(\textit{call\_stack}, \textit{prev\_block}, \textit{cur\_block})$. \fig{ctx_eg_2} shows the additional information provided by \ctx over \ec. Here, we see an example where a buggy input \colorbox{red!36}{\texttt{[0,8]}} has the exact same edge coverage as the clean input \colorbox{blueish!63}{\texttt{[1,0]}}. However, the call context information can differentiate these two inputs based on the call stacks at \texttt{line 12} and \texttt{14}.

We model \ctx in our framework as an auxiliary task. We first assign a unique id to every call. Next, at run time, when we encounter a call at an edge ($edge\_id$), we first compute a $hash$ to record all the functions on current call stack as: $call\_stack = call\_id_1 \oplus ... \oplus call\_id_n$, 
% In order to instrument \ctx, we first assign a unique id to every call. Next, at run time, when we encounter a call at an edge ($edge\_id$), we first compute the $hash$ value with $\oplus$ to record all the functions on current call stack as below:
% \begin{equation*}
% \label{eq:call_stack}
% \small
% call\_stack = call\_id\_1 \oplus ... \oplus call\_id\_n
% \end{equation*}
where $call\_id\_i$ represents the \inlinemathit{i}-th function on current call stack and $\oplus$ denotes XOR operation. Next, we compute the \textit{context sensitive edge  id} as: $call\_trace\_id = call\_stack \oplus edge\_id$.
% 
%  
% {
%  \setlength{\abovedisplayskip}{0pt}
%  \setlength{\belowdisplayskip}{0pt}
% \begin{equation}
% \label{eq:call_trace}
% call\_trace\_id = call\_stack \oplus edge\_id
% \end{equation}
% }

%Note, the $edge\_id$ denotes the current edge id, as per~\eq{edge_id}. 
%Using \eq{call_trace},
Thus we obtain a unique $call\_trace\_id$ for every function called from different contexts (\ie, call sites). We then create a bit-map of all the $call\_trace\_id$s. Unlike existing implementations of context-sensitive edge coverage~\cite{chen2018angora, Wang2019}, we assign an additional id to each call instruction while maintaining the original $edge\_id$ intact. Thus, the total number of elements in our bit map reduces to sum of $call\_trace\_id$s and $edge\_id$s 
rather than a product of $call\_trace\_id$s and $edge\_id$s. An advantage of our design is that we minimize the bitmap size. In practice, existing methods requires around $7\times$ larger bitmap size than just \ec~\cite{chen2018angora}; our implementation only requires around $1.3\times$ bitmap size of \ec. The smaller bitmap size can avoid edge explosion and improve performance.


In our multi-tasking framework, the \ctx ``task'' is trained to predict the mapping between the inputs and the corresponding $call\_trace\_id$s  bitmaps. This can enable us to learn the difference between two inputs in a more granular fashion. For example, an ML model can learn that under certain circumstances, the second input byte (\texttt{input[1]} in~\fig{ctx_eg}) can cause crashes. This information cannot be learned by training to predict for \ec alone since both inputs will have the same edge coverage (as shown in~\fig{ctx_eg_2}).


% \input{tex/background_fig_1.tex}
\input{body/3_methodology_stage_1}
\input{body/3_methodology_stage-2_2.tex}
% \input{body/3_methodology_stage_2.tex}
\input{body/3_methodology_stage_3.tex}

==> body/3_methodology_stage_2.tex <==
\subsection{Stage-II: Gradient guided mutation}
\label{sect:stage-2}
% \red{
%     \be
%     \item before anything, what is the purpose of this stage
%     \item first establish that the compact layer is better than the task specific layer to obtain hotbytes
%     \item then explain how hotbytes affect the compact layer
%     \item Then introduce gradients a way to measure the extent of impact.
%     \ee
% }

% \red{Version 1 (talks about why not to use task specific decoders last):}~
% This phase uses the trained MTNN to generate new inputs that can maximize the code coverage. This is achieved by focusing mutation on the byte locations in the input that can most influence the branching behavior of the program (\textit{hot-bytes}). 

% We use the the compact embedding layer of the MTNN (shown in \colorbox{greenish}{green} in \fig{bg_fig_1}) to infer the distribution of the hot-bytes. The compact embedding layer is well suited for this because, it captures the most semantically meaningful features (\ie, bytes) in the input in a compact and an interpretable manner. It learns to ignore task specific noise patterns~\cite{kumar2017variational} paying more attention to the important bytes that apply to all tasks~\cite{chen2016, kulkarni2015, Bengio13}.  Note that, we refrain from using the task-specific decoders to infer \textit{hot-bytes} because they tend to offer a localized view of the hot-byte distribution limited to the program regions previously explored by that task.

% \red{Version 2 (talks about why not to use task specific decoders first):}~
This phase uses the trained MTNN to generate new inputs that can maximize the code coverage. This is achieved by focusing mutation on the byte locations in the input that can most influence the branching behavior of the program (\textit{hot-bytes}). Task-specific decoders can't be used to infer \textit{hot-bytes} because they tend to offer a localized view of the hot-byte distribution limited to the program regions previously explored by that task.

We use the the compact embedding layer of the MTNN (shown in \colorbox{greenish!80}{green} in \fig{bg_fig_1}) to infer the distribution of the hot-bytes. The compact embedding layer is well suited for this because it (a)~captures the most semantically meaningful features (\ie, bytes) in the input in a compact and an interpretable manner; and (b)~learns to ignore task specific noise patterns~\cite{kumar2017variational} paying more attention to the important bytes that apply to all tasks~\cite{chen2016, kulkarni2015, Bengio13}.  

% \red{Version 3 (shortest):}~
% This phase uses the trained MTNN to generate new inputs that can maximize the code coverage. This is achieved by focusing mutation on the byte locations in the input that can most influence the branching behavior of the program (\textit{hot-bytes}). 

% We use the the compact embedding layer of the MTNN (shown in \colorbox{greenish}{green} in \fig{bg_fig_1}) to infer the distribution of the hot-bytes. The compact embedding layer is well suited for this because, it captures the most semantically meaningful features (\ie, bytes) in the input in a compact and an interpretable manner. It learns to ignore task specific noise patterns~\cite{kumar2017variational} paying more attention to the important bytes that apply to all tasks~\cite{chen2016, kulkarni2015, Bengio13}.  

% It is not advisable to use the task-specific decoders to infer the \textit{hot-byte} distribution because they tend to offer a localized view of the hot-byte distribution closely tied to the program regions previously explored by the task.



% \red{Version 2:}~
% This phase uses the trained MTNN to generate new inputs that can maximize the code coverage. This can be achieved by focusing mutation on the byte locations in the input that can most influence the branching behavior of the program (\textit{hot-bytes}). 
% We choose to use the compact embedding layer of MTNN (shown in \colorbox{greenish}{green} in \fig{bg_fig_1})

% Gathering hot-byte information from each task can be bad because localized to one task therefore noise and closely tied to a small program region


% Instead we guide the mutations using the feedback the common embedding layer. This will retain the important features only and discard the noise.

% Ignore task specific noise patterns in the compact layer.

% Pay more attention to the important bytes that apply to all tasks. 

% The compact embedding layer of MTNN (shown in \colorbox{greenish}{green} in \fig{bg_fig_1}) is a dense and a feature rich representation of the sparse input space (see \fig{bg_fig_1}). It captures all the semantically meaningful factors in the inputs with a substantially lower number of dimensions, \ie, it contains all the information present in the inputs but in a compact and an interpretable manner~\cite{chen2016, kulkarni2015, Bengio13} while discarding other spurious information~\cite{kumar2017variational}.

Formally, we can represent the input (shown in \colorbox{orangish!80}{orange} in \fig{bg_fig_1}) as a byte vector $xb=\{xb^1, xb^2, ..., xb^n\}\in\mathrm{\left[0, 255\right]^n}$, where $xb^i$ is the $i^{\text{th}}$ byte in $xb$ and $n$ represents the input dimensions (\ie, number of bytes). 
Then, after the MTNN has been trained, we obtain the compact embedding layer $\mathbf{z}=\{z^1, z^2, ..., z^m\}$ consisting of $\mathit{m}$ nodes. Let $f_i(\mathbf{xb})$ denote the function that embeds the input \inlinemathbf{xb} into the $i$-th node $z^i$ in the embedding layer. Then, we may express the compact embedding as follows:
\beq
\label{eq:mapping}
\begin{bmatrix} z^1 \\ z^2 \\ \vdots \\ z^m
\end{bmatrix} = 
\begin{bmatrix} f_1(\mathbf{xb})\\ f_2(\mathbf{xb}) \\ \vdots \\ f_m(\mathbf{xb})\end{bmatrix} = 
\begin{bmatrix} f_1(xb^1, \cdots, xb^n)\\ f_2(xb^1, \cdots, xb^n) \\ \vdots \\ f_q(xb^1, \cdots, xb^n)\end{bmatrix}
\eeq

% In the context of this paper, the input $\mathbf{xb}$ represents a binary file format. Hence, a \textit{feature} refers to the input bytes and each of the $p$ features represents a byte. 

An important property of \eq{mapping} is that, for every byte that changes in $\mathbf{xb}=\{xb^1,...,xb^n\}$, we obtain corresponding changes to every node in $\mathbf{z}=\{z^1, ..., z^m\}$. The extent of the change is determined by how influential each of the $n$ bytes in the input $\mathbf{xb}$ are to all the tasks in the MTNN model. Changes to the \textit{hot-bytes}, which are more influential, will result in \textit{larger} changes to $\mathbf{z}$. This property may be used to discover the \textit{hot-bytes}.% compared to the less influential bytes. % In theory, if we can measure the magnitude of the 

To determine how influential each of the bytes in $\mathbf{xb}$ are, we compute the partial derivatives of the nodes in compact layer with respect to all the input bytes. The partial derivative of the $j$-th node in the embedding layer \inlinemathbf{z} with respect to the \inlinemathit{i}-th byte in the input is given by:
\beq
\label{eq:partial_d}
\nabla_{\mathbf{xb}}~\mathbf{z}=\dfrac{\partial f_j(\mathbf{x})}{xb^i} = \dfrac{\partial z^j}{\partial xb^i}
\eeq
%. Gradient computation is supported by a rich literature on techniques such as \textit{automatic differentiation}~\cite{wengert1964simple,block1991siam,baydin2018automatic}. In this paper, we compute the gradient between the nodes in the compact embedding layer ($\mathbf{z}$) \wrt to the input bytes ($\mathbf{xb}$). 
Since there are \inlinemathit{n} bytes in the input layer \inlinemathbf{xb} and \inlinemathit{m} nodes in the embedding layer, computing the partial derivatives results in the following \textit{Jacobian Matrix}: 
\begin{equation}
    \label{eq:jacobian}
    \mathbb{J}_{m\times n} = \begin{bmatrix}
    \dfrac{\partial {z^1}}{\partial xb^1} & \cdots & \dfrac{\partial {z^1}}{\partial xb^n} \\
    \vdots & \ddots & \vdots\\
    \dfrac{\partial {z^m}}{\partial xb^1} & \cdots & \dfrac{\partial {z^m}}{\partial xb^n} 
\end{bmatrix}  
\end{equation}
The above Jacobian matrix has a dimensionality of $m\times n$. Here, 
\be
\item Every row in the jacobian matrix corresponds to a node in the embedding layer $z^i\in z$. %Since there are $\mathit{m}$ nodes in the embedding layer, the jacod
\item Every column in the jacobian matrix corresponds to an input byte $xb^i\in z$.
\ee
% An element $(i,j)$ in the above matrix represents the gradient of the embedding layer node $z^i$ \wrt the input byte $xb^j$, \ie, \inlinemath{\partial z^i/\partial xb^j}.

In order to infer the importance of each byte $xb^i\in xb$, we compute the sum of every column in \eq{jacobian}. 
% Since there is one column for every input byte, we would obtain  

\begin{equation}
    \label{eq:hot_byte}
    \mathrm{S}(\mathbf{xb}) = \begin{bmatrix}
    \sum_i{\left|\dfrac{\partial z^i}{xb^1}\right|} & \cdots & \sum_i{\left|\dfrac{\partial z^i}{xb^n}\right|} \end{bmatrix} 
    % = \begin{bmatrix}
    % \sum_{i=1}^{p}{\dfrac{\partial \mathbf{z^i}}{\partial xb^1}} & \cdots & \sum_{i=1}^{p}\dfrac{\partial \mathbf{z^i}}{\partial xb^q} \end{bmatrix}  
\end{equation}
Here, $\mathrm{S}(\mathbf{xb})$ is a vector of length $\mathit{n}$. The $i$-th element in $\mathrm{S}(\mathbf{xb})$ represents the sum of all the gradients of the compact-embedding nodes ($\mathbf{z}$) \wrt the  $i$-th input byte $xb^i$.
Note that, 
\bi 
\item The $\mathit{i}^{th}$ element in $\mathrm{S}(\mathbf{xb})$ measures the \textit{average influence} the $\mathit{i}^{th}$ input byte ($xb^i$) has on \textit{all} the nodes in the compact layer. 

\item The numeric value of each of the $\mathit{n}$ elements in $\mathrm{S}(\mathbf{xb})$ determines the hotness of each of the bytes. The larger the value, the more likely it is that the byte is potentially a \textit{hot-byte}.
\ei 

\input{tex/hot_bytes.tex}

Using the \textit{saliency map} ($\mathrm{S}(\mathbf{xb})$) from~\eq{hot_byte} we can now mutate the existing inputs to generate new ones. To do this, we identify the $\mathit{top-k}$ bytes with the largest saliency values as shown below:
\beq
H(k) = arg\left(top_k\left(\mathrm{S}(\mathbf{xb})\right)\right)
\eeq
Here, $H(k)$ represents the byte-locations of the $\mathit{top-k}$ \textit{hot-bytes} that will be mutated by our algorithm. The specifics of the mutation scheme is presented in our pseudocode shown in \fig{pseudo}. 

\input{tex/pseudo.tex}

To demonstrate that this gradient guided mutation is effective at mutating the \textit{hot-byte} location, we inspect the extent of mutation at each byte location is mutated in ELF binaries (see \fig{hotbytes}). We find that the key regions such as \textit{ELF header} and \textit{Section header} are mutated to the greatest extent. Intuitively, this make sense because these regions play a major role in triggering unique program behaviors as compared to other regions. 



==> body/5_evaluation.tex <==
% \section{Evaluation}

% \begin{figure}[tbp!]
%     \centering
%     \includegraphics[width=0.5\linewidth]{figures/edge_cov.jpg}
%     \caption{{\small New edge coverage comparison of NEUZZ++ and NEUZZ}}
% \end{figure}

% 1. normalization of dataset ensures better convergence of NN model, thus we can have more accurate gradient. explain how to perform the normalization by giving a equation. x\_norm = (x\_ori - x\_mean)/x\_std (find more detail in Neutaint paper), then explain briefly why the normalization helps faster convergence. NEUZZ++ (first scale into [0,1], then subtract by mean and divide by standard deviation) VS NEUZZ (just linearly scale byte value from [0, 255] to [0,1])

% 2. adaptive loss function mitigates the imbalance of training data, therefore NN can approximate branching behaviors more accurately and further produce more accurate gradient (i.e., hot bytes). First, explain the imbalance issue is inherent to inputs dataset obtained from fuzzer. The reason is that fuzzer only save a single inputs for a new edge coverage in order to maintain a minimal corpus. For many rare edges, only a single inputs can trigger them while remaining inputs cannot trigger them.--> imbalance dataset. Second, the effect of imbalance dataset, NN learned a biased estimator of branching behaviors even it can fit/converge perfectly. Third, adaptive loss function mitigate it, define a formal equation for weighted loss.

% 3. Better heuristic edge and seed selection guides NEUZZ++ to focus mutating newest inputs whose execution path are on the boundary of current edge coverage, rather than the common inputs whose execution path lie in the center of overall edge coverage. These newest inputs ensures more efficient new/rare edge discovery since their execution path, compared with the common inputs',  are closer to the unexplored edges.  

==> body/_3_0__framework_intro.tex <==

%\input{tex/intro_fig.tex}

In \noindent\tion{theory}, we described a theoretical fuzzing framework, based on NN, that is flexible and that can adaptively incorporate several mutation parameters. In this section, we introduce our tool, \tool, and demonstrate more concretely how this flexibility can be leveraged in a real world scenario. Specifically, we propose mutation parameters to help address three common issues faced by current greybox fuzzers.
\squishlisttwo
\item[1]. \textit{Rare-edges}: We observe that certain edges in the programs control flow graph are rarely invoked. It would be desirable for fuzzing to invoke these edges more often. We show in \tion{offset_selection} how a mutation parameter in the form of adaptive loss can compensate for this to guide fuzzing more towards rare branches. 
\squishend

% The general framework of \tool is shown in~\fig{intro_fig_1}. Here, blocks highlighted in \colorbox{lightgray}{gray} to represent the mutation parameters that we choose to address the common challenges faced by the current state-of-the-art fuzzers. 
% \squishlisttwo
% \squishend




% In \tool, we use a simple NN to approximate the relationship between a provided input (labeled $I$ in \fig{intro_fig_1}) and a numeric value (labeled $P$ in \fig{intro_fig_1}) quantifying how the input affects the \cfg. In \fig{intro_fig_1}, we represent this encoding in a block labeled ``Input selection and encoding''. The encoding is a parameter that controls the mutation There exist several possibilities to encode an input's effect on a program's \cfg. Edge coverage is one such example, other measures such as branch distance metric~\cite{arcuri2010does} may also be used. 

% % -- here if an input invokes a certain edge, it is assigned a value 1 and 0 otherwise. As we shall discuss in \tion{soft_label}, just using edge coverage with either 1 or a 0 may be too coarse an quantification. In some cases, we may opt to include some additional information to such as branch distance metric~\cite{arcuri2010does} that measures how close an input is to invoking an edge. Accordingly, \tool is designed to learn the relationships between inputs and \textit{any representation} of it's effect on a program's \cfg.

% % As shown in~\fig{motivate}, \tool contains an input layer, one intermediate layer, and an output layer. The length of the input layer is the same as the number of bytes in an input, such that each input byte corresponds to one input node. The total number of input nodes is equal to the total number of bytes in the largest input. Note that, the shorter inputs are padded with \texttt{0x00} for consistency. 

% Similarly, each node in the output layer of \tool corresponds to an edge in the \cfg. The  numeric value associated with each node represents the impact of the input for the corresponding edge on the program's \cfg.  The total number of output nodes, therefore, should be equal to the total number of edges in the \cfg see so far. 
% Note that it is difficult to know before hand the exact number of edges in a give program. Thus, we train the network with a set of edges that have been already 
% seen by the training inputs. When new egdes are reached, the output layer is updated accordingly. %and the edges in their vicinity (e.g., the non-taken edges whose guard conditions have been evaluated). 
% % \rahul{say something about branch distance}



==> body/_3_1__motivating_example.tex <==
% \subsection{Motivating Example}
% \label{sect:motivate}


%To demonstrate how fuzzing can be performed with neural networks and first order optimization, in this section, we present a simple contrived example. \fig{motivate}(a) shows a sample source code and the corresponding control-flow graph used for this purpose. 

% In the code, we take as an input an array like object \texttt{x[]}. The program branches conditioned on the value of the \textit{second} element of the input \texttt{x[1]}. We assume that there is a vulnerbility lurking in the code that gets called upon for a very specific value of \texttt{x}, i.e., \texttt{x[1]$\geq$20}. This specific edge (labeled ``c'' in~\fig{motivate}(a)) is highlighted in \colorbox{lightpink}{pink}. The goal of fuzzing is to generate test inputs to somehow reach this vulnerable edge.

%To demonstrate how \tool works, in this section, we present a simple contrived example. 

\subsubsection{Motivating Example.}~
\label{sect:motivate}
\fig{motivate}(a) shows a sample source code and the corresponding \cfg with the edges labeled {\tt a}, {\tt b}, {\tt c}, and {\tt d}(move a to edge, not node). The program takes an array-like object \texttt{x[]} of length 2 as input and branches conditioned on the value of the \textit{second} element of the array \texttt{x[1]}. We assume that there exists a vulnerability along edge {\tt d} (highlighted in \colorbox{lightpink}{pink}), that gets called when \texttt{x[1]$\geq$20}. The goal of fuzzing is to generate test inputs to reach this vulnerable edge.

%Our preferred way to do this is to first construct a neural network which learns to predict for the edges invoked on the \cfg for given inputs. This neural network contains an input layer, one or more intermediate layers, and an output layer. The length of the input layer is the same as the length of the input, i.e., each byte in the input corresponds to one node of the input layer. Similarly, the length of the output layer is equal to the number of branches (in this case, 4).  Given a sample of inputs and the corresponding edges invoked by those inputs, the neural network is trained to model this relationship as accurately as possible. 
First, \tool learns to predict the extent to which edges on the \cfg are affect by the given inputs. For each edge, a value close to 1 represents that the edge is likely to be affected by the input and a value close to 0 represents that the edge is not likely to be affected by the input.
%This NN contains an input layer, one or more intermediate layers, and an output layer. The length of the input layer is the same as the length of the input, i.e., each byte in the input corresponds to one node of the input layer (in this case, 2). Similarly, the length of the output layer is equal to the number of edges (in this case, 4).  
In this example, the NN contains two nodes in the input layer as input contains only 2 bytes and output layer has four neurons as per the \cfg of 
\fig{motivate}(a). We begin with two initial inputs, i.e., (i) Input 1:~\texttt{x=[1,5]} that affects edge \textit{a}~(\texttt{E=[1,0.2,0.15,0.15]}), \ie, $\norm{E}$=1; (ii) Input 2:~\texttt{x=[1,15]} that affects edges \textit{b, d}~(\texttt{E=[0.15,1,1,0.15]}), \ie, $\norm{E}$=1.4. 

These inputs are provided as training data to the \tool so that it may predict for the effect of inputs on the edges as accurately as possible. 
%This trained NN will now represent the surrogate representation of the control-flow graph shown in \fig{motivate}(a). Given an input, it will predict for which edges are invoked in the control-flow graph.  

% The next step is to generate a new input from the seeds. To do this, we compute the gradients from the neural network. Specifically, we compute the gradients of the edge coverage (i.e.,the output layer of the neural network) with respect to the bytes in the input (i.e., input layer of the neural network). These gradients inform us of the extent to which each byte affects the edge coverage. 
Next, to generate a new input from these seeds, we compute the gradients from \tool. Specifically, we compute the gradients of the covered edges (\ie, NN output) \wrt the input bytes (i.e., NN input). These gradients inform us which bytes affect the output and by how much; thus, guiding where to mutate. For example, in \fig{motivate}(a), a change in the value of \texttt{x[1]} from \texttt{5}~to~\texttt{15} will cause the affected edges to change from \texttt{a} to \texttt{b,c}, \ie 2 new edges are affected. 
Therefore, the gradients $\nabla_{\text{\texttt{x[1]}}} = (1.4-1)/(15-5) = 0.4/10 = 0.04$. On the other hand, changes in \texttt{x[0]} does not cause any change in the corresponding edge coverage. Therefore, $\nabla_{\text{\texttt{x[0]}}} = 0$. In summary, the gradient vector obtained will be $\nabla_{\text{\texttt{x}}}  = [0,~0.04]$

%In the case of \fig{motivate}, we notice that a change in the value of \texttt{x[1]} from \texttt{x[1] = 5}~to~\texttt{x[1] = 15} will cause the edge coverage to change from $1$ to $2$. Therefore, the gradients $\nabla~\text{\texttt{x[1]}} = \tfrac{\delta~Y}{\delta~\text{\texttt{x[1]}}} = 0.1$. On the other hand, it can be seen that changes in \texttt{x[0]} does not cause any change in the corresponding edge coverage. Therefore, $\nabla~\text{\texttt{x[0]}} = \tfrac{\delta~Y}{\delta~\text{\texttt{x[0]}}} = 0$. In summary, the gradient vector obtained will be $\nabla~\text{\texttt{x}} = \tfrac{\delta~Y}{\delta~\text{\texttt{x}}} = [0,~0.1]$

After obtaining the gradient vector, we can use it to generate a new input using gradient ascent according to~\eq{eq_7}. We would make no changes to \texttt{x[0]} since it had a zero gradient, and we would increase the value \texttt{x[1]} since it had a positive gradient. Assuming that the step size was sufficiently large, we would now obtain a new seed, say \texttt{[1,~25]}, with this procedure, that would invoke the vulnerable edge {\tt d}. 


==> body/_3_methodology.tex <==
\section{Methodology}
%\section{Gradient Guided Fuzzing with \textsc{NABLA}}
\label{sect:our_method}

%\input{body/3_0__framework_intro.tex}

%\noindent\tion{theory} lays out the basic working principle of \tool. 
This section describes the methodology of \tool in detail. 
~\fig{intro_fig_1} shows a generic workflow. 

\input{tex/motivating_example.tex}

\subsection{Overview}
\label{sect:overview}

\subsubsection{\tool Architecture.}~ We use a feed-forward NN to learn an embedded representation of program inputs and predicts three program behaviors in a multi-task learning fashion. 
%For fuzzing task, each unique coverage metric could affects fuzzer's performance by targeting different program behaviors~\cite{Wang2019Be}. In practice, a fuzzer with combined coverage metric could yield better result than a fuzzer with single coverage metric fuzzer. 
To be specific, our nn models takes in program inputs and encode them into embedded feature vectors. Then we pass these embedded feature vectors into three decoders to predict \circled{1} control flow edges, \circled{2} function call traces and \circled{3} diverging distance from branching point during the dynamic execution of tested program. Given a specified test input, the multi-task NN model can learn to predict various dynamic program behaviors at the same time.
%Thus, we choose three coverage metrics (\ie \circled{1} edge coverage, \circled{2} function call context coverage and \circled{3} distance-aware edge coverage) and train a NN model to learn these metrics in a multiple-task learning fashion. \tool takes test input bytes ($I$) as input and outputs three set of labels indicating either a unique edge, a unique function call trace or a unique branch is covered, respectively. 
%We will explain the detail for each task in the later section. Accordingly, \tool is designed to learn the relationships between inputs and \textit{any representation} of its effect on various program's behaviors. 
\begin{comment}
model the probability of \cfg edges being invoked based on the test inputs and use the NN to decide the mutation parameters, as shown in~\eq{formal_main}. 
\tool takes test input bytes ($I$) as input and numeric values ($P$) quantifying how the input affects the \cfg edges as output. There are several possible ways to quantify an input's effect on a program's \cfg. Edge coverage is one such example-- here if an input invokes a certain edge, it is assigned a value 1 and 0 otherwise. As we shall discuss in \tion{soft_label}, just using edge coverage with either 1 or a 0 may be too coarse an quantification. In some cases, we may opt to include some additional information like branch distance metric~\cite{arcuri2010does} that measures how close an input is to invoking an edge. Such information can be encoded using ``Encoding" function. 
Accordingly, \tool is designed to learn the relationships between inputs and \textit{any representation} of it's effect on a program's \cfg. Moreover, \tool also supports custom input selection functions as shown in~\eq{formal_main} to customize the order of the inputs to be mutated.
\end{comment}

%where all these strategies can be incorporated as configurable parameters. For example, inputs $I$ and corresponding output labels ($P$) are selected by Input Selection and Encoding step. An user can choose to encode the information source that she wants to target for fuzzing strategy. 
%$\beta$ is also another configurable parameter in loss function to control the learning rate. The whole network is optimized with gradients $\nabla$.

% We use a simple NN to approximate fuzzing algorithm, as shown in~\eq{formal_main}. 
% Users can provide an input format alf's optimization strategy as shown in  relationship between a provided input and a numeric value quantifying how the input affects the \cfg. There exist several possibilities to quantify an input's effect on a program's \cfg. Edge coverage is one such example-- here if an input invokes a certain edge, it is assigned a value 1 and 0 otherwise. As we shall discuss in \tion{soft_label}, just using edge coverage with either 1 or a 0 may be too coarse an quantification. In some cases, we may opt to include some additional information to such as branch distance metric~\cite{arcuri2010does} that measures how close an input is to invoking an edge. Accordingly, \tool is designed to learn the relationships between inputs and \textit{any representation} of it's effect on a program's \cfg.

%As shown in~\fig{intro_fig_1}, \tool contains an input layer, potentially several intermediate layers, and an output layer. The length of the input layer is the same as the number of bytes in an input,
%such that each input byte corresponds to one input node.
%The total number of input nodes is equal to the total number of bytes in the largest input. Note that, the shorter inputs are padded with \texttt{0x00} for consistency. 

As shown in~\fig{intro_fig_1}, each input byte corresponds to one input node in \tool. Therefore, the total number of input nodes is equal to the total number of bytes in the largest input and the shorter inputs are padded with \texttt{0x00} for consistency. Similarly, each node in the output layer of \tool corresponds to a control flow edge, a function call trace, or a diverging distance to an edge depending on different decoders. The numeric value associated with each node represents the impact of the input for the corresponding program behaviors. %edge on the program's \cfg.  %The total number of output nodes, therefore, should be equal to the total number of edges in the \cfg seen so far. 
%Note that it is difficult to know before hand the exact number of edges in a give program. Thus, we train the network with a set of edges that have been already 
%seen by the training inputs. When new edges are reached, the output layer is updated accordingly. %and the edges in their vicinity (e.g., the non-taken edges whose guard conditions have been evaluated). 
% \rahul{say something about branch distance}

The network is trained using a weighted sum of loss functions over all individual tasks with parameter $\beta$ that is configurable by the user to control the weight between different tasks. We also include another parameter $\alpha$ in the loss function to adaptively change the class weight for positive and negative samples in order to mitigate the issue of imbalanced dataset. 
%For instance, we show in \tion{offset_selection} that by appropriately setting $\beta$, we can train the NN to learn the relationships between the inputs and the rare edges in the \cfg. 
\tool computes the gradients $\nabla$ of the outputs \wrt the inputs to guide fuzzer to generate more inputs that explore unseen edges.

In the rest of this section, we first describe three tasks (coverage metrics) learnt simultaneously by our NN model and then illustrate \tool's methodology using a simple motivating example. Finally we explain the adaptive loss and prioritized seed selection.
%strategies that we implemented using \tool to show its applicability for real-world programs. 

\subsubsection{Coverage Metrics.}~
\label{sect:cover}
\note{ Dongdong: focus on multiple tasks, not coverage metric. Our contribution is to extract different information from dynamic execution for training. Do we need to add implementation detail like how to instrument the call instruction and distance-aware edge?}


\noindent\textbf{Edge Coverage.} Edge coverage is a common metric used by almost all fuzzers. In this metric, each basic block of the tested program is assigned an unique id. The control flow edges are tracked by computing a hash value over the basic block transitions defined as a tuple ($prev\_block$, $cur\_block$), where $prev\_block$ denotes the id of the previously visited basic block and $cur\_block$ denotes the id for the currently visited basic block. The edge id is computed as:
\begin{equation}
\label{eq:edge_id}
edge\_id = (prev\_block>>1) \oplus cur\_block
\end{equation}  
Edge coverage measures program execution states at runtime through recording a set of control flow edges. Although its simplicity and effectiveness in practice, it misses several other factors of program states (\eg function call stack, memory access, sequences of past edges and reachability of branching points). Afl-sensitive~\cite{Wang2019Be} shows memory-access-aware coverage and sequences of past edges coverage(\ie N-gram edge coverage) could have seed explosion on large complex programs. Therefore, we choose two novel coverage metrics -- function call trace coverage and distance-aware edge coverage to track function call trace and reachability of branching points. These two coverage metrics, along with edge coverage, enable \tool to measure program states in three different granularities.    

\noindent\textbf{Function Call Trace Coverage.} A function invoked from different calling sites or call traces indicates different program state. But for edge coverage metric, these different states are considered as same since no new edge is found. Angora~\cite{chen2018angora} proposes to solve this problem by incorporating call trace into every edge id computation. A major limitation of their method is edge id explosion (around $7.1$X total edge ids compared to common edge coverage metric). Moreover, the larger edge id incurs additional runtime overhead to maintain such large edge hashmap because it cannot fit into CPU cache anymore. 

Our solution is to record unique call trace ids for every \emph{call instruction}, rather than every edge. We check call trace for each call instruction executed during runtime and record all unique call trace states. Like edge coverage metric, we first assign a unique id to every call instruction. Then we compute a corresponding hash value to record all the functions on current call stack. Finally, the call trace id is computed over the tuple ($call\_stack$, $edge\_id$). The call stack hash value \emph{call\_stack} is formally defined as follows:
\begin{equation}
\label{eq:call_stack}
call\_stack = (call\_id_1 \oplus ... \oplus call\_id_n)
\end{equation}
, where $call\_id_n$ represent n function call ids on current call stack. Then we define call trace id $call\_trace$ as:
\begin{equation}
\label{eq:call_trace}
call\_trace = call\_stack \oplus edge\_id
\end{equation}
$edge\_id$ denotes the current edge id defined in equation ~\ref{eq:edge_id}.

\begin{figure}[]
    \includegraphics[scale=0.07]{figures/call_cov.jpg}
    \caption{Call trace coverage VS context-sensitive edge coverage.}
    \label{fig:call_trace}
\end{figure}
Fig~\ref{fig:call_trace} shows a simple code snippet and its corresponding function call trace coverage. Function $a()$ includes four control flow edges. Inside function $main()$, there are $2$ unique calling sites for function $a()$, shown in line 10 $a_1()$ and line 12  $a_2()$. Additionally, there is a unique call trace to reach function $a()$ in line 11 $b() \rightarrow a_3()$. Hence, function call trace coverage generates $3$ corresponding call traces for function $a()$. As shown in the call trace hashtable, function call trace coverage only uses 3 slots to distinguish the same function invoked from different calling sites or from different calling traces. On the contrary, context-sensitive edge coverage need to make a copy of all edge slots for the function $a()$ each time it encounters a new call trace. In the end, context-sensitive coverage requires $12=4*3$ slots to distinguish different call traces. Compared with context-sensitive edge coverage, call trace coverage can measure different call traces with minimal overhead. Moreover, the smaller number of call trace features generated by call trace coverage is more suitable to \tool because the NN model can converge better when learning from less number of features.

\noindent\textbf{Distance-Aware Edge Coverage.} In common edge coverage metric, a control flow edge is marked as 1 if it is taken during runtime or 0 if not taken. When an edge is marked as 0, edge coverage fails to capture the distance between the targeted edge and the edge where actual execution path diverge from the targeted edge. The distance is defined as $approach\ level$ to measure how far the execution path of a test input diverge from the target edge~\cite{Phil2004Hyber}. 
For example, assume our targeted edge is the edge $d$ shown in Fig~\ref{fig:motivate} (a). The aim is to generate inputs reaching edge $d$ and further trigger the vulnerability. Input $x[1]=10$ exercises the first condition at line 2, but fails to reach the second condition at line 4 guarding the vulnerability code. The $approach\ level$ of input $x[1]=10$ is the distance (\ie number of edges) from the targeted edge $d$ to the diverging edge $a$ (\ie 1). Input $x[1]=20$ exercises both conditions at line 2 and 4 but fails to satisfy the final conditions leading to the edge $d$. The $approach\ level$ of input $x[1]=20$ is 0 since the distance between the targeted edge $d$ and the diverging edge $c$ is 0. Obviously, input $x[1]=20$ is a more promising seed to mutate than input $x[1]=10$ because it is nearer to the vulnerability. Nevertheless, both of them are marked with label 0 and treated equally by edge coverage. To include $approach\ level$ into edge coverage, we propose a novel distance-aware edge coverage metric defined as follows: 
\begin{equation}
\label{eq:dist_edge}
dist\_edge=
    \begin{cases}
    1, & \text{if the edge is taken} \\ 
    \beta, & \text{if}\ approach\ level =0 \\
    0, & \text{if} \ approach\ level >0\\
\end{cases}
\end{equation}
When the edge is taken, distance-aware edge is same with vanilla edge coverage. If the edge is not taken and its $approach\ level$ equals 0, we set it as $\beta$ (a constant float number between 0 and 1) to indicate the input reaches the nearest branching point but fails to satisfy the condition. If the edge is not taken and its $approach\ level$ great than 0, we set it as 0 which means the input doesn't reach the nearest branching point at all.     





\input{body/3_1__motivating_example.tex}




% \input{tex/pseudo.tex}
%\subsubsection{Approach.}~
%To perform fuzzing, we first train \tool with an initial set of valid seed inputs obtained by running AFL for 1 hour.
%\tool is trained to take some inputs and predicts for the corresponding covered edges (using edge-coverage encoding).
%The training phase of the NN is dictated by an  adaptive loss function discussed in~\tion{offset_selection}. After training the neural network, we obtain gradients of the output layer of the NN (representing edge coverage) \wrt the input layer (representing the bytes in the inputs) as described in~\eq{eq_5}. This can be done quite easily with the help of automatic differentiation~\cite{wengert1964simple,block1991siam,baydin2018automatic}. The gradients obtained above are represented as a vector of length equal to that of the input layer, i.e., for each byte in the input layer, there exists a gradient value. The magnitude of the gradients and the step size (~\eq{eq_7}) determine how much a byte will be mutated. Next, from all the new inputs generated after mutation, we retain the most important inputs for the next round based on importance sampling strategy (\tion{seed_selection}). 
%The above steps are repeated iteratively until the allocated resources for fuzzing have been exceeded. \tool uses a user provided mutation budget as a criteria for determining available budget.

% To perform fuzzing, \tool follows the key steps listed below.

% \noindent
% \mybullet\textbf{Step 1: Initialization}: Similar to existing \gf, \tool starts with an initial set of seed inputs. This is obtained by running AFL for 1 hour and saving the valid inputs. The number of initial inputs vary from 2000 to 5000 depending on the program. These inputs would be used to train \tool, compute the gradients, and generate new test inputs.

% \noindent
% \mybullet\textbf{Step 2: Mutation location selection}: In this step, we first train a neural network model (NN) which takes in the sampled inputs and predicts for the corresponding covered edges. The training phase of the NN is dictated by an  adaptive loss function discussed in~\tion{offset_selection}. After training the neural network, we obtain gradients of the output layer of the NN (representing edge coverage) \wrt the input layer (representing the bytes in the inputs) as described in~\eq{eq_5}. This can be done quite easily with the help of automatic differentiation~\cite{wengert1964simple,block1991siam,baydin2018automatic}. The gradients obtained above are represented as a vector of length equal to that of the input layer, i.e., for each byte in the input layer, there exists a gradient value. The magnitude of the gradients will determine how likely each byte is to impact the edge coverage. 

% % We will select byte locations with top gradient values for further mutations\rahul{may need to elaborate}.

% \noindent
% \mybullet\textbf{Step 3: Mutation operation selection}:
% Next, we mutate the inputs with using gradient ascent is accordance with~\eq{eq_7} . For each byte in the input, we mutate the byte based on the value of the gradient. The extent of mutation is controlled by the step size. Note that, if the gradient for a specific byte location is zero, there would be no change at that byte location. 

% \noindent
% \mybullet\textbf{Step 4: Input selection}: Finally, from among of all generated inputs, we retain a sample of the most important inputs for the next round. This step realizes $xb\in C(\mathcal{X})$ of~\eq{eq_8}. \tion{seed_selection} discusses our sampling strategy in detail. 
% %For each input, we represent the edge coverage as an array of 1's and 0's with 1's representing edges that are taken and 0's representing the edges that are not taken. 

% \noindent
% \mybullet\textbf{Step 5: Repeat until budget is available}: Steps 2 to 4 are repeated iteratively until the allocated resources for fuzzing have been exceeded. \tool uses a user provided mutation budget as a criteria for determining available budget.

% The framework of \tool described above is flexible in that it allows for us to easily incorporate several mutation strategies to enhance each of the above steps. These mutation strategies improve the overall performance of \tool. The rest of the section discusses how these mutation strategies are incorporated into \tool.

%on different information sources that we adapted to implement these steps to improve \tool's performance. 

%\subsection{Incorporating Heuristics}
\subsection{Mutation Strategies}

\note{need a consistent word like "feature" or "program behaviors" to replace "edge" since each output node may belongs to different task. Equations are updated.}
\subsubsection{Adaptive loss for multi-task model}\hfill\\
\label{sect:offset_selection}
In our framework, edge coverage is represented by a Boolean array where each array-index represents an edge in the \cfg. If an input invokes an edge the corresponding index location contains a `1' and a `0' otherwise. We maintain such an array for each input. Since \tool tries to predict the edge-coverage, each node of the output layer would correspond to an edge
%(\ie an array index).  
If a node outputs value close to 1, 
\tool predicts that the corresponding edge will be invoked. Likewise, a value close to 0 would indicate that the corresponding edge will not be invoked. Such NN can be viewed as being trained as a multi-class classifier with each edge representing a class. %, and the number of classes is the same as the total number of edges in a program's \cfg.

% 
% 

%After obtaining a sample of the most important inputs, we train a neural network that predicts for the edge coverage. 
% In our framework, the edge coverage is represented by a Boolean array where each index of that array corresponds to an edge in the control-flow graph. For each input, if an edge is invoked, that index location contains a `1' and a `0' if it is not invoked. %It is worth noting that this neural network can be viewed as being trained for a multi-class classification task where each class represents an edge and the number of classes is the same as the total number of edges in a program's control-flow graph.
% Since edge-coverage is modeled as the output of the NN, the output layer of the NN returns values in the range of 0 to 1. Each node on the output layer corresponds on an edge and a value close to 1 would indicate that it predicts for the edge corresponding that node will be invoked. Likewise, a value close to 0 would indicate a prediction that the edge corresponding that node will not be invoked.

To classify the edges accurately, we must define a \textit{loss function}. 
However, defining a loss-function for edge-coverage turns out to be non-trivial, as their invocations are highly imbalanced: some edges are invoked very often (\ie mostly 1 value),  while some other edges are invoked rarely (\ie mostly 0 value). The problem aggravates as  fuzzing progresses and we keep discovering new edges that have never been invoked before. Due to such imbalance, a NN trained with off-the-shelf loss functions such as cross entropy (\eq{xent}) is ill suited for fuzzing, because they are prone to both (a)~\textit{Type-I errors} (or false positive errors) and (b)~\textit{Type-II errors} (or false negative errors). The binary cross entropy loss function, is formulated as:
%p is a binary value. 1 means the edge was actually taken, 0 means it was not taken.
% In order to classify the edges accurately, we must define a \textit{loss function}. 
% A program's edge coverage is subject to a number of peculiarities. Specifically, we find that while some edges are invoked very often, some other edges are invoked very rarely. This is especially true for new inputs that invoke edges that have never been invoked before. Due to this imbalance, a neural network trained with off-the-shelf loss functions such as cross entropy are ill suited for this fuzzing, because they are prone to both (a)~\textit{Type-I errors} (or false positive errors) and (b)~\textit{Type-II errors} (or false negative errors). The binary cross entropy loss function, is formulated as:
{
% \setlength{\abovedisplayskip}{0pt}
% \setlength{\belowdisplayskip}{0pt}
\begin{equation}
    \label{eq:xent}
    \mathcal{L}  = -\sum_{~\text{edge}}\left[p\cdot log(\hat{p}) + (1 - p)\cdot log(1-\hat{p})\right]
\end{equation}
}
Here, $p\in \{0,1\}$ is the {\em true} edge-invocation value: 1 means the edge was actually taken, and 0 means it was not taken, and $\hat{p}$ indicates the corresponding prediction probability. 

To illustrate why the above loss function is not suitable for fuzzing, consider the example in \fig{class_imbalance}. Here we highlight two edges labeled \textit{a} and \textit{b}. Edge \textit{a} is invoked 99\% of the times; therefore, wrongly classifying it as 1 for 1\% of the time does not adversely affect the loss in~\eq{xent}. Likewise, edge \textit{b}, a rare edge, is invoked only 1\% of the time and wrongly classifying it as 0 would again not adversely affect the loss in~\eq{xent}. 
%However, the latter miss-classified edges is often among the rarest of edges, and it is precisely these edges that need to be correctly classified for better fuzzing performance. 
However, these miss-classified edges are often important ones that influence fuzzing performances. 
For example, in~\fig{class_imbalance}, edge {\it b} is a rare edge, and we should focus fuzzing towards it, while edge {\it a} is already covered so many times that it might be fine not to cover it any longer. 

\begin{figure}[tbp!]
    \centering
    \includegraphics[width=\linewidth]{figures/class_imbalance.pdf}
    \caption{A typical example of imbalance in edges invoked.}
    %\caption{Class Imbalance Example}
    \label{fig:class_imbalance}
\end{figure}

In order to accurately train a NN, we ought to mitigate for these errors. For this, we must penalize both false positive (Type I) and false negative (Type II) errors and modify the loss function accordingly so that these errors would significantly increase the loss. To do this, we introduce a parameter called \textit{penalty} (denoted by $\beta$) to penalize miss-classification. For each edge, the penalty is the ratio of the number of times it is not invoked over the number of times it is invoked. That is, 
{
\setlength{\abovedisplayskip}{0pt}
\setlength{\belowdisplayskip}{0pt}
\begin{equation*}
    \text{Penalty}_\text{edge} = \beta_\text{edge} = \frac{\text{\# times an edge is \textit{not} invoked}}{\text{\# times an edge is invoked}}
\end{equation*}
With this, we compute the loss as follows:
\begin{equation*}
    \label{eq:adap_ent}
    \displaystyle
    \mathcal{L}_{adaptive} = -\sum_{\text{edge}}\left(\beta_\text{edge}\cdot p\cdot log(\hat{p}) + (1 - p)\cdot log(1-\hat{p})\right)
\end{equation*}
}
For each of the edges, the penalty ($\beta_\text{edge}$) takes 3 possible values:
\squishlisttwo
\item $\beta_\text{edge}>1$: This means the edge is very rarely invoked. Therefore, we penalize $p\cdot log({\hat{p}})$, representing false negatives (Type II), a lot more.
\item $\beta_\text{edge}=1$: This means the edge is invoked and not invoked equal number of times. Here, we penalize both false positives and false negatives equally.
\item $\beta_\text{edge}<1$: This means the edge is invoked more often than not. Here, we penalize $(1-p)\cdot log({1 - \hat{p}})$, representing false positives (Type I), a lot more.% \note{RAHUL: Tie this better with gradients}
\squishend

Note that, for each edge, $\beta$ is dynamically evaluated\textemdash as fuzzing progresses, a rare edge can become frequent edge and vice-versa and thus, the value of $\beta$ must be evaluated at every round of fuzzing to account for this change. Such adaptiveness is particularly desirable due to fuzzing's online learning setting. Finally, we compute the total loss for our multi-task NN model with $K$ tasks as:
\begin{equation*}
    \label{eq:adap_total}
    \displaystyle
    \mathcal{L}_{total} = -\sum_{i=1}^K\alpha_{i}\mathcal{L}_{i} 
\end{equation*}
This is the weighted sum of the adaptive loss $\mathcal{L}_{i}$ for each individual task.
% \subsubsection{Mutation operation selection with gradient ascent}\hfill\\
% \label{sect:opertaion_selection}

\subsubsection{Input selection with importance sampling}\hfill
\label{sect:seed_selection}

As discussed in \tion{theory}, sampling inputs is an important step as the choice of inputs can significantly affect the fuzzing performance. 
Also, as fuzzing progresses, the pool of available inputs keeps growing in size. Without some form of sampling strategy, training the NN and computing gradients would take prohibitively long. 

To this end, we propose an importance sampling~\cite{mcbook} strategy where inputs are sampled such that they reach some {\em important region} of the \cfg instead of randomly sampling from available input. In particular, our sampling strategy first retains all inputs that invoke previously unseen edges. Then, we sort the remaining inputs based on how many 
rare edges they have triggered. Note that an edge is considered rare if it is invoked least often by the available seeds. We reason that, by selecting the inputs that invoke the rare edges, we may explore deeper regions of the program on subsequent mutations. In order to limit the number of inputs sampled, we introduce a sampling budget that determines how many inputs will be selected per iteration.  
% We propose an importance sampling~\cite{mcbook} for the input selection where the inputs are selected based on the following considerations:
% \squishlisttwo
% \item Sampling budget determines how many inputs can be retained.
% \item Some edges in the control-flow graphs are invoked very rarely 
% \item We would like guide the fuzzing towards invoking these rare edges more often to ensure that the new inputs will explore deeper regions of the program.
% \squishend
%
% . The pseudocode in \protect\fig{seed_selection} highlights our importance sampling strategy. To determine the importance of an input, we note following considerations:
% \squishlisttwo
% \item Sampling budget determines how many inputs can be retained.
% \item Some edges in the control-flow graphs are invoked very rarely 
% \item We would like guide the fuzzing towards invoking these rare edges more often to ensure that the new inputs will explore deeper regions of the program.
% \squishend
%
% 
% 

We illustrate our seed selection approach with a simple example, consider the \fig{seed_select_example}. 
\begin{figure}
\centering
\begin{subfigure}{\linewidth}
    \begin{center}
        \resizebox{0.5\linewidth}{!}{
        \begin{tabular}{r|l|l|l|l}
            & A    & B    & C    & D\textsubscript{NEW}    \\ \hline
            Input 1    & 1    & 0    & 1    & 0     \\ 
            Input 2    & 1    & 0    & 0    & 0     \\
            Input 3    & 1    & 1    & 1    & 0     \\
            New Input    & 0    & 1    & 1    & 1 \\\hline
            Frequency & 75\% & 50\% & 75\% & 25\%
        \end{tabular}}\\[0.5em]
        Sorted edges=$\{D_{new}, B, A, C\}$\\
        Sorted inputs=$\{\text{\textit{~New Input, Input~3, Input~1, Input~2~}\}}$
    \end{center}
    % \caption{A example of seed selection with importance sampling.}
    % \label{fig:seed_select_example}
\end{subfigure}%\\[0.2em]
% \begin{minipage}{0.7\linewidth}
% \begin{subfigure}{\linewidth}
% \inputminted[numbersep=5pt, linenos=true, fontsize=\small]{python}{code/seed_select.py}
% \caption{Pseudocode for seed selection.}
% \label{fig:seed_selection_pseudo}    
% \end{subfigure}\\[0.2em]
% \end{minipage}
\caption{A example of seed selection with importance sampling.}%.Seed selection with importance sampling}
\label{fig:seed_select_example}    
\end{figure}
Here, we have 4 inputs: \textit{Input 1, Input 2, Input 3}, and \textit{New Input}, where \textit{New Input} is an input that was generated by \tool. Let us also assume that there are 4 edges in the \cfg labeled \textit{A, B, C,} and \textit{D\textsubscript{NEW}}, where \textit{D\textsubscript{NEW}} is a new edge invoked by \textit{New Input}. The last row measures the frequency of the edges. Sorting the edges of \fig{seed_select_example} gives us the order: $\{D_{NEW}, B, A, C\}$, sorted by new edge followed by rare edge and then others.

% The pseudo code in \protect\fig{seed_selection}b highlights our importance sampling strategy. Here, we first sort the inputs by recency from most recently generated input to the least recently generated input (line 10). Then, the edges invoked by those inputs are sorted by rarity from most-to-least rare (line 13). Note, edges such as $D_{NEW}$ in the example of \fig{seed_select_example}, that are invoked by for the first time by newly generated input $\text{New Input}$  will be selected first. Next, contingent on the budget, we loop through each of the remaining inputs (\protect\fig{seed_selection}(b), line 13 onward). We first keep the inputs that invoke the rarest edge. Then, if more budget is available, we keep inputs that invoke the next rarest edge and so on until the budget is exhausted (\protect\fig{seed_selection}(b), line 15). \rahul{[FIXED] the pseudocode is a bit problematic.}


\subsubsection{Soft-labeling with Branch Distance}\hfill
\label{sect:soft_label}
%\input{tex/soft_label.tex}
In \gf, it is a well established practice to generate test inputs based on edge-coverage-based feedback. 
%It is reasoned that, by maximizing edge coverage one can inspect wider regions of code thereby maximizing the likelihood of discovering hidden bugs or vulnerabilities. 
However, often certain regions of code (or edges in \cfg) are very hard to reach with coverage information alone.  

To illustrate such situations, consider a predicate, \ie, branch condition {\tt a$<$10000}; if evaluated to be {\tt True}, branch $X$ is taken, otherwise branch $Y$ is taken (which, say, contains a vulnerability). However, it is very difficult for a fuzzer to reach the vulnerable branch $Y$ starting from an input that sets a to say $a=2$. In order to trigger edge $Y$ the fuzzer must set $a$ to be larger than $10000$ which is hard to do with edge-coverage-based feedback alone as the predicate is unknown to the fuzzer.  

In order to overcome this issue, a popular heuristic used in search-based software engineering is called \textit{Branch Distance}~\cite{arcuri2010does, mcminn2004search}, which computes how far an input is from the predicate value, \ie 10000 here, and use it to guide the search process. Thus, for input $a=1$, the branch distance will be $9999$. As the input value changes, say from 1 to 3, the branch distance will change (i.e., from $9999$ to $9997$) even though the edge coverage does not change. Such branch distance heuristic generalizes to a wide variety of predicates~\cite{arcuri2010does}. 

%To illustrate such situations, consider the example presented in~\fig{soft_label}. Here, we have a very simple function called \texttt{foo}, which takes an input \texttt{a}. Depending on the value of \texttt{a}, the program takes one of two edges (labeled \textit{X} and \textit{Y} in the \cfg of~\fig{soft_label}). Beyond a specific value of \texttt{a} (\texttt{a>=10000}), the program takes the branch \textit{Y}, in all other cases it would take \textit{X}. If we were to compute edge coverage, we find that it would always be equal to 1 because one of the two branches are always taken. In the example of~\fig{soft_label}, we intend to reach the branch \textit{Y} since there is a vulnerability in that branch. However, edge coverage is quite uninformative for this purpose since it does not distinguish between the branches. Specifically, in case of \tool, since the edge coverage is always the same, the computed gradients are always zero as shown in~\fig{soft_label} and therefore it is not possible to guide \tool to prefer one branch over the other.
% \input{tex/branch_distance_table.tex}

%In order to overcome this issue, we seek an alternative to edge coverage. Specifically, we require a heuristic that can quantify how far a given input is from reaching a desired edge. A popular heuristic used in search-based software engineering, known as \textit{Branch Distance}, is best suited for this purpose~\cite{arcuri2010does, mcminn2004search}. To understand branch distance, we first define the term predicate. A predicate is a conditional statement that determines which edge in the control-flow graph will be taken. Given two possible edges arising at a conditional statement, if the predicate is \texttt{True}, then we take one edge and if the predicate is \texttt{False} we would take the other edge. For example in \textit{line 2} of the pseudocode in~\fig{soft_label}, the predicate would be \texttt{a < 10000}. Here, if the predicate is \texttt{True}, i.e., \texttt{a < 10000}, then we choose the edge \textit{X}; otherwise, if the predicate is \texttt{False}, i.e., \texttt{a $\geq$ 10000}, then we choose the edge \textit{Y}. The branch distance heuristic generalizes to a wide variety of predicates~\cite{arcuri2010does}. 

%For the example in~\fig{soft_label}, 
In the mutation strategy, we may replace edge coverage with branch distance as our information source. %computed in accordance to~\tab{branch_distance_table}\rahul{[COMMENTED OUT] [MAYBE REMOVE?] where is this table?}. 
In contrast to edge coverage which stays constant at 1 for all values of \texttt{a=0...10000}, the branch distance decreases monotonically (in this particular case) as \texttt{a} goes from \texttt{a=0} to \texttt{a=10000}. Such changes allow us to compute gradient to guide the mutations towards reaching the remote branch \textit{Y}.






==> body/case_study.tex <==
% % \section{Case Study}
% % \label{sect:case_study}
% \begin{figure}[t!]
%     \centering
%     \inputminted[xleftmargin=15pt, numbersep=10pt, linenos=true,fontsize=\small,fontfamily=tt]{c}{code/pdf_bug.c}
%     \caption{Heap overflow bug in \texttt{mupdf}}
%     \label{fig:pdf_bug}
% \end{figure}
% In this section, we analyze a new heap-overflow vulnerability exclusively found by \tool. Fig~\ref{fig:pdf_bug} shows a function in \texttt{mupdf} that allocates memory for each objects of a pdf file and fill content to these memory chunks. At \texttt{line 6}, it first tries to obtain the total number of objects by reading a field value \texttt{xref->num\_objects} which is controlled by program input--a pdf file. \tool can leverage gradient to identify the hot bytes which control \texttt{xref->num\_objects} and further set it with a negative value. As a result, \texttt{num} maintains its initial value $1$. Then, at \texttt{line 10}, the function allocates memory space for a single object. However, in \texttt{line 14}, it tries to fill more than one objects to \texttt{new\_sub->table} and causes a heap overflow. 


==> body/formalization_bck.tex <==
\section{Problem Formalization}% and Motivation}
% \be
% \item (Optional) Add a terminologies section \note{(to be deleted)}
% \item Explain fuzzing in detail
% \item Fuzzing is an optimization problem \note{(move to section 3)}
% \item Add a block diagram with a simple example \note{(move to section 2.1)}
% \item Pivot to gray box fuzzing
% \bi
% \item "Hot-bytes" --> Taintscope 2010 and Angora
% \item "Rare-Edges" --> FairFuzz and masking bytes
% \item "Branch-Distance" --> Acruri 2013 and SBSE
% \ei
% \item Deep learning and universal approx with bounded discontinuous functions. Cite universal approximation with k-lipschitz functions paper. \note{(move to the intro section)}
% \ee,4.
% \subsection{Traditional Greybox Fuzzing}
% \subsection{Fuzzing as an Optimization Problem} 

% In this paper, 
%Given an input to a {program under test} we study which of the edges in the programs control-flow graph are exercised by that input through light instrumentation. The objective is to generate inputs such that the number of edges triggered in the control-flow graph by the inputs is maximized.

% The goal of fuzzing is to explore the program input space to maximize the number of detected bugs. Since it is hard to predict the bug locations,  typical \textit{greybox fuzzers} (\GF) tries to maximize the edge coverage instead, which is a well-defined metric.  
% Thus, GF can be thought of a search optimization problem, where it search over the entire input space with the aim of optimizing edge coverage. 
% However, the input space is typically large; thus, exhaustive search  is not feasible. Instead, one needs to identify and focus the search in promising region\textemdash evolutionary optimization technique is a standard practice to achieve this goal. To exhaustively search, most of the evolutionary fuzzers use random mutations.  


% Typically, such coverage guided greybox fuzzing explores the input space through mutation\textemdash starting from a set of random seed inputs, it generates new inputs through mutations that are more likely to cover unexplored edges. The genetic algorithm (GA) based evolutionary search strategy is a popular technique to generate these mutants, where GA picks those inputs that increase edge coverage and generate new mutants through corss-over and mutation operations. The success of a greybox fuzzer typically depends on (i) \textit{Initial seeds} that will start the edge exploration and dictate the creation of subsequent mutants; (ii) \textit{Mutation location}, i.e., which byte location (offset) will be mutated, and (iii) \textit{Mutation operator} that determines the mutation operation to perform on those byte locations. 
The goal of fuzzing is to explore the program input space to maximize the number of detected bugs. Since it is often hard to know the bug locations a priory, typical \textit{greybox fuzzers} (\GF) tries to maximize the edge coverage instead, which is a well-defined metric. Also, in practice all fuzzer is limited by a time budget. Thus, \GF can be thought of an optimization problem, where it searches over the entire input space to maximize the edge coverage. However, the input space of real-world programs is typically large; thus, an exhaustive search is infeasible. Instead, one needs to identify and focus the search on promising regions\textemdash evolutionary optimization techniques are standard practices to achieve this goal.  For example, a  genetic algorithm based fuzzer like AFL~\cite{} starts from a set of random seed inputs and 
select those inputs for further mutations that have explored new edges. 
To identify promising inputs, most of these fuzzers introduce some randomness while generating new mutants. Such randomness essentially makes \GF a \textit{stochastic optimization} process, %\textemdash GA creates new mutants through random mutation operations. 
where randomness can be introduced through 
(i) \textit{Seed input}, i.e., the input to mutate; 
(ii) \textit{Mutation location}, i.e., which byte location (offset) will be mutated, and 
(iii) \textit{Mutation operator} that determines the mutation operation to perform on those byte locations. 

% Thus, a \GF can be formally represented as a search over an input space $\mathcal{X}$ , where  $\mathrm{X}=\{X_1, X_2, ..., X_n\}\in\mathrm{\{0, 255\}^n}$ represents any single input and $X_i$ is the $i^{\text{th}}$ byte in $\mathrm{X}$, $\mathrm{X}$ contains $n$ bytes, and $\mathrm{X}\in\mathcal{X}$. Next, let us define $\mathrm{Y}=\{Y_1, Y_2,..., Y_m\}\in\{0, 1\}^m$ as the edges invoked in response to providing the input $\mathrm{X}$ to the program where $Y$ contains $m$ edges and $Y_i$ is the $i^\text{th}$ edge of the program's control flow graph. The goal of fuzzing then is to discover $x\in\mathcal{X}$ than maximizes the number of edges invoked, and this is usually performed using \textit{stochastic optimization} techniques. 
In this section, we will provide a more formal definition of how greybox fuzzing is performed using \textit{stochastic optimization}. Following this, we highlight the demerits of the current state-of-the-art and how our framework can help address these issues.

% Formally, let $\mathcal{X}$ represents the space of all possible inputs that can be provided to a program and let $\mathrm{X}=\{X_1, X_2, ..., X_n\}\in\mathrm{\{0, 255\}^n}$ represents any single input where $X_i$ is the $i^{\text{th}}$ byte in $\mathrm{X}$, $\mathrm{X}$ contains $n$ bytes, and $\mathrm{X}\in\mathcal{X}$. Next, let us define $\mathrm{Y}=\{Y_1, Y_2,..., Y_m\}\in\{0, 1\}^m$ as the edges invoked in response to providing the input $\mathrm{X}$ to the program where $Y$ contains $m$ edges and $Y_i$ is the $i^\text{th}$ edge of the program's control flow graph. The goal of fuzzing then is to discover $x\in\mathcal{X}$ than maximizes the number of edges invoked and this is usually performed using \textit{stochastic optimization} techniques. The rest of this section will provide a more formal definition of how fuzzing can be performed \textit{stochastic optimization}. Following this, we highlight the demerits of the current state-of-the-art and how our framework can help address these issues.


\subsection{Fuzzing with Stochastic Optimization}


% The remainder of this section details fuzzing from a stochastic optimization perspective. 

% In contrast, classical deterministic optimization assumes that perfect information
% is available about the loss function (and derivatives, if relevant) and that this
% information is used to determine the search direction in a deterministic manner at every step of the algorithm. In many practical problems, such information is not
% available.


% \bray{Define greybox fuzzing informally}


Stochastic optimization methods generate and use random variables to solve the optimization problem that is fuzzing. These methods work by introducing randomness into the fuzzing-process to accelerate the process of generating new seeds. For understanding how fuzzing is performed with stochastic optimization, it would be beneficial to view the input to the fuzzer $\mathrm{X}$ as a random vector and each byte in the input $\mathrm{X}_i$ as a random variable\footnote{The random vector $\mathrm{X}$ can be arbitrarily long. However, for this discussion, we limit $\mathrm{X}$ to a constant size of $n$. It can quite easily be generalized to any variable input length.}. The space of all inputs $\mathcal{X}$ would then represent the \textit{vector space} of all possible random vectors $\mathrm{X}$. Along the same vein, we can view the edges in the control-flow graph of the program $Y$ as another random vector with each edge $Y_j\in Y$ as a random variable. 

Stochastic optimization always occurs over a optimization objective. In order the formalize this optimization objective in the context of fuzzing, let us assume that there exists an underlying conditional distribution
\begin{equation}
    \label{eq:underlying distribution}
    \mathbb{P}(\mathrm{Y_j}=1~|~\mathrm{X}_i=x_i)
\end{equation}
 \eq{underlying distribution} measures the probability that the $j^{th}$ edge in the control-flow graph is invoked given that $\mathrm{X}_i$ (the $i^{th}$ byte in the input $\mathrm{X}$) is set to the value $x_i$. Then, over all the bytes in the input $\mathrm{X}$, we can compute the expected value of this conditional probability as follows:
\begin{equation}
    \label{eq:eq_a}
    \operatorname{E}(Y_j|X) = \frac{1}{n}\sum_{i=1}^{n}\mathbb{P}(Y_j=1~|~X_i=x_i)~\hspace{1em}x_i\in\left[0, 255\right]
\end{equation}
In other words,~\eq{eq_a} measures the expected value that the edge $Y_j$ is invoked as a result of passing the input $\mathrm{X}$ (represented as a random vector of byte values $x_i$, where $0\leq x_i \leq 255$). If we want this edge $Y_j$ to be invoked, we would want the stochastic optimization to maximize this expected value. That is, we want to
\begin{equation}
    \label{eq:eq_b}
    \maximize_{\mathrm{X}\in\mathcal{X}}~\operatorname{E}(Y_j|X) = \maximize_{\mathrm{X}\in\mathcal{X}}~\frac{1}{n}\sum_{i=1}^{n}\mathbb{P}(Y_j=1~|~X_i=x_i)
\end{equation}
We may generalize~\eq{eq_b} to include all the edges (represented by the random vector $Y$) in the control-flow graph as follows:
% 
% 
% Now, given a program with $m$ edges in its control-flow graph, an input $x$ will invoke certain edges in 
% 
% 
\begin{equation}
    \label{eq:formal_main}
    \maximize_{\mathrm{X}\in\mathcal{X}}\|\operatorname{E}(Y|X)\|\equiv\maximize_{\mathrm{X}\in\mathcal{X}}\left[\sum_{j=1}^{m}|\operatorname{E}(Y_j|X)|^2 \right]^{\frac{1}{2}}
\end{equation}
That is, we measure the norm of the expectation of edge invocation conditioned on a given input for all the output edges. When an input triggers a large number of edges, the norm is \textit{large}. Therefore, the goal of the overall optimization in \eq{formal_main} is to attempt to \textit{maximize} the norm so as to trigger as many edges as possible.

% may be understood as, \textit{``''}
% \note{a plain english description of~\eq{formal_main}: (a) What the norm represents (b) Why larger the norm the better?}
An input that satisfies~\eq{formal_main} exists in the vector space $\mathcal{X}$. In reality, this space, $\mathcal{X}$, of all possible inputs is combinatorially large. Further, each of the inputs $\mathrm{X}$ in $\mathcal{X}$ are highly nonlinear, high dimensional, and are otherwise inappropriate for deploying deterministic optimization strategies to solve for \eq{formal_main}. As a result, all greybox fuzzers, our work included, deprecate deterministic optimization in favor of \textit{stochastic optimization} for fuzzing. 

The stochasticity of the optimization arises as a result of the following three operations (i.e., functions over the vector space $\mathcal{X}$, and the random variables $\mathbb{X}$ and $\mathbb{Y}$) that are performed by all greybox fuzzers iteratively:
\squishlisttwo
\item[1.]\underline{Input selection}: Since, the original search space ($\mathcal{X}$) is extremely large, any optimization can realistically only occur over a subset of $\mathcal{X}$. This step, therefore, attempts to generate a subset of the input space \textit{randomly} over which the subsequent steps of fuzzing can take place. We denote this stochastic function by \texttt{Select}$(\mathcal{X})$ (note that this operation will return a subset of the original search space, i.e., \texttt{Select}$(\mathcal{X})\subset\mathcal{X}$); 
\item[2.]\underline{Mutation location selection}: For the inputs $X=\{X_1, X_2, ..., X_n\}\in\{0, 255\}^n$ that were obtained by performing \texttt{Select}$(\mathcal{X})$, greybox fuzzers \textit{randomly} choose certain byte locations (offsets) to perform mutations over. We shall discuss the rationale behind this in greater detail in \tion{hotbytes}. This stochastic function, that determines where in the input the mutations should occur, is denoted by \texttt{Offset}$(X)$; and, 
\item[3.]\underline{Mutation operator selection}: After sampling the original space of all inputs ($\mathcal{X}$) with \texttt{Select}$(\mathcal{X})$ and selecting locations (or offsets) in each test input $x$ where mutations are to be performed with \texttt{Offset}$(x)$, greybox fuzzers \textit{randomly} choose a mutation operation to perform on those byte locations. This stochastic function, that implements the  mutation is denoted by \texttt{Mutate}$(x)$.  
\squishend
In order to solve~\eq{formal_main}, traditional approaches use an stochastic evolutionary optimization strategy. To do this: 
\squishlisttwo
\item[] {\bfseries Step 1.} They apply \texttt{Select}$(\mathcal{X})$ to generate a sample population of initial seed inputs. 
\item[] {\bfseries Step 2.} Then, for every seed $\mathbb{X}$ that was obtained in the previous step, they apply \texttt{Offset}$(X)$ to select specific byte offsets where the mutations should occur.
\item[] {\bfseries Step 3.} Finally, for the bytes locations (offsets) that were chosen above, the current seed input $X=\{X_1, X_2, X_3, ..., X_n\}\in\{0, 255\}^n$ to produce a new mutated input $\hat{X}=\{\hat{X}_1, \hat{X}_2, ..., \hat{X}_n\}\in\{0, 255\}^n$. The new mutated input $\hat{X}$ is retained if it results in a larger value for~\eq{formal_main}, i.e., if it invokes more edges as compared to the old input $X$. In other words, $\hat{X}$ is retained if:
\begin{equation}
\label{eq:eq_2}
\left\|~\operatorname{E}\left(\mathrm{Y}~|~\hat{X}\right)~\right\| > \|\operatorname{E}\left(\mathrm{Y}~|~x\right)\|
\end{equation}
If~\eq{eq_2} is not satisfied, the new test input is discarded. The population is then updated with the retained test inputs $\hat{X}$. This process is performed for all the seeds from step 1 keeping new seeds that perform better and discarding those that do not.  
\squishend
The three steps above are repeated iteratively. This evolutionary strategy was first popularized by a greybox fuzzer called American Fuzzy Lop (hereafter referred to as AFL)~\cite{zalewski2017american}. As symptom of using stochastic evolutionary optimization for fuzzing, it was discovered that certain byte locations in an input are far more likely to invoke new edge coverage compared to certain other byte locations. These byte locations are called \textit{hot-bytes} and have consistently been observed by several researchers~\cite{taintscope, rajpal2017not,lemieux2017fairfuzz,chen2018angora,vuzzer}. These \textit{hot-bytes} have been used in a variety of ways to improve fuzzing. 

\input{tex/hot_bytes.tex}

\fig{hot_bytes} illustrates the distribution of hot-bytes in \textit{readelf} (one of our test programs). This figure was obtained after running AFL for 1 hour and gathering the byte-location of the mutations and the corresponding edge coverage. Notice that the locations highlighted in red have significantly higher probability of invoking new edges as compared to the rest; these locations represent the \textit{hot-bytes}.

\subsubsection{Distribution of Hot-bytes}
\label{sect:hotbytes}
In order to define \textit{hot-bytes} formally, we reflect on the conditional distribution $\mathbb{P}(\mathrm{Y_j}=1~|~\mathrm{X}_i=x_i)$ (\eq{underlying distribution}) which measures the probability that the $j^{th}$ edge in the control-flow graph is invoked given that $\mathrm{X}_i$ (the $i^{th}$ byte in the input $\mathrm{X}$) is set to some value $x_i$. We can generalize the conditional distribution over all the edges using the \textit{total influence} function $\operatorname{\mathbb{I}}(\cdot)$ from boolean algebra~\cite[p.~49, \S~2.3]{o2014analysis}, which is given below:
% 
% let us represent a test input $x$ of length $n$ as a set of bytes $x=\{x_1, x_2, x_3, ..., x_n\} \in \{0, 255\}^n$. Each byte $x_i$ in $x$ is in-turn comprised of 8 bits. This means that a byte $x_i$ is a boolean function $x_i\equiv f:\{0, 1\}^k$ where $k$ is called the \textit{arity} of the boolean function $f$. Since a byte contains 8 bits, $k=8$, i.e., $x_i\equiv f:\{0, 1\}^8$. If a byte $x_i$ is ``hot'', then a change in at least one of the bits in $x_i$ will lead to a corresponding change in the edge coverage $Y$. This allows us to define a ``probability
% that the $j^{th}$ bit in $x_i$ affects the number of edges invoked $\mathrm{Y}$''. This probability is known as the \textit{influence} function $\operatorname{Inf_j}(\cdot)$~\cite[p.~46, \S~2.2]{o2014analysis}:
%
% \begin{equation}
%     \operatorname{Inf}_j[x_i] = \mathbb{P}(\mathrm{Y}~|~x_{i,~j}=1)
% \end{equation}
% %
% Here, $x_i$ is a byte in the input $x$, and the $j^{th}$ bit in $x_i$ is represented as $x_{i,~j}$. To measure if the whole byte $x_i$ is a ``hot-byte'', we need to aggregate the influence $\operatorname{Inf_j}(\cdot)$ for all the 8 bits in $x_i$. This measure is called the total influence $\operatorname{I}(\cdot)$ in boolen algebra~\cite[p.~49, \S~2.3]{o2014analysis}, it is defined as follows:
%
\begin{equation*}
    \operatorname{\mathbb{I}}(X_i) =  \left\|\mathbb{P}(\mathrm{Y}~|~X_i=x_i)\right\|~\hspace{1em}x_i\in\left[0, 255\right]
\end{equation*}
\begin{equation}
    \label{eq:total_influence}
     \hspace{-2em}= \left[\sum_{j=1}^{m}\mathbb{P}(\mathrm{Y}_j~|~X_i=x_i)\right]^{\frac{1}{2}}
\end{equation}
%
From the context of hot-bytes, the \textit{total influence} measure $\operatorname{\mathbb{I}}(\cdot)$ can be understood as follows:
%
\be[leftmargin=*]
\item $\operatorname{\mathbb{I}}(x_i) = 0$: The total influence of a byte $x_i$ is zero. This means that, regardless of which bit $j$ in $x_i$ is changed, it has no impact on the edge coverage $Y$. Therefore this byte will not be a ``hot-byte''.
\item $\operatorname{\mathbb{I}}(x_i) > 0$: The total influence of a byte $x_i$ is positive. This means that, when one or more bits $j$ in $x_i$ are changed, there is a \textit{non-zero impact} on the edge coverage $Y$. Therefore this byte will potentially be a ``hot-byte''. Note that, the \textit{larger} the value of $\operatorname{\mathbb{I}}(x_i)$, the \textit{more likely} the byte $x_i$ is a ``hot-byte''. 
\ee
%
Now, it becomes possible to obtain all the hot-bytes in an input $X={X_1,~X_2,~...~,~x_n} \in \{0,~255\}^n$. To do this, let us partition the set of input bytes $X_i \in X$ into two disjoint subsets $A\subset X$ and $B\subset X$ such that $A\cap B=\varnothing$ and $A\cup B=X$. Then $A$ would represent all the \textit{hot-bytes} in $x$ if:
\begin{equation}
\label{eq:eq_3}
    \operatorname{\mathbb{I}}(X_p) > \operatorname{\mathbb{I}}(X_q)\hspace{1em} \forall X_p\in A,~X_q\in B    
\end{equation}
Biasing fuzzing towards these \textit{hot-bytes} can be achieved trivially if the conditional distribution of~\eq{underlying distribution} is known. All that would have to be done is: 
%
\be[leftmargin=*]
\item Partition the input bytes according to~\eq{eq_3};
\item For each byte $X_p$ in the set of hot-bytes $A$, bias the mutation until ~\eq{formal_main} is satisfied. 
\ee
Unfortunately, it is not possible to know $P(\mathrm{Y}~|~x)$ before hand and therefore, evolutionary greybox fuzzers like AFL resort to performing random mutations over the bytes in the input. At each iteration they only retain those mutated inputs that achieve new edge coverage. Since hot-bytes are most likely to increase coverage, these newly generated test inputs are most likely to have had mutations performed on the locations corresponding to these hot-bytes. Consequently, over a large number of iterations, greybox fuzzers gradually focus the mutations on these ``hot'' byte locations. 

\subsubsection{Improving greybox fuzzing with heuristics}
\label{sect:heuristics}
As discussed above, at each iteration, an evolutionary greybox fuzzer makes three choices regarding:
\squishlisttwo
\item Input selection; 
\item Mutation location selection; and, 
\item Mutation operator selection.
\squishend
Traditional greybox fuzzers such as AFL make each of these choices randomly and are hence susceptible to wasting valuable resources in fruitless mutations.
Therefore, much research has focused on developing \textit{heuristics} in order to guide these choices. As an example, consider the following studies (for details see~\tion{related} on related work):

\squishlisttwo
\item \textit{On input selection}: In AFLFast~\cite{bohme2017coverage}, B\"{o}hme et al. propose the use of heuristics such as power schedules in conjunction with Markov chains to assist in prioritizing the input queue for mutation.
\item \textit{On mutation location selection}: In FairFuzz~\cite{lemieux2017fairfuzz}, Lemieux et al. propose a modified mutation strategy with an input mask to prevent from mutating certain important byte locations. Additionally, a number of alternative heuristics have been proposed for this task~\cite{vuzzer,chen2018angora, steelix,You2019SLFFW,You2019ProFuzzerOI}.
\item \textit{On mutation operator selection:} In Angora by Chen et al.~\cite{chen2018angora} and NeuZZ by She et al.~\cite{she2018neuzz}, gradients are used to guide mutations, while Vuzzer by Rawat et al.~\cite{vuzzer} uses a hybrid approach involving static analysis to perform the mutation operation.
\squishend
These heuristics are designed to help expedite the generation of test inputs that invoke new edge-coverage by guiding mutations towards the hot-bytes. They still function under the permise that the conditional distribution $P(\mathrm{Y}~|~x)$ that defines a given program is unknown. As a result, for every new program, it becomes difficult to determine which of these heuristics are important and which are not without having to perform extensive empirical analysis.  

\subsection{Gradient Guided Greybox Fuzzing}
\input{tex/ga_vs_gd.tex}

In this section, we explore how greybox fuzzing can be solved with the help of gradient guided (or first-order) optimization techniques. We demonstrate that the gradient guided optimization can enable us to develop an extensible framework that can easily incorporate all the individual heuristics introduced  by evolutionary fuzzers that were discussed above. 

\subsubsection{Fuzzing as a first-order optimization problem}
\label{sect:adaptive_framework} 

The evolutionary fuzzers discussed previously fall under a family of so called \textit{zeroth-order} methods~\cite{Maheswaranathan2018}. The term zeroth-order refers to the fact that they make no assumptions regarding the underlying distribution and therefore do not use any first- or higher-order derivatives to solve the optimization problem. However, being able to use gradient guided (first-order) methods to perform fuzzing is a particularly enticing alternative due to their ease of implemetation, efficiency, and strong convergence guarantees~\cite{Maheswaranathan2018, sra2012optimization, juditsky2011first}.

Gradient based methods can be only be used when the underlying distribution of a the problem is known. However, even when this is not the case, a number of recent studies have shown that it is still possible to employ gradient based methods by using an artificial neural network to learn a \textit{surrogate} representation of the distribution~\cite{Maheswaranathan2018, she2018neuzz}. This is by virtue of the \textit{universal approximation theorem} which states that, ``A feed-forward network with one or more hidden layers, containing a finite number of neurons, can approximate any non-linear, non-convex, or a bounded discontinuous function''~\cite{funahashi1989approximate, csaji2001approximation, anil2018sorting}.

Using the universal approximation theorem, we can cast the fuzzing problem as that of a learning problem where the goal is to use artificial neural networks to learn an approximation of the conditional probability branch coverage with respect to a given test input for the program being inspected, i.e., we want to learn an approximation of $P(\mathrm{Y}~|~X)$. For formalization, let us again assume that $\mathcal{X}$ represents the space of all possible inputs that can be provided to a program. Then, any single input can be represented as $\mathrm{X}=\{X_1, X_2, ..., X_n\}\in\mathrm{\{0, 255\}^n}$ where $X_i$ is the $i^{\text{th}}$ byte in $X$ and $\mathrm{X}\in\mathcal{X}$. Next, let us say $\mathrm{Y}=\{Y_1, Y_2, ..., Y_n\}\in\mathrm{\{0, 1\}^m}$ represents all the edges invoked in response to providing the input $\mathbb{X}$ to the program. With this, we construct an artificial neural network by providing $X$ as the input and predicting for $\mathrm{Y}$. After training this neural network with inputs $x\in\mathcal{X}$, we now obtain an surrogate conditional distribution $\hat{P}(\mathrm{Y}_j~|~X_i)$ of the true conditional distribution $P(\mathrm{Y}_j~|~X_i)$. For simplicity, in the remainder of this paper we denote the surrogate distribution $\hat{P}(\mathrm{Y}~|~x)$ as $\mathrm{G}(x)$. 

Using the surrogate distribution, the original optimization problem from~\eq{eq_1}, may now be restated as:
\begin{equation}
    \label{eq:eq_4}
        \text{Fuzzing}~\equiv~\max_{x \in \mathrm{X}}\left[\sum_{i=1}^{n}P(\mathrm{Y}~|~x_i)\right]~\equiv~\max_{x \in \mathrm{X}}\left[\sum_{i=1}^{n}G(_i)\right]
\end{equation}
A desirable property of surrogate distribution $\hat{P}(\mathrm{Y}~|~x)$ generated using an artifical neural network is that it allows for computing first- and higher order derivatives. Specifically, it is possible for us to algorithmically evaluate the derivative of $\hat{P}(\mathrm{Y}~|~x)$ with respect to $x$. There is a rich literature on techniques such as \textit{automatic differentiation} which have been used extensively for computing derivatives of the parameters in an artifical neural network~\cite{wengert1964simple,block1991siam,baydin2018automatic}. 

In our case, with the trained artificial neural network, we can generate the gradients of edge coverage $\mathrm{Y}$ with respect to the bytes in the test input $x$. That is, we can obtain:
\begin{equation}
    \label{eq:eq_5}
        \nabla\mathrm{G(x)} = \left[\frac{\delta\mathrm{G}}{\delta x_1},~\frac{\delta\mathrm{G}}{\delta x_2},~\frac{\delta\mathrm{G}}{\delta x_3},~...~,~\frac{\delta\mathrm{G}}{\delta x_n}  \right]
\end{equation}
The values of the gradient serve as a useful tool for understanding how the bytes in the input to the program affect the edge coverage. For each byte, there are two possibilities:
\be[leftmargin=*]
\item $\left| {\frac{{\delta G(x)}}{{\delta {x_i}}}} \right| > 0$: For a byte  $x_i\in x$, if the absolute value of the gradient $\nabla_{x_i}G(x)$ is \textit{non-zero}, then a change in $x_i$ results in some change in the edge coverage $\mathrm{Y}$.
\item ${\frac{{\delta G(x)}}{{\delta {x_i}}}} = 0$: For a byte $x_i\in x$, if the gradient $\nabla_{x_i}G(x)$ is \textit{zero}, then a change in $x_i$ \textit{does not} result in a change in the edge coverage $\mathrm{Y}$.
\ee
It can be observed that, conceptually, the value of the gradients resembles the distribution of \textit{hot-bytes} discussed previously. Our results demonstrate that this is indeed the case. For example, in~\fig{grad_dist} we plot the distribution of gradients for readelf along with the hot-bytes obtained from AFL. We note that the distribution of hot-bytes obtained from AFL closely resembles the value of the gradients computed at those byte locations. This demonstrates that deriving gradients from an artificial network is analogous to learning the distribution of hot-bytes.

Using the gradients from~\eq{eq_5} we can now solve the original fuzzing problem of~\eq{eq_4} using a simple \textit{gradient ascent} method. Given a test input $x^{t}$, we can create a new test input $x^{t+1}$ as follows:
\begin{equation}
    \label{eq:eq_6}    
    x^{t+1} = x^{t} + \alpha \cdot \nabla G(x)
\end{equation}
Here, $\alpha$ is the step-size of the mutation. We may expand~\eq{eq_6}, for each byte $x_i\in x$ as follows: 
\begin{equation}
    \label{eq:eq_7}    
    x^{t+1}_i = x^{t}_i + \alpha \cdot \frac{\delta\mathrm{G}}{\delta x_i}\hspace{1em}\forall x_i\in~x
\end{equation}
From~\eq{eq_7}, we see that when $\nabla_{x_i}G(x)$ is \textit{non-zero}, that byte location is mutated by the step-size $\alpha$ and when $\nabla_{x_i}G(x)$ is \textit{zero}, we make no change to that byte. This ensures that bytes that have some effect on invoking edge coverage (i.e., \textit{hot-bytes}) are mutated while the remaining bytes remain unchanged.

\subsubsection{Constructing an adaptive framework}
\label{sect:adaptive_framework} 
In theory, the above formulation (\eq{eq_4}) for solving fuzzing as a gradient based optimization can ensure strong convergence guarantees~\cite{Maheswaranathan2018}, in practice however, it may take prohibitively long to converge. It is therefore advisable to incorporate additional parameters to the optimization in form of budget constraints. 
\input{tex/eq_fig.tex}
According to~\eq{eq_4}, the input samples $x$ belonged to the space of all possible samples $\mathrm{X}$ (i.e., $x\in X$). This space is combinatorially large and for practical purposes it may not be possible to exhaustively explore the whole space. Therefore, we introduce a optimization budget $K$ that limits the number of samples we choose from the space of $\mathrm{X}$. We introduce a \textit{selection operator} $C_K(\mathrm{X})$ that selects the $K$ most salient samples from the original space of $\mathrm{X}$. Now, we may reformulate the original optimization problem as:
\begin{equation}
    \label{eq:eq_8}
    \text{Fuzzing}~\equiv~\max_{x \in C_K(\mathrm{X})}\left[\sum_{i=1}^{n}G(x_i)\right]
\end{equation}

It is worth noting that solving~\eq{eq_8} with gradient ascent is an inherently adaptive framework. It lends itself neatly to incorporating a number of heuristics. We see that the heuristics discussed in \tion{heuristics} manifest themselves as parameters of the optimization problem. By carefully choosing these parameters, we can guide the fuzzing towards the most desirable regions of the input. This is illustrated in~\fig{optimization_parameters},
\be[leftmargin=*]
\item In \subfig{4_a}, \circled{1} shows that the optimization occurs over the space defined by the \textit{selection operator} $C_K(\mathrm{X})$. This parameter is similar to the input selection strategies of studies like that of B\"{o}hme et al. discussed in \tion{heuristics}. Details of our preferred selection operator are discussed in \tion{XXX}.
\item In \subfig{4_b}, \circled{2} shows that the gradients are use to make updates to the specific byte locations. If, at a specific byte, the gradient is zero, then no update happens there. This is comparable to the mutation location selection strategies of studies like that of FairFuzz discussed in \tion{heuristics}. In \tion{YYY}, we discuss in detail how gradient guided mutation may be used to direct fuzzing.
\item In \subfig{4_b}, \circled{3} represents the step-size of the mutation. By modifying this parameter, we can control how the mutation operator is implemented. This is analogous to the heuristics proposed by Angora~\cite{chen2018angora}. In \tion{YYY}, we discuss how to choose this parameter.
\item Finally, \circled{4} in \subfig{4_b} represents a novel contribution of this paper. We show in \tion{ZZZ} that, with our neural framework, it is possible to replace the dependent variable $Y$ (which represents edge coverage) with alternatives such as \textit{branch distance} to further guide fuzzing towards \textit{hard-to-reach} sections of the code. 
\ee



\subsection{Motivating Example}
\input{tex/motivating_example.tex}

==> body/intro_bck.tex <==
Fuzzing is a popular technique for detecting bugs and security vulnerabilities in real-world software systems~\cite{zalewski2017american, cgc}. It is arguably one of the most popular and effective approaches used by both researchers and industry practitioners to test different types of software~\cite{zalewski2017american, manes2018fuzzing, wang2019superion,Nilizadeh2019,You2019,lemieux2017fairfuzz,she2018neuzz, godefroid2008, arya2012fuzzing, evans2011fuzzing, moroz2016guided}. 

The key idea behind a fuzzer is to execute the program under test on a large number of automatically generated test inputs and monitor the executions for buggy behaviors. However, as the input space of a program is typically very large, unguided test input generation is not effective at finding bugs. 
Therefore, most popular fuzzers, especially the graybox ones, use some form of evolutionary search to maximize code coverage (\eg edge coverage) in the hope of finding more bugs as more code is executed. Essentially, these fuzzers start with a set of seed inputs, mutate them to generate new inputs, execute the test program with these inputs, and identify the promising inputs using an evolutionary fitness function for further mutation~\cite{zalewski2017american, wang2019superion,Nilizadeh2019,You2019, wei2018singularity, steelix, godefroid2017learn,lemieux2017fairfuzz,jiang2018contractfuzzer}. 

The mutation process is the key to a fuzzer's effectiveness. Ideally, fuzzers want to spend more mutations in parts of the program input space that are likely to result in higher edge coverage. In fact, most of fuzzing research effort has been spent on designing and fine-tuning different mutation strategies. There are three main parameters in the mutation process:
(i) which inputs to mutate ~\cite{bohme2017coverage}? 
(ii) which locations in each input to mutate ~\cite{lemieux2017fairfuzz, vuzzer,chen2018angora, steelix,You2019SLFFW,You2019ProFuzzerOI}?  and, 
(iii)~which new values should replace the old values during mutation ~\cite{she2018neuzz, chen2018angora, vuzzer}? 
However, despite significant effort, manually %developing effective mutation strategies and 
finding appropriate parameter values that work well across different programs have turned out to be very difficult. 
The key challenge is that {the mutation parameters not only vary widely across different test programs but also change drastically depending on the actual input values being mutated for the same program. }
Therefore, it is important to build a {fuzzer}  that:

\squishlisttwo
    \item 
    Learns optimized mutation parameters \wrt different mutation strategies. 
    \item 
    Automatically adapts itself across different target programs.
    \item
    Automatically adapts itself across different test inputs for the same target program.
\squishend


% To address these challenges, 
% %In order to adapt the mutation parameters in a test-program-specific way, 
% prior work proposes leverages different information sources (\eg reached but not taken vs.~rare vs.~frequently covered edges, \etc), \eg  to implement different mutation strategies. However, these strategies often work in isolation and 
In order to adapt the mutation parameters, 
%in a test-program-specific way, 
prior works either use aggregated statistics on program behavior~\cite{bohme2017coverage,lemieux2017fairfuzz} or depend on  program analysis approaches like taint tracking~\cite{vuzzer,chen2018angora, steelix}. Unfortunately, both of these approaches suffer from significant limitations\textemdash while aggregated-statistics-based approaches often miss many input-specific variations, taint-tracking-based approaches suffer from high false positives and false negatives~\cite{she2019neutaint}. Therefore, we seek alternative approaches to learn important mutation parameters automatically. 

% Recently, several projects have shown initial promise in using machine learning techniques that use input/program features for designing mutation strategies~\cite{}. However, all of the existing approaches formulate the learning task in ways that are very specific to particular classes of features like test input formats~\cite{} or program branching behaviors~\cite{}. Due to this inherent limitation, it is very hard, if not infeasible, to make these models use any features other than the original one.

In the recent past, several projects have shown initial promise in using machine learning (ML) techniques to automatically learn the mutation parameters for the target program. 
%However, all of these existing approaches formulate the learning task for specific mutation strategies. 
For example, Learn\&Fuzz uses an RNN-based language model to learn input PDF format~\cite{godefroid2017learn} for PDF fuzzing, NEUZZ uses a feed-forward neural network to distinguish between taken and non-taken program branches~\cite{she2018neuzz}.  All these tasks first model a particular information source (\eg input format, branching behavior, etc.) and then use a specialized algorithm to extract promising input regions from these models for further mutations. 

However, in practice, achieving high edge coverage often requires leveraging different mutation strategies that targets different types of information from different parts of the target program (\eg reached but not taken vs.~rare vs.~frequently covered edges, \etc) as well as test inputs (\eg which byte locations to mutate). 
Such information sources have long been exploited in ad hoc fashion by the fuzzing community by customizing the fitness function of evolutionary fuzzing frameworks like AFL\cite{zalewski2017american}. 
For ML-based fuzzers, it is not clear how similar effects can be achieved. While it is theoretically possible to build different models for different information sources and combine their results, finding good parameter values, optimizing, and managing such ensemble models are very hard in practice. Moreover, the training those ensemble models add significant computation cost that will slow down the fuzzing process.

%It is not practical and efficient to create different models for different sources and combine their results. 


To this end, in this paper, we describe a generic ML framework, \tool, that can learn from different types of program- and input-specific information using a simple neural network (NN) and use gradient-guided optimization to identify optimal mutation parameters in each round of the mutation process. One of the main challenges behind using ML for learning mutation parameters is that as the fuzzing explores new parts of the target program and the input space, the mutation parameters may change drastically. A good adaptive mutator should be able to learn and generalize from different behaviors gathered from already explored parts to the unseen parts of the program. However, this is very hard to achieve with existing ML-based fuzzers. For example, ML models like NEUZZ~\cite{she2018neuzz} that tries to predict edge-coverage purely based on the already explored edges is unlikely to predict rare edges that the model has never seen before (\ie model does not know about its existence). 

Traditionally, researchers have been able to incorporate the  information of seen vs.~unseen region using some distance metrics, \eg how far a fuzzer is from executing an edge can be measured using branch distance~\cite{arcuri2010does}).  Existing ML-based fuzzers cannot incorporate such information easily. 
To address such issues, \tool allows learning from different sources of information through different encodings of training data and customized loss functions.
To learn optimal parameter values in an information-source-agnostic way, \tool further uses a  gradient-guided optimization technique.
Our key insight is that the mutation operation can be thought of as a parameterized function operating on the program input space and edge probability space. \tool can model a smooth function between the program inputs and the probability of each edge being taken from diverse information sources (e.g., different features from program traces) and use the gradient of that neural network to find mutation parameters that maximize the probability of unseen edges being taken. 
%Traditionally, researchers have been able to incorporate information like how close the fuzzer came to executing some edges using different distance metrics (e.g., branch distance~\cite{arcuri2010does}) to distinguish such edges from the ones that were further away from execution path. Existing ML models for fuzzing cannot incorporate such information easily. To address such issues, \tool allows learning from different sources of information through different encoding of training data and customized loss functions. \tool further uses a information-source-agnostic gradient-guided optimization technique for finding optimal parameter values. Our key insight is that the mutation operation can be thought of as a parameterized function operating on the program input space and edge probability space. \tool can model a smooth function between the program inputs and the probability of each edge being taken from diverse information sources (e.g., different features from program traces) and use the gradient of that neural network to find mutation parameters that maximize the probability of unseen edges being taken. 

\input{tex/intro_fig.tex}
%Our gradient-guided framework adaptively identify good mutation strategies during the fuzzing process based on the observed test program behavior. The main challenge behind using machine learning for learning mutation strategies is how to formulate the problem so that the model can generalize the observed behavior from already explored parts of the program to unseen branches parts of the program. Note that a naive formulation like using the ML model directly trying to predict which input values are likely to trigger  unexplored branches will not work without any data about that branch. To avoid such issues, we formulate the mutation strategy of a fuzzer as an optimization problem and use gradient-guided optimization for finding optimal parameter values. Our key insight is that the mutation operation can be thought of as a parameterized function operating on a whose behavior for each input for a given program can be smoothly modeled using a neural network and the gradient of the neural network can be used to select and adapt the parameter values as the program behavior as well as the explored input region changes.


Overall, our paper makes the following key contributions:
\squishlisttwo

\item[1.] 
We propose \tool, a neural-network-based adaptive framework that can automatically find good mutation parameters by learning from different information collected from prior mutations and program executions. To achieve this, we formulate the problem of finding optimal parameters for mutation as an optimization problem which \tool solves using gradient descent to automatically find the optimal mutation parameters at any given step the fuzzing operation.

\item[2.] We present a new parameterized mutation scheme that can leverage information about the probability of different control flow edges being taken in a program for different inputs to distribute mutations to maximize the chances of new edge discovery. We model the mapping between program inputs and the probability of edges being taken using a neural network and use its gradients to guide the parameter selection of the mutation operation. 


\item[3.] Experiments demonstrate that our gradient-guided mutator outperforms current state-of-the-art methods in discovering more rare-edges and also in exploring  novel seeds (see~\tion{offset_selection} and RQ2 in~\tion{rqs}). Our experiments further  that our framework can leverage different types of information sources like a branch-distance~\cite{arcuri2010does} based soft-labeling scheme and a customized loss function to prioritize mutations that might result in exploring rare edges according to our ML model. 

\item[4.] We demonstrate that our ML models mapping from program input to edge probability space offer a high degree of transferability. A network trained using data from one program can be used to efficiently update the parameters of a similar program (e.g., a program that parses the same file format as the first one). We believe that such sharing of models can potentially result in drastic reduction of fuzzing overhead for programs with similar functionality.
\squishend


The rest of this paper is structured as follows. \tion{formalization} describes the problem formulation and explains the concept of gradient guided smoothing. \tion{beetle} describes our methodology In \tion{expt}, we present experimental setup and followed by answers to research questions in \tion{results}. In \tion{disc}, we discuss our findings further and answer some additional questions pertaining to our results. \tion{threats} describes some threats to validity. Finally, related work and conclusion are presented in \tion{related} and \tion{conclusion} respectively.

==> body/methodology_bck.tex <==
\input{tex/heursitics.tex}
\input{tex/pseudo.tex}

\section{\textsc{FuzzNN} Methodology}
%\section{Gradient Guided Fuzzing with \textsc{NABLA}}
\label{sect:our_method}

Section~\ref{sec:theory} lays out the basic working principle of \tool 
with a simple example. Here, we will describe different design choices that makes \tool applicable for real-world programs. 

%The previous section presented a very simple example example to demonstrate how a neural network is used to generate gradients that can guide fuzzing. Real world programs are seldom this straightforward; it is therefore imperative that our neural network and the gradients derived from it accomodate the challenges such as complexity and size that most often accompany real world scenarios. Thus, in the rest of this section, we present a more general adaptive neural framework called \tool that generalizes the example discussed in \tion{motivate} to a wide variety of real world programs. 

% \subsection{General Framework}
% \label{sect:general_framework}
A complete pseudocode of \tool is shown in \fig{pseudo}. For this subsection, we focus on the main method used to perform fuzzing, shown in \protect\fig{general_framework}. It contains the following key elements:
\squishlisttwo
\item \noindent{\textit{\protect\fig{general_framework}, Line 7 (Intialization)}}: We begin with a initial set of valid seed inputs. To obtain this, we run AFL for 1 hour and save all the valid seeds it generates. This gives us about 2000 to 5000 seed inputs depending on the size of the programs. These seed inputs will be used to train the neural network and compute the gradients to generate newer inputs.

\item \noindent{\textit{\protect\fig{general_framework}, Line 8 (Begin fuzzing)}}: This step initiates fuzzing. Here, the parameter \texttt{n\_rounds} controls the number of iterations of fuzzing to perform. \tool can run perpetually, so we need to limit the duration of fuzzing based on the available resources.

\item \noindent{\textit{\protect\fig{general_framework}, Lines 9--13 (Seed selection)}}: From the set of all available inputs, we obtain a sample of the most important inputs. This is performed with the help of the method \texttt{sample\_inputs($\cdot$)}. In \tion{seed_selection} we will discuss in much greater detail why sampling is important and how we implement this method.  After sampling inputs, we obtain the egdes invoked by each of the sampled inputs with \texttt{get\_coverage()}. The coverage is represented as an array of 1's and 0's; a 1 represents that the edge is invoked and a 0 represents that the edge is not taken. %It follows that the length of the coverage array is the total number of edges in a program's control-flow graph.

\item \noindent{\textit{\protect\fig{general_framework}, Lines 14--20 (Mutation offset selection)}}: To determine the locations (byte offsets) in the input to perform the mutations, we train a neural network (line 16). The sampled seeds obtain previously on line 11 are provided as inputs to the neural network. 
\noindent In this neural network: 
\squishlisttwo
\item Each input layer node corresponds to a byte in the test input;
\item Accordingly, the total number of nodes in the input layer of the neural network would therefore be equal to the total number of bytes in the largest test inputs. Note that the shorted test inputs are padded with \texttt{0x00} for consistency.
\squishend
As for the output layer of the neural network, each node corresponds to one edge of the program's control-flow graph. Thus, the total number of output nodes will be equal to the total number of edges in a program's control-flow graph. After training the neural network with adaptive loss function in line 18, the last step in \textit{mutation offset selection} is to obtain gradients of the output layer of the neural network (i.e., the edge converage) with respect to the input layer (i.e., the bytes in the input). This can be done quite easily with autodiff~\cite{block1991siam}. The gradients obtained in line 20, is a vector whos length is same as that of input layer, i.e., for each byte in the input layer, there will exist a gradient value. The magnitude of the gradients will determine how likely each byte is to impact the edge coverage. If the gradient of an input byte is zero, then that byte has no effect on increasing the converage.

\item \noindent{\textit{\protect\fig{general_framework}, Lines 21--25 (Mutation operation)}}: Finally, we mutate the inputs with using gradient ascent as discussed in \tion{operation_selection}.\\[-1.5em]
\squishend
\subsection{Incorporating Heuristics}
\note{A few lines here about how other use heuristics and how this is different and more effective ...}
\subsubsection{Input selection with importance sampling}\hfill\\
\label{sect:seed_selection}
Sampling the inputs is an important step because, as fuzzing progresses, the pool of available inputs keeps growing in size. Without some sampling strategy, training the neural network and subsequently computing gradients will take prohibitively long. 

We propose an importance sampling based input selection strategy. The pseudocode in \protect\fig{seed_selection} highlights our importance sampling strategy. To determine the importance of an input, we note following considerations:
\squishlisttwo
\item Sampling budget determines how many inputs can be retained.
\item Some edges in the control-flow graphs are invoked very rarely 
\item We would like guide the fuzzing towards invoking these rare edges more often to ensure that the new inputs will explore deeper regions of the program.
\squishend
On that account, our sampling strategy must keep inputs that invoke these rare edges. To do this, we first sort the edges by rarity from most-to-least rare (see \protect\fig{seed_selection}, line 13). The rarer the edge, the more important it is. As an example, consider the \fig{seed_select_example}. 
\begin{figure}
    \begin{center}
        \resizebox{0.5\linewidth}{!}{
        \begin{tabular}{l|l|l|l|l}
            & a    & b    & c    & d    \\ \hline
            input 1    & 1    & 1    & 0    & 1    \\
            input 2    & 1    & 0    & 0    & 0    \\
            input 3    & 0    & 1    & 1    & 1    \\
            input 4    & 1    & 0    & 0    & 1    \\ \hline
            Frequency & 75\% & 50\% & 25\% & 75\%
        \end{tabular}}\\[0.5em]
        Sorted edges=$\{c, b, a, d\}$\\
        Sorted inputs=$\{\text{\textit{input~3, input~1, input~2, input~4}}\}$
    \end{center}
    \caption{A example of importance sampling seed selection.}
    \label{fig:seed_select_example}
\end{figure}
Here, we have 4 inputs and 4 edges. The last row measures the frequency of the edges. Sorting the edges of \fig{seed_select_example} gives us the order: $\{c, b, a, d\}$.

Next, contingent on the budget, we loop through each of the inputs (\protect\fig{seed_selection}, line 15). We first keep the inputs that invoke the rarest edge. Then, if more budget is available, we keep inputs that invoke the second rarest edge and so on until the budget is exhausted (\protect\fig{seed_selection}, line 19) as illustrated in \fig{seed_select_example}. 

\subsubsection{Mutation location selection with adaptive loss}\hfill\\
\label{sect:offset_selection}
\begin{figure}[tbp!]
    \centering
    \includegraphics[width=\linewidth]{figures/class_imbalance.png}
    \caption{Class Imbalance Example}
    \label{fig:class_imbalance}
\end{figure}
After obtaining a sample of the most important inputs, we train a neural network that predicts for the edge coverage. In our framework, the edge coverage is represented a boolean array where each index of that array corresponds to an edge in the control-flow graph. For each input, if an edge is invoked, that index location contains a `1' and a `0' if it is not invoked. 
It is worth noting that this neural network can be viewed as being trained for a multi-class classification task where each class represents an edge and the number of classes is the same as the total number of edges in a program's control-flow graph.

The output layer of the neural network returns values in the range of 0 to 1. Each node on the output layer corresponds on an edge and a value close to 1 would indicate that it predicts for the edge corresponding that node will be invoked. Likewise, a value close to 0 would indicate a prediction that the edge corresponding that node will not be invoked. 

In order to classify the edges accurately, we must define a \textit{loss fuction}. A program's edge converage is subject to a number of perculiarites. Specifically, we find that while some edges are invoked very often, some other edges are invoked very rarely. As a result, a neural network trained with off-the-shelf loss fuctions such as cross entropy are ill suited for this purpose, because they are prone to both (a)~\textit{Type-I errors} (or false postive errors) and (b)~\textit{Type-II errors} (or false negative errors). 

In order to accurately train a neural network, we must mitigate for these errors. \fig{class_imbalance} illustrates the false postive (Type I) and false negative (Type II) errors. The most commonly used loss fuction, the binary cross entropy measure, is formulated as follows:
\begin{equation}
    \label{eq:xent}
    \text{loss} = -\sum\left(p\cdot log{\hat{p}} + (1 - p)\cdot log(1-\hat{p})\right)
\end{equation}
In \fig{class_imbalance}, for an input (input 1) we highlight two egdes namely, \textit{a} and \textit{b}. Edge \textit{a} is invoked 99\% of the times, therefore a missclassification of this edge 1\% does not adversly affect the loss. Similary,edge \textit{b} is invoked only 1\% of the times, and wrongly classifying it as 0 would again not adversly affect the loss. However, it is excatly these edges that we need to correctly classify as they have significant impact on the gradients that are computed. 

Therefore, we must penalize both false postive (Type I) and false negative (Type II) errors and modify the loss function accordingly so that these errors would significantly increase the loss. Therefore, in \protect\fig{train_adaptive} line 3, we define a penalty for each edge (i.e., output node of the neural network). This penalty function measures, for each edge, the ratio of the number of times it is not invoked over the number of times it is invoked. 
\begin{equation}
    \label{eq:xent}
    \text{loss} = -\sum\left(\text{penalty}\cdot\hat{p}\cdot log{p} + (1 - \hat{p})\cdot log(1-p)\right)
\end{equation}
For edge, the penalty can take 3 possible values:
\squishlisttwo
\item $\text{penalty}>1$: This means the edge is very rarely invoked. Therefore, we penalize $p\cdot log{\hat{p}}$, representing false negatives, a lot more.
\item $\text{penalty}=1$: This means the edge is invoked and not invoked equal number of times. Here, we penalize both false positive and false negative equally.
\item $\text{penalty}<1$: This means the edge is invoked more often than not. Here, we penalize $(1-p)\cdot log{1 - \hat{p}}$, representing false positives, a lot more.
\squishend
\note{RAHUL: Tie this better with gradients}

% \subsubsection{Mutation operation selection with gradient ascent}\hfill\\
% \label{sect:opertaion_selection}


% \subsection{Branch distance based ``soft-labeling'' scheme}
% \label{sect:soft_label}
\input{tex/soft_label.tex}

==> body/notes_for_intro.tex <==
Limitation of ML-based fuzzer:
1. It is hard for NN to converge with a single task model and limited number of training set. Hence, multi-task model can implicitly increase the training data set size by learning from multiple tasks. 
2. Better NN model(encoder/decoder), multi-task models has more layers and complex model capacity to converge.
3. Further, joint optimization of multiple tasks could mitigate over fitting issue.

==> colors.tex <==
\sethlcolor{lightgray}
\definecolor{pink}{RGB}{252,145,149}
\definecolor{lightpink}{RGB}{252,145,149}
\definecolor{lightgray}{gray}{0.8}
\definecolor{darkgray}{gray}{0.6}
\definecolor{Gray}{rgb}{0.88,1,1}
\definecolor{Gray}{gray}{0.85}
\definecolor{Blue}{RGB}{0,29,193}
\definecolor{MyDarkBlue}{rgb}{0,0.08,0.45} 
\definecolor{pink}{RGB}{231,95,110}
\definecolor{lightergray}{rgb}{0.85, 0.85, 0.85}
\definecolor{lightestgray}{rgb}{0.95, 0.95, 0.95}
\definecolor{codebg}{HTML}{F4F4F4}

% ---- Grays ----
\definecolor{gray05}{gray}{0.95}
\definecolor{gray10}{gray}{0.90}
\definecolor{gray12}{gray}{0.88}
\definecolor{gray15}{gray}{0.85}
\definecolor{gray20}{gray}{0.80}
\definecolor{gray25}{gray}{0.75}
\definecolor{gray30}{gray}{0.70}
\definecolor{gray40}{gray}{0.60}
\definecolor{gray50}{gray}{0.50}
\definecolor{gray60}{gray}{0.40}
\definecolor{gray70}{gray}{0.30}
\definecolor{gray75}{gray}{0.25}
\definecolor{gray80}{gray}{0.20}
\definecolor{gray90}{gray}{0.10}


==> tex/branch_distance_table.tex <==
\begin{table}[]
    \centering
    \caption{Computing branch distance for various predicates. Note, $I$ represents an input, and $D(I)$ represents the branch distance~\cite{arcuri2010does}.}
    \label{tab:branch_distance_table}
    \resizebox{0.75\linewidth}{!}{%
    \begin{tabular}{@{}lll@{}}
    \toprule
    Predicate  & Notation          & Branch Distance $D(\cdot)$         \\ \midrule
    % $A$        & $D_A(I)$          & 0 if $A$ is \texttt{True} else $A$ \\
    $A == B$   & $D_{A==B}(I)$     & 0 if $|A-B|=0$ is \texttt{True}    \\
               &                   & else $|A-B|$                       \\
    $A \neq B$ & $D_{A\neq B}(I)$  & 0 if $A-B<0$ is \texttt{True}      \\
               &                   & else some constant $k$             \\
    $A < B$    & $D_{A < B}(I)$    & 0 if $A-B<0$ is \texttt{True}      \\
               &                   & else $|A-B|$                         \\
    $A \leq B$ & $D_{A \leq B}(I)$ & 0 if $A-B\leq 0$ is \texttt{True}  \\
               &                   & else $|A-B|$                         \\
    % $A > B$    & $D_{A > B}(I)$    & $D_{B < A}(I)$                     \\
    % $A \geq B$ & $D_{B \geq A}(I)$ & $D_{B \leq A}(I)$                  \\
    $\neg A$   & $D_{\neg A}(I)$   & Replace $A$ by $\neg A$ in all the \\
               &                   & children of the current edge       \\\bottomrule
    % $A\land B$ & $D_{A\land B}(I)$ & $D_{A}(I)+D_{B}(I)=0$              \\
    % $A \lor B$ & $D_{A \lor B}(I)$ & $min(D_{A}(I), D_{B}(I))$          \\ 
    \end{tabular}%
    }
\end{table}

==> tex/code_example.tex <==
\begin{figure}
\centering
\resizebox{0.87\linewidth}{!}{
\begin{minipage}{\linewidth}
\inputminted[bgcolor=codebg, numbersep=5pt, linenos=true, fontsize=\small]{c}{code/example.c}
\end{minipage}}
%\\[-1em]
\caption{A real-world example of successful input generation using branch-distance in \texttt{libxml}}
\label{fig:code_example}    
\end{figure}

==> tex/edge_cov.tex <==
\begin{table}[!t]
%\setlength{\tabcolsep}{2pt}
%\renewcommand{\arraystretch}{1.1}
\centering
\footnotesize
\caption{\textbf{\small The \textit{average} edge coverage of \tool compared with other fuzzers after 24 hours runs for 5 repetitions. The binaries were complied with \texttt{afl-clang}.}}
\label{tab:afl_cov_main}
\begin{tabular}{lrrrrrr}
   \hlineB{2}
   Programs & \textbf{\tool}  & \textbf{Neuzz} & \textbf{Angora} & \textbf{FairFuzz}& \textbf{\afl} & \textbf{\aflfast}\\ 
    \hlineB{1.5}
    readelf -a & \bf 8,109 & 5,953 & 7,757 &3,407 &  701 & 1,232 \\
    nm -C & \bf 4,112 & 1,245 & 3,145 & 1,694 & 1,416 & 1,277 \\
    objdump -D & \bf3,762 &  1,642& 1,465 & 1,225 & 163 &  134 \\
    size & \bf2,786 &1,170  &  1,586& 1,350 & 1,082 & 1,023 \\
    strip & \bf4,406 & 1,653 & 2,913 & 1,920 & 596 & 609 \\
    libjpeg & \bf543 & 328 & 201 & 504 & 327 & 393 \\
    libxml & \bf1,615 &1,419  & n/a & 956 & 358 & 442 \\
    mupdf & \bf1,107 & 533 & n/a & 503 & 419 & 536 \\
    zlib & \bf298 & 297 & n/a & 294 & 196 & 229 \\
    harfbuzz & \bf3,276 & 3,000 & n/a & 3,060 & 1,992 & 2,365 \\
  \hlineB{2}
\end{tabular}
\end{table}

==> tex/edge_cov_gcc.tex <==
\begin{table}[!htpb]
%\setlength{\tabcolsep}{2pt}
%\renewcommand{\arraystretch}{1.1}
\centering
\footnotesize
\caption{\textbf{\small Comparing the average edge coverage of \tool with other fuzzers for 24 hours runs for 5 repetitions on GCC-compiled binaires.}}
\label{tab:afl_cov_gcc}
\begin{tabular}{lrrrrrr}
\hlineB{2}
   Programs & \textbf{\tool}  & \textbf{Neuzz} & \textbf{Angora} & \textbf{FairFuzz}& \textbf{\afl} & \textbf{\aflfast}\\ 
   \hlineB{1.5}
    readelf -a & \bf 6,701  & 4,769 & 6,514 &3,423 &  1,072 & 1,314 \\
    nm -C & \bf 4,457 & 1,456 & 2,892 & 1,603 & 1,496 & 1,270 \\
    objdump -D & \bf5,024 & 2,017& 1,783 & 1,526 & 247 & 187\\
    size & \bf3,728 & 1,737  & 2,107 & 1,954 & 1,426 & 1,446 \\
    strip & \bf6,013 &2,726 & 3,112 & 3,055 & 764 & 757 \\
    libjpeg & \bf1,189 & 719 & 499 & 977 & 671  & 850 \\
    libxml & \bf1,576 &1,357 & n/a & 1,021& 395 & 388 \\
    mupdf & \bf1,107 & 533 & n/a & 503 & 419 & 536 \\
    zlib & \bf298 & 297 & n/a & 294 & 196 & 229 \\
    harfbuzz & \bf6,325 & 5,629 & n/a & 5,613 & 2,616  & 3,692 \\
    \hlineB{2}
\end{tabular}
\end{table}

==> tex/eq_fig.tex <==
\begin{figure}[tbp!]
    \begin{subfigure}[t]{0.45\linewidth}
        \centering
        \includegraphics[width=0.55\linewidth]{figures/eq_fig_1.pdf}
        \caption{The optimization problem}
        \label{subfig:4_a}
    \end{subfigure}%
    \begin{subfigure}[t]{0.45\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/eq_fig_2.pdf}
        \caption{Gradient ascent}
        \label{subfig:4_b}
    \end{subfigure}
    \caption{{\small A mathematical representation of performing fuzzing with a gradient guided optimization. Numbered circles represent various parameters that can be controlled to guide the optimization.}}
    \label{fig:optimization_parameters}
\end{figure}

==> tex/ga_vs_gd.tex <==
\begin{figure}[bp!]
    \begin{subfigure}[t]{0.45\linewidth}
        \centering
        \includegraphics[width=0.75\linewidth]{figures/ga.jpg}
        \caption{{\small Zeroth order optimization}}
        \label{subfig:ga}
    \end{subfigure}~~~~~~~%
    \begin{subfigure}[t]{0.45\linewidth}
        \centering
        \includegraphics[width=0.75\linewidth]{figures/gd.jpg}
        \caption{{\small First order Optimization}}
        \label{subfig:gd}
    \end{subfigure}
\caption{{\small Compares zeroth order (evolutionary) optimization with a first order (gradient guided) optimization~\cite{she2018neuzz}.}}
\label{fig:ga_v_gd}
\end{figure}
    

==> tex/heursitics.tex <==
\begin{table}[!b]
    % \centering
    \footnotesize
    %\vspace{-0.4cm}
    \caption{A summary of mutation parameters used by popular \gfz. 
    \tool incorporates them into its NN framework.}
\label{tab:who_does_what}
\resizebox{0.95\linewidth}{!}{%
\begin{tabular}{
    >{\columncolor[HTML]{FFFFFF}}l 
    >{\columncolor[HTML]{FFFFFF}}l 
    >{\columncolor[HTML]{FFFFFF}}l 
    >{\columncolor[HTML]{FFFFFF}}l }
\hline
\multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}}                         & \multicolumn{3}{c}{\cellcolor[HTML]{FFFFFF}Mutation Parameters}                                             \\ \cline{2-4} 
\multicolumn{1}{l}{\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}Fuzzer}} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}Seed Selection} & Offset Selection & Mutation\\ \hline
AFL~\cite{zalewski2017american}   & \textit{Def}  & \textit{Def}  & \textit{Def} \\
AFLFast~\cite{bohme2017coverage}  & \textit{Power}    & \textit{Def} &   \textit{Def}            \\
FairFuzz~\cite{lemieux2017fairfuzz}    &  \multicolumn{1}{l}{\textit{Rare}} & \textit{Mask}     & \textit{Def}  \\
Driller~\cite{You2019SLFFW}  &  \textit{Def}   & \textit{Sym} & \textit{Sym}                  \\
VUzzer~\cite{vuzzer}  &   \textit{Def}  &  \textit{Taint}  & \textit{Magic}            \\
KleeFL~\cite{cadar2008klee}   &  \textit{Def}  &  \textit{Sym} & \textit{Sym}                 \\
RNNFuzzer~\cite{rajpal2017not}   &    \textit{Def}                                                         &           \textit{Mask} &      \textit{Def}               \\
Steelix~\cite{steelix}   &    \textit{Def}   &     \textit{Taint}  &    \textit{Def}                 \\
T-Fuzz~\cite{tfuzz}    &   \textit{Def}  &    \textit{Def}     &  \textit{Def}            \\
Angora~\cite{chen2018angora}            & \textit{Def}                                                    & \textit{Taint}                & \textit{Coord}                   \\
NeuZZ~\cite{she2018neuzz}                                                                & \textit{Def}       & \textit{NN}, \textit{Grad}           &  \textit{Def}            \\
Learn\&Fuzz~\cite{godefroid2017learn}                                                                & \textit{Def}       & Recursive \textit{NN}           &  \textit{Def}            \\
\rowcolor{lightergray} \tool                                                                & Smart sampling                                                     & \textit{Adaptive NN}           & \textit{Gradient ascent} \\       \hline
\end{tabular}}
\begin{tabular}{ll}
    \textit{Def}: AFL-like default setting&
    \textit{Power}: Power schedule\\
    \textit{Taint}: Dynamic Taint analysis&
    \textit{Sym}: Symbolic execution \\
    \textit{Mask}: Byte Masking&
    \textit{Magic}: Magic  Value insertion\\
    \textit{NN}: Neural Networks&
    \textit{Grad}: Gradient-guided\\
    \textit{Rare}: Seeds invoking rare edges&
    \textit{Coord}: Coordinate descent 
    
\end{tabular}
\end{table}

==> tex/hot_bytes.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/hot_bytes.pdf}
    \caption{{\small Hot-byte distribution for readelf}}
    \label{fig:hotbytes}
\end{figure}


==> tex/intro_fig.tex <==
\begin{figure}[tbp!]
    \centering
    \includegraphics[width=\linewidth]{figures/intro_fig.pdf}
    \caption{{\small Overview of \tool. Here, $I$: inputs, $P$: Edge label, $\hat{P}$: Estimated edge labels by the NN, and $\nabla_{I}(\hat{p})$: Gradients from the NN. Blocks labeled \colorbox{black!15}{grey} represent user modifiable parts.}}
    \label{fig:intro_fig_1}
\end{figure}


==> tex/intro_fig_2.tex <==
% % \begin{figure}[t!]
% % \begin{center}
% % \begin{minipage}{0.95\linewidth}
% % 
% % \end{minipage}\\[0.1cm]
% % \end{center}
% % \caption{A framework for  gradient-guided neural fuzzing}
% % \label{fig:intro_fig_2}
% % \end{figure}

% \begin{figure}[t!]
% \begin{center}
% \begin{minipage}{0.495\linewidth}
% \includegraphics[width=0.9\linewidth]{figures/fig1_2}
% % \begin{equation*}
% % \hspace{-3em}\text{\textit{maximize}}~\sum_{x\in C_K(X)} G(x)
% % \end{equation*}
% \end{minipage}~~%
% \begin{minipage}{0.495\linewidth}
% \includegraphics[width=0.9\linewidth]{figures/fig1_3}
% % \begin{equation*}
% % \hspace{-3em}\text{\textit{maximize}}~\sum_{x\in C_K(X)} H(x)
% % \end{equation*}
% \end{minipage}
% \caption{A comparison of gradients from: (a)~Total vulnerabilities discovered (i.e., $G(x)$) and (b)~Branch coverage (i.e., $H(x)$). Note that the gradients over $H(x)$ are much smoother than those over $G(x)$.}
% \label{fig:intro_fig_2}
% \end{center}
% \end{figure}

% \begin{figure}[t!]
% \centering
%  \caption{{\small A general framework of evolutionary graybox fuzzers}}
%  \label{subfig:intro_fig_1}
% \end{figure}







% \begin{subfigure}[t]{0.95\linewidth}
%     \centering
%     \includegraphics[width=0.85\linewidth]{figures/fig1_1}
%     \caption{{\small A general framework of evolutionary graybox fuzzers}}
%     \label{subfig:vanilla_greybox}
% \end{subfigure}\\
% \begin{subfigure}[t]{0.95\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{figures/fig_1_2_1.eps}
%     \caption{{\small A general framework of evolutionary graybox fuzzers}}
%     \label{subfig:vanilla_greybox}
% \end{subfigure}\\

% \end{figure}

\begin{figure}
    \begin{subfigure}[t]{0.85\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/fig1_1.pdf}
        \caption{{\small Traditional Greybox Fuzzers}}
        \label{subfig:racing}
    \end{subfigure}\\
    \begin{subfigure}[t]{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/fig_1_2_1.pdf}
        \caption{{\small Adaptive Gradient-Guided Fuzzing}}
        \label{subfig:racing}
    \end{subfigure}\\
    \begin{subfigure}[t]{0.5\linewidth}
        \centering
        \includegraphics[width=0.75\linewidth]{figures/fig1_2.pdf}
        \caption{{\small Bugs vs. inputs}}
        \label{subfig:racing}
    \end{subfigure}~~%
    \begin{subfigure}[t]{0.5\linewidth}
        \centering
        \includegraphics[width=0.75\linewidth]{figures/fig1_3.pdf}
        \caption{{\small Branch coverage vs. inputs}}
        \label{subfig:racing}
    \end{subfigure}
    
    % \begin{minipage}{0.495\linewidth}
    % \includegraphics[width=0.9\linewidth]{figures/fig1_2}
    % % \begin{equation*}
    % % \hspace{-3em}\text{\textit{maximize}}~\sum_{x\in C_K(X)} G(x)
    % % \end{equation*}
    % \end{minipage}~~%
    % \begin{minipage}{0.495\linewidth}
    % \includegraphics[width=0.9\linewidth]{figures/fig1_3}
    % % \begin{equation*}
    % % \hspace{-3em}\text{\textit{maximize}}~\sum_{x\in C_K(X)} H(x)
    % % \end{equation*}
    % \end{minipage}
        
    \end{figure}
    

==> tex/motivating_example.tex <==
\begin{figure*}[!htpb]
    \centering
    \begin{subfigure}[t]{0.49\linewidth}
        \includegraphics[width=\linewidth]{figures/motivating_example.pdf}
        \caption{A sample program and corresponding control-flow graph.}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.49\linewidth}
        \includegraphics[width=\linewidth]{figures/motivating_example_2.pdf}
        \caption{An example of fuzzing with \tool.}
    \end{subfigure}
    %\caption{A simple example of gradient guided fuzzing.}
    \caption{A motivating Example}
    \label{fig:motivate}
\end{figure*}


==> tex/pseudo.tex <==
\begin{figure}[t!]
    \raggedleft
    \includegraphics[width=\linewidth]{figures/pseudo.pdf}
\caption{{\small Pseudocode of saliency guided mutation.}}
\label{fig:pseudo}
\end{figure}


==> tex/pseudo_copy.tex <==
\renewcommand\thesubfigure{\alph{subfigure}}
\begin{figure*}[ht!]
\centering
\begin{minipage}{.45\linewidth}
\centering
\resizebox{0.925\linewidth}{!}{
\begin{subfigure}[t]{\linewidth}
\inputminted[bgcolor=codebg, numbersep=5pt, linenos=true, fontsize=\small]{c}{code/overall.py}
\vspace{-1.8em}
\caption{The overall framework of \tool}
\label{fig:general_framework}    
\end{subfigure}}\\[0.3em]
\resizebox{0.925\linewidth}{!}{
\begin{subfigure}[t]{\linewidth}
\inputminted[bgcolor=codebg, numbersep=5pt, linenos=true, fontsize=\small]{python}{code/get_cov.py}
\vspace{-1.8em}
\caption{Method to obtain edge coverage}
\label{fig:coverage}    
\end{subfigure}}%~
\end{minipage}\hspace{0.1em}%
\begin{minipage}{.5\linewidth}
\centering
\resizebox{0.925\linewidth}{!}{
\begin{subfigure}{\linewidth}
\inputminted[bgcolor=codebg, numbersep=5pt, linenos=true, fontsize=\small]{python}{code/seed_select.py}
\vspace{-2em}
\caption{Method to perform seed selection with importance sampling.}
\label{fig:seed_selection}    
\end{subfigure}}\\[-0.2em]
\resizebox{0.925\linewidth}{!}{
\begin{subfigure}{\linewidth}
\inputminted[bgcolor=codebg, numbersep=5pt, linenos=true, fontsize=\small]{python}{code/train_adaptive.py}
\vspace{-2em}
\caption{Method to compute adaptive loss for training neural network.}
\label{fig:train_adaptive}    
\end{subfigure}}\\[-0.2em]
\resizebox{0.925\linewidth}{!}{        
\begin{subfigure}{\linewidth}
\inputminted[bgcolor=codebg, numbersep=5pt, linenos=true, fontsize=\small]{python}{code/mutate.py}
\vspace{-2em}
\caption{Method to generate new inputs with gradient ascent.}
\label{fig:mutation}    
\end{subfigure}}
\end{minipage}\\[0.3em]
\caption{{\small Pseudocode of \tool.}}
\label{fig:pseudo}
\end{figure*}


==> tex/sl_eg.tex <==
\begin{wrapfigure}[16]{R}{0.45\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/approach_eg.pdf}
    % \vspace{-4mm}
    \caption{\small Approach Bitmap vs. Edge Bitmap. The edge `d' has a visited parent edge `b' and is thus marked 0.5 in the approach bitmap.}
    \label{fig:sl_eg}
    % \vspace{-3mm}
\end{wrapfigure}

==> tex/soft_label.tex <==
\begin{figure}[tbp!]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/soft_label_vertical.pdf}
    \caption{Soft labeling Example}
    \label{fig:soft_label}
\end{figure}

